DoS and DDoS Mitigation Using Variational Autoencoders

DoS and DDoS attacks have been growing in size and number over the last decade and existing solutions to mitigate these attacks are in general inefficient. Compared to other types of malicious cyber attacks, DoS and DDoS attacks are particularly more challenging to combat. With their ability to mask themselves as legitimate traffic, developing methods to detect these types of attacks on a packet or flow level, has proven to be a difficult task. In this paper, we explore the potential of Variational Autoencoders to serve as a component within an intelligent security solution that differentiates between normal and malicious traffic. Two methods based on the ability of Variational Autoencoders to learn latent representations from network traffic flows are proposed. The first method resorts to a classifier based on the latent encodings obtained from Variational Autoencoders learned from traffic traces. The second method is rather an anomaly detection method where the Variational Autoencoder is used to learn the abstract feature representations of exclusively legitimate traffic. Then anomalies are filtered out by relying on the reconstruction loss of the Variational Autoencoder. Both of the proposed methods have been thoroughly tested on two separate datasets with a similar feature space. The results show that both methods are promising, with a slight superiority of the classifier based method over the anomaly based one. %that the first method is able to successfully detect individual traffic flows with high precision on the training and validation data, slightly less successfully on the test data. For the second method, the Variational Autoencoder will require further adjustments to be able to sufficiently filter out anomalies from network traffic flows.

==> duoforside.tex <==
%% Standard headers:

\DeclareOption{american}{\def \duo@lang {eng}}
\DeclareOption{english}{\def \duo@lang {eng}}
\DeclareOption{UKenglish}{\def \duo@lang {eng}}
\DeclareOption{USenglish}{\def \duo@lang {eng}}
\DeclareOption{norsk}{\def \duo@lang {bm}}
\DeclareOption{nynorsk}{\def \duo@lang {nn}}

\ExecuteOptions{norsk}
\ProcessOptions \relax


%% Initial code:

\RequirePackage{graphicx,keyval,xifthen}
\IfFileExists{type1cm.sty}{\RequirePackage{type1cm}}{}
\IfFileExists{type1ec.sty}{\RequirePackage{type1ec}}{}
\RequirePackage[T1]{url}


%% The main command:

\newcommand{\duoforside}[1][]{{%
  \parindent = 0pt   \parskip = 0pt
  \@ifundefined{hypersetup}{}{\hypersetup{pageanchor=false}}
  \setkeys{duo@keys}{#1}
  \duo@page@i
  \@ifundefined{duo@thesisname@eng}
    {\if@twoside \duo@blankpage \fi}
    {\duo@page@ii \duo@page@iii \duo@page@iv}
  \setcounter{page}{1}
  \@ifundefined{hypersetup}{}{\hypersetup{pageanchor=true}}
}}

\newcommand{\duo@empty}{}

\newcommand{\duo@page@i}{%
  \begin{titlepage}
    \fontfamily{\duo@font}\fontencoding{T1}
    \def \and {\\}
    \centering
    \fontsize{16}{19pt}\selectfont
    \null\par
    \vspace*{-2cm}
    {\fontsize{24}{28pt}\selectfont \duo@title\par}
    \vspace{1\baselineskip}
    \ifx \duo@subtitle = \duo@empty
    \else
        {\fontsize{20}{23pt}\fontshape{sl}\selectfont \duo@subtitle\par}
        \vspace{1\baselineskip}
    \fi
    \duo@author\par
    \vspace{1\baselineskip plus 3fill}
    \includegraphics[width=6cm]{DUO_UiO_segl}\par
    \vspace{1\baselineskip plus 4fill}
    \ifx \duo@kind = \duo@empty
    \else
      \duo@kind\par
      \vspace{1\baselineskip}
    \fi
    \ifx \duo@dept = \duo@empty
    \else
      \duo@dept\par
    \fi
    \ifx \duo@fac = \duo@empty
    \else
      \duo@fac\par
      \vspace{1\baselineskip}
    \fi
    \MakeUppercase{\csname duo@uio@\duo@lang\endcsname}\par
    \vspace{1\baselineskip}
    {\fontsize{12}{14pt}\selectfont \duo@date\par}
    \vspace{-2cm}
    \null
  \end{titlepage}
}

\newcommand{\duo@page@ii}{%
  \duo@blankpage
}

\newcommand{\duo@page@iii}{%
  \begin{titlepage}
    \def \and {\\}
    \centering
    \null\vfill
    {\fontsize{24}{28pt}\fontseries{bx}\selectfont \@title\par}
    \vfill
    {\fontsize{20}{23pt}\fontshape{sl}\selectfont \duo@subtitle\par}
    \vfill
    {\fontsize{16}{18pt}\selectfont \@author\par}
    \vfill\vfill\vfill
    \ifthenelse{\equal{\duo@image}{}}{}
      {\includegraphics[keepaspectratio,width=10cm,height=8cm]{\duo@image}\par\vfill\vfill}
  \end{titlepage}
}

\newcommand{\duo@page@iv}{%
  \begin{titlepage}
    \null
    \vfill
    \raggedright
    \def \and {, }
    \textcopyright~\arabic{duo@cur@year} \duo@author\\[\baselineskip]
    \leavevmode\duo@title\\[\baselineskip]
    \url{http://www.duo.uio.no/}
    \ifthenelse{\equal{\duo@printer}{}}{}
      {\\[\baselineskip] \csname duo@printertitle@\duo@lang \endcsname:
        \duo@printer}
  \end{titlepage}
}


%% The options:

\define@key{duo@keys}{author}{\def \duo@author {#1}}
\define@key{duo@keys}{date}{\def \duo@date {#1}}
\define@key{duo@keys}{dept}{\def \duo@dept {#1}}
\define@key{duo@keys}{fac}{\def \duo@fac {#1}}
\define@key{duo@keys}{image}{\def \duo@image {#1}}
\define@key{duo@keys}{kind}{\def \duo@kind {#1}}
\define@key{duo@keys}{long}[60]{\def \duo@sp {#1}}
\define@key{duo@keys}{nosp}[0]{\def \duo@sp {#1}}
\define@key{duo@keys}{option}{\def \duo@opt {(#1)}}
\define@key{duo@keys}{printer}{\def \duo@printer {#1}}
\define@key{duo@keys}{program}{\def \duo@program{#1}}
\define@key{duo@keys}{short}[30]{\def \duo@sp {#1}}
\define@key{duo@keys}{subtitle}{\def \duo@subtitle {#1}}
\define@key{duo@keys}{title}{\def \duo@title {#1}}

\newcommand{\duo@uio@eng}{University of Oslo}
\newcommand{\duo@uio@bm}{Universitetet i Oslo}
\newcommand{\duo@uio@nn}{Universitetet i Oslo}

\newcommand{\duo@fac@eng}{Faculty of mathematics and natural sciences}
\newcommand{\duo@fac@bm}{Det matematisk-naturvitenskapelige fakultet}
\newcommand{\duo@fac@nn}{Det matematisk-naturvitenskaplege fakultet}

\def \duo@author {\@author}
\providecommand{\duo@date}{\today}
\def \duo@dept {}
\def \duo@fac {\csname duo@fac@\duo@lang \endcsname}
\def \duo@image {}
\providecommand{\duo@kind}{}
\def \duo@opt {}
\def \duo@printer {Reprosentralen, \csname duo@uio@\duo@lang \endcsname}
\providecommand{\duo@program}{}
\def \duo@sp {60}
\def \duo@title {\@title}


%% Additional commands:

\newcommand{\subtitle}[1]{\def \duo@subtitle{#1}}
\subtitle{}


%% Find the best font:

\newcommand{\duo@font}{phv}  % Helvetica is always available, but use
\IfFileExists{t1ua1.fd}{\renewcommand{\duo@font}{ua1}}{} % Arial if possible.


%% Determine the term (as in "Spring 2016"):

\newcounter{duo@cur@year}   \setcounter{duo@cur@year}{\the\year}
\newcounter{duo@cur@month}  \setcounter{duo@cur@month}{\the\month}

\ifthenelse{\theduo@cur@month<7}
  {\newcommand{\duo@term@eng}{Spring}%
   \newcommand{\duo@term@bm}{V\aa ren}%
   \newcommand{\duo@term@nn}{V\aa ren}}
  {\newcommand{\duo@term@eng}{Autumn}%
   \newcommand{\duo@term@bm}{H\o sten}%
   \newcommand{\duo@term@nn}{Hausten}}
\newcommand{\duo@term}{\csname duo@term@\duo@lang\endcsname}
\newcommand{\duo@year}{\arabic{duo@cur@year}}


%% Other utilities:

\newcommand{\duo@blankpage}{%
    \thispagestyle{empty}
    \null
    \newpage}

\endinput


==> parts/abstract.tex <==
\begin{document}

\chapter*{Abstract}

DDoS and DoS attacks have been growing in size and number over the last decade. Existing solutions employed to mitigate these attacks have proven to be inefficient in combating the problem. Compared to other types of malicious computer network traffic, DDoS and DoS attacks are particularly difficult to mitigate. With their ability to mask themselves as legitimate traffic, developing methods to detect attacks on a packet or flow level, has proven itself to be a difficult challenge.

Two methods based on the ability of a Variational Autoencoder to learn useful latent representations from network traffic flows are proposed, to differentiate between normal and malicious traffic. The first method is implemented as a classifier on the latent encodings of the Variational Autoencoder. The classifier learns through the abstract feature space of the encoder, based on input features extracted from  pre-generated traffic flows. In the second method, the Variational Autoencoder is used to learn the abstract feature representations of exclusively legitimate traffic. Then anomalies are filtered out through the reconstructed output of a Variational Autoencoder, based on their dissimilarities from the normal traffic probability distribution.

Both proposed methods have been thoroughly tested on two separate datasets with a similar feature space. The results show that the first method is able to successfully detect individual traffic flows with high precision on the training and validation data, slightly less successfully on the test data. For the second method, the Variational Autoencoder will require further adjustments to be able to sufficiently filter out anomalies from network traffic flows.


\end{document}


==> parts/analysis.tex <==
\begin{document}

\chapter{Analysis}
\label{analysis}

The performance of the two proposed approaches are measured by logging key features of the models, using Tensorboard plots, and confusion matrices. From Tensorboard, the graphs are plotted every 50 steps, where one step represents one batch (1,024) of flows being fed through a model. Graphs are plotted for the training dataset, the validation set, and the test set. The plotted graphs are of the prediction accuracy, P-Loss, KL-Loss, R-Loss\footnote{As discussed in \cref{methodology-llc-vae}}, and total loss mean values, as they develop over time during training, validation, and testing. The prediction accuracy mean values represents the mean accuracy of each batch. Recall back to \cref{methodology-datasets}, where the number of flows of the different flow types were presented. There is an overweight of benign traffic in the used datasets, which will influence the overall accuracy score by giving benign accuracy more weight. With this in mind, we will only use the mean accuracy score for development and performance improvement, and not as a metric to show model results. As an alternative, we can also use less benign flows, or only draw a certain percentage from each traffic type, from the datasets. To determine how well each model performs on different tuning settings, we will use confusion matrices to show the overall benign versus malicious flow traffic accuracy. As well as the accuracy within individual attack classes, separated and unaffected by the other flow accuracy scores.

\section{LLC-VAE Results}

The first approach that will be analyzed is the LLC-VAE. We will begin with training the model on the settings defined by the presets from \cref{experimental-setup}, \nameref{experimental-setup}, defined in table \ref{tab:es-presets}. After that, we will analyze model performance when fine tuning the model settings, to see how precise the LLC-VAE can become. For all training runs, we will be using the CSECICIDS2018 dataset, with a 60-40 split between the training set and validation set respectively, unless noted otherwise. The training set has been modified to contain an equal amount of benign and malicious flows, to prevent learning bias. For the test set, we will be using the whole CICIDS2017 dataset.

\subsection{Performance of the Presets}
\label{analysis-preset-performance}

Overview of the LLC-VAE performance on the presets.

\subsubsection{Preset 1}

The first training run, on preset 1 \ref{tab:es-p1}, did not perform well. After just 400 steps, the accuracy stops improving, and does not improve past 50\%, as seen in figure \ref{fig:p1-tr-acc}. This means that the model predictions are done more or less at random, since the training dataset has a 1 to 1 ratio between benign and malicious traffic. The overall loss starts as a NaN value and does not improve over time. As seen in figure \ref{fig:p1-tr-total} the total loss is even out bounds of the graph.

The first preset does not perform any scaling on the flow features, only on each individual flow across the features, with batch normalization. This is most likely to be the explanation for why the loss is out of bounds, and for why the accuracy does not improve past 50\%. In machine learning, higher learning rates generally means that neural networks converge faster, but can lead to too large weight value updates every iteration, ruining the previous weight values. This could lead to worse and unstable end results, as can be seen in figure \ref{fig:p1-tr-acc}. By looking at the accuracy and total loss plots from figure \ref{fig:p1-summaries}, it is obvious that preset 1 should not be used for training the LLC-VAE.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p1_tr_acc.csv}{Accuracy}{scale=0.6}
        \caption{P1 Accuracy}
        \label{fig:p1-tr-acc}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p1_tr_tloss.csv}{Value}{scale=0.6}
        \caption{P1 Total Loss}
        \label{fig:p1-tr-total}
    \end{subfigure}
    \caption[Preset 1 Results]{Training results for preset 1. Note that the total loss graph has no plot, this is \textbf{not an error}, as the loss values grew out of bounds.}
    \label{fig:p1-summaries}
\end{figure}

\subsubsection{Preset 2}

Training with preset 2 \ref{tab:es-p2} showed improved results for the training and validation sets in regards to overall accuracy and loss, as seen in figure \ref{fig:p2-summaries}, and is an improvement to the results from preset 1, as seen in \ref{fig:p1-summaries}. The graphs are jittery, seen by how the graphs spike between relatively large values. This could point to the learning rate being the culprit, which remained the same from preset 1, or that the model overfits towards specific types of traffic flows. The main difference between preset 1 and 2, is that preset 2 uses normalization of the datasets. As discussed previously in \cref{methodology-scaling}, there are multiple features in the dataset lacking true max and min values, this was solved by sampling from the training dataset, CSECICIDS2018. Normalization with sampled max and min values were not as beneficial for testing as it was for training and validation. Since we sampled from the CSECICIDS2018 dataset, the model was unable to generalize, because the two datasets have different feature distributions. The test results showed bad overall accuracy, and did not improve after step 450. From figure \ref{fig:p2-tr-total}, we can see that the total loss decreases very quickly, then has trouble stabilizing, which explains why the accuracy was unstable as well. The loss values from training, validation, and testing spiked occasionally to relatively large values. Sometimes they spiked to NaN values, showing that something is very wrong with preset 2. This is likely due to the sampled max and min not providing a good representation for the test set, CICIDS2017.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p2_tr_acc.csv}{Accuracy}{scale=0.6}
        \caption{P2 Training Accuracy}
        \label{fig:p2-tr-acc}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p2_tr_tloss.csv}{Value}{scale=0.6}
        \caption{P2 Training Total Loss}
        \label{fig:p2-tr-total}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p2_te_acc.csv}{Accuracy}{scale=0.6}
        \caption{P2 Test Accuracy}
        \label{fig:p2-te-acc}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p2_te_tloss.csv}{Value}{scale=0.6}
        \caption{P2 Test Total Loss}
        \label{fig:p2-te-total}
    \end{subfigure}
    \caption[Preset 2 Results]{Training and test results for preset 2.}
    \label{fig:p2-summaries}
\end{figure}
\FloatBarrier

\subsubsection{Preset 3}

For preset 3 \ref{tab:es-p3}, the training is much more stable in comparison to the last two presets, as the learning rate has been reduced to $1 \cdot 10^{-4}$, as seen in figure \ref{fig:p3-summaries}. The training accuracy converges at above 99\% accuracy, at around step 26,000, as seen in figure \ref{fig:p3-tr-accuracy}. Preset 3 was overall an improvement to the previous two presets, and achieved much better test results. Still, the test results were unsatisfactory, and the P-Loss gets increasingly worse after step 2,000, as seen in figure \ref{fig:p3-te-ploss}. One of the settings changed from the previous preset, is that we are now using normalization on the datasets, with min and max values sampled from both the training set and the test set. This is likely to be the reason why the test results have improved. Important to note is that this was done to try out normalization with more accurate min and max values, but will not be used as a final solution. This is because sampling from the test set goes against the principle of using a test set. It is supposed to be data we do not have access to during training. It should only be used for testing, and not as part of the implementation.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p3_tr_acc.csv}{Accuracy}{scale=0.6}
        \caption{P3 Training Accuracy}
        \label{fig:p3-tr-accuracy}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p3_tr_tloss.csv}{Value}{scale=0.6}
        \caption{P3 Training Total Loss}
        \label{fig:p3-tr-tloss}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p3_te_acc.csv}{Accuracy}{scale=0.6}
        \caption{P3 Test Accuracy}
        \label{fig:p3-te-acc}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p3_te_tloss.csv}{Value}{scale=0.6}
        \caption{P3 Test Total Loss}
        \label{fig:p3-te-tloss}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p3_tr_kloss.csv}{Value}{scale=0.6}
        \caption{P3 Training KL Loss}
        \label{fig:p3-tr-kloss}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p3_te_ploss.csv}{Value}{scale=0.6}
        \caption{P3 Test Prediction Loss}
        \label{fig:p3-te-ploss}
    \end{subfigure}
    \caption[Preset 3 Results]{Training and test results for preset 3.}
    \label{fig:p3-summaries}
\end{figure}
\FloatBarrier

\subsubsection{Preset 4}

For preset 4 \ref{tab:es-p4} the training results remained on par with the results from preset 3. We reduced the KL-Loss multiplier even further in preset 4, which made the KL-Loss improve slower compared to in preset 3, but still managed to decrease over time, see figure \ref{fig:p4-tr-kloss} compared to figure \ref{fig:p3-tr-kloss}. It seems the KL-Loss value does not have a large, positive impact on the overall accuracy scores, as seen when comparing figure \ref{fig:p4-summaries} for preset 4, and \ref{fig:p3-summaries} for preset 3. For the test set, there was a significant improvement to both overall accuracy and P-Loss, as see in figure \ref{fig:p4-te-ploss} for preset 4, and \ref{fig:p3-te-ploss} for preset 3. The P-Loss continued to decrease over time until it converged at around step 28,000, as seen in figure \ref{fig:p4-te-ploss}. Logarithmic scaling seems to be a superior method of scaling the datasets as compared to the other scaling approaches tried on previous presets. This makes the process of scaling better suited for a generalized solution, since it does not rely on knowing the total population min, max, mean, or standard deviation values.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p4_tr_acc.csv}{Accuracy}{scale=0.6}
        \caption{P4 Training Accuracy}
        \label{fig:p4-tr-acc}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p4_tr_tloss.csv}{Value}{scale=0.6}
        \caption{P4 Training Total Loss}
        \label{fig:p4-tr-tloss}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p4_te_acc.csv}{Accuracy}{scale=0.6}
        \caption{P4 Test Accuracy}
        \label{fig:p4-te-acc}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p4_te_tloss.csv}{Value}{scale=0.6}
        \caption{P4 Test Total Loss}
        \label{fig:p4-te-tloss}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p4_tr_kloss.csv}{Value}{scale=0.6}
        \caption{P4 Training KL Loss}
        \label{fig:p4-tr-kloss}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p4_te_ploss.csv}{Value}{scale=0.6}
        \caption{P4 Test Prediction Loss}
        \label{fig:p4-te-ploss}
    \end{subfigure}
    \caption[Preset 4 Results]{Training and Test results for preset 4.}
    \label{fig:p4-summaries}
\end{figure}
\FloatBarrier

\subsubsection{Preset 5}

For preset 5 \ref{tab:es-p5}, we kept the logarithmic scaling of the datasets, only changing the hidden layer architecture. Instead of using convolutional layers, we used fully connected layers for the encoder and decoder. The results showed preset 5 to be mostly on par with preset 4 in terms of training accuracy, although slightly worse. Important to note, as seen in the figures of preset 5 \ref{fig:p5-tr-tloss} and preset 4 \ref{fig:p5-tr-tloss}, the total loss of preset 5 is noticeably larger than compared to the total loss of preset 4. How large any loss value is for each different run is inconsequential to the model performance, what is important, is that it improves over time. Between preset 4 \ref{fig:p4-te-acc} and preset 5 \ref{fig:p5-te-acc} the biggest difference was in the test set accuracy, where preset 5 showed noticeably worse results, and converged already at about step 7,000. As shown by both the results from preset 4 \ref{fig:p4-summaries} and 5 \ref{fig:p5-summaries}, logarithmic scaling of the datasets, and convolutional layers for the encoder and decoder, has so far been the optimal choice, when compared to previous results.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p5_tr_acc.csv}{Accuracy}{scale=0.6}
        \caption{P5 Training Accuracy}
        \label{fig:p5-tr-acc}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p5_tr_tloss.csv}{Value}{scale=0.6}
        \caption{P5 Training Total Loss}
        \label{fig:p5-tr-tloss}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p5_te_acc.csv}{Accuracy}{scale=0.6}
        \caption{P5 Test Accuracy}
        \label{fig:p5-te-acc}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p5_te_tloss.csv}{Value}{scale=0.6}
        \caption{P5 Test Total Loss}
        \label{fig:p5-te-tloss}
    \end{subfigure}
    \caption[Preset 5 Results]{Training and Test results for preset 5.}
    \label{fig:p5-summaries}
\end{figure}
\FloatBarrier

\subsubsection{Preset 6}

To see how well the LLC-VAE performs compared to other deep learning frameworks, we have included a simple, convolutional network. It will be used as a baseline for analyzing whether a VAE is a worthwhile architecture to base a DDoS and DoS mitigation system on. Preset 6 \ref{tab:es-p6} has the same neural network structure as preset 4, but we no longer use the KL-Loss from the latent layer, and the R-Loss from the decoder, only the P-Loss. This means that preset 6 is simply a convolutional neural network that performs dimensionality reduction, and data classification.

Preset 6 showed promising results for training accuracy. Compared with the training accuracy of preset 4 \ref{fig:p4-tr-acc}, the accuracy of preset 6 \ref{fig:p6-tr-acc} were mostly on par, but performed slightly better. For the test results \ref{fig:p6-summaries}, this preset showed results on par with preset 4 \ref{fig:p4-summaries}, but still not a good enough generalization. Compared with preset 4, preset 6 showed more uncertainty in terms of test accuracy, as seen by how the graph is jittery in figure \ref{fig:p6-te-acc}, so preset 4 might be better as a generalized solution. Looking back at figure \ref{fig:p4-summaries}, preset 4 had yet to converge on a solution before it was stopped. Given more time, it might prove to be as good, or better than preset 6 in terms of training, validation, and test results.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p6_tr_acc.csv}{Accuracy}{scale=0.6}
        \caption{P6 Training Accuracy}
        \label{fig:p6-tr-acc}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p6_tr_tloss.csv}{Value}{scale=0.6}
        \caption{P6 Training Total Loss}
        \label{fig:p6-tr-tloss}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p6_te_acc.csv}{Accuracy}{scale=0.6}
        \caption{P6 Test Accuracy}
        \label{fig:p6-te-acc}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p6_te_tloss.csv}{Value}{scale=0.6}
        \caption{P6 Test Total Loss}
        \label{fig:p6-te-tloss}
    \end{subfigure}
    \caption[Preset 6 Results]{Training and test results for preset 6.}
    \label{fig:p6-summaries}
\end{figure}
\FloatBarrier

%\begin{figure}[htbp]
%    \centering
%    \includegraphics[scale=0.5]{img/cm/p6_va.pdf}
%    \caption[Preset 6 Confusion Matrix of Validation Dataset]{Confusion matrix of validation dataset for preset 6.}
%    \label{fig:p6-va-cm}
%\end{figure}

\subsection{Further Adjustments}

In the following subsections, we will present further adjustments to the two most promising presets, preset 4 \ref{tab:es-p4} and preset 6 \ref{tab:es-p6}. Compared with the other presets, preset 4 and preset 6 had the overall best test results, and achieved much higher test accuracy, as can be seen in figure \ref{fig:p4-te-acc} for preset 4, and \ref{fig:p6-te-acc} for preset 6. We use the test accuracy as the deciding factor for choosing to build on these presets, because it is the best metric to show how well the LLC-VAE generalizes. The further adjustments will be used to discuss how the LLC-VAE can be improved further, and analyze whether it can be considered as a method for creating a mitigation system.

\subsubsection{LIME}
\label{analysis-lime}

In addition to the feature selection done by the convolutional layers, and the selection through dimensionality reduction by the encoder of the LLC-VAE model, we can manually select what input features the model should learn from. Using LIME\cite{Ribeiro-et-al-2016}, we can analyze how the presets weighed each feature, to find out which ones had the largest, and which ones had the smallest impact on the learning process. LIME shows how much impact each input feature from a flow, had on a prediction. An example of how LIME visualize the prediction probabilities for a single flow can be seen in figure \ref{fig:lime_example}. The flow from the example figure has been predicted to be a DoS Hulk attack, with a probability of 62\%. On the right hand side, we can see the top six most impactful input features, in order from most to least. Features on the side named "Not DoS Hulk", weighs against this particular flow being predicted to be a DoS Hulk attack, and vice versa for the opposite side named "DoS Hulk". The number next to each feature name represents how much they are weighted by the model, rounded to the closest, second decimal point. We can use LIME to understand how the LLC-VAE classifies flows, as well as for manual feature removal, to ensure better generalization.

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.8]{img/figures/lime_example.pdf}
    \caption[LIME Example For a Single Flow]{LIME example figure for a single flow. Result achieved by running LIME on the LLC-VAE using preset 4 \ref{tab:es-p4}.}
    \label{fig:lime_example}
\end{figure}

To find out which input features were the most influential on the LLC-VAE training process, we ran LIME on the model after it was trained using preset 4, with the same training and validation datasets that were used previously. Running LIME is a time consuming process, so we have shortened the process by using a sample size of 50,000 flows. This produced a list of the most impactful features, in sorted order.

\begin{table}
\centering
\arrayrulecolor{black}
\resizebox{\columnwidth}{!}{
\begin{tabular}{llll}
\hline
Column 1          & Column 2         & Column 3         & Column 4                                                    \\
\arrayrulecolor{black}\hline
Bwd IAT Std       & Bwd Pkt Len Mean & Fwd Header Len   & Fwd IAT Tot                                                 \\
Pkt Len Mean      & Bwd Pkt Len Max  & Pkt Len Std      & Bwd Pkt Len Min                                             \\
Fwd IAT Max       & Active Min       & Fwd Pkt Len Max  & Bwd IAT Tot                                                 \\
Bwd IAT Min       & Idle Max         & TotLen Fwd Pkts  & Flow IAT Max                                                \\
Dst Port          & Flow Duration    & Subflow Fwd Byts & Bwd Header Len                                              \\
Init Bwd Win Byts & Bwd Pkt Len Std  & Flow IAT Min     & Subflow Fwd Pkts                                            \\
Pkt Size Avg      & Fwd IAT Std      & Fwd IAT Mean     & Active Std                                                  \\
Pkt Len Max       & Bwd IAT Mean     & Flow IAT Mean    & TotLen Bwd Pkts                                             \\
Idle Mean         & Pkt Len Var      & Fwd Seg Size Avg & Idle Min                                                    \\
Init Fwd Win Byts & Bwd IAT Max      & Fwd IAT Min      & Pkt Len Min
\end{tabular}
} %End resizebox
\caption[Top Features After LIME]{Top 40 features remaining after using LIME on the LLC-VAE with preset 4 \ref{tab:es-p4}. The features are ordered from most to least impactful, from top to bottom and left to right.}
\label{tab:lime_top}
\end{table}

\subsubsection{Results After Feature Selection With LIME}

To test whether manual feature selection is constructive for the LLC-VAE model performance, we tried to remove the least impactful features, only keeping the top 40, as seen in table \ref{tab:lime_top}. By removing the least impactful features, we allow the model to emphasize more on the remaining features. This could help prevent overfitting, since the model no longer tries to learn from less important data. Another method could be to select individual features, if they are deemed to be potential causes for overfitting. Doing so would be much more time consuming, and will not be done for this thesis, but will be discussed further in \cref{discussion-selection}.

The confusion matrices from figure \ref{fig:p4-te-cm}, and figure \ref{fig:p6-te-cm}, shows the test results of of preset 4 and preset 6 respectively, before performing manual feature selection with LIME\footnote{Note that at the bottom of the confusion matrices, there are no LOIC-UDP or HOIC-HTTP attacks. This is because the test dataset contains no samples for those attack types, as described in \cref{methodology-datasets}.}. Preset 6 showed slightly better benign accuracy than preset 4, but both models had trouble classifying the malicious traffic flows. Preset 4 were particularly bad at classifying the attack \texttt{DoS SlowHTTPTest}, while preset 6 were mostly unable to classify the attacks \texttt{DoS Slowloris} and \texttt{DoS SlowHTTPTest}. Recall back to table \ref{tab:methodology-2018}, showing the number of flows for each flow type from the training dataset, CSECICIDS2018. \texttt{DoS Slowloris} had relatively few samples compared with the other attack types, which could explain why the convolutional network, using preset 6, were unable to generalize well enough to correctly classify this attack. The attack \texttt{DoS SlowHTTPTest} had relatively many flow samples in the training set, but the LLC-VAE and the convolutional network was still unable to generalize well, using preset 4 and  respectively 6. This conceptualizes the idea that the attack \texttt{DoS SlowHTTPTest} is too similar to to benign traffic flows for the LLC-VAE and the convolutional network, using preset 4 and 6, to classify it correctly.

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.4]{img/cm/p4_te.pdf}
    \caption[Preset 4 Confusion Matrix of Test Dataset]{Confusion matrix of test dataset for preset 4.}
    \label{fig:p4-te-cm}
\end{figure}

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.4]{img/cm/p6_te.pdf}
    \caption[Preset 6 Confusion Matrix of Test Dataset]{Confusion matrix of test dataset for preset 6.}
    \label{fig:p6-te-cm}
\end{figure}

After having used LIME to find the least impactful features, we kept the top 40 most impactful features, as seen in table \ref{tab:lime_top}, and ran more tests on variations of preset 4 and preset 6, as seen in table \ref{tab:presets-a}. Since differentiating between individual attack classes seemed difficult for the LLC-VAE to handle, we decided to compress them into one class named \texttt{malicious}, and instead perform binary classification. In addition to this, we have also changed the latent layer size, by changing the convolutional layers. For preset 4 and preset 6, the kernel size was 5 for each layer, and the first layer had a stride size of 2, as described in \cref{es-parameters}. The kernel size remains the same for these tests, at a size of 5, but now each of the layers have a stride size of 1. Hence the top 40 input features, \ref{tab:lime_top}, will be reduced to 28 abstract features in the latent layer, from dimensionality reduction. The confusion matrix for the test results on preset \textbf{4a} \ref{tab:p4a} can be seen in figure \ref{fig:p4-improved-LIME}, and the test results on preset \textbf{6a} \ref{tab:p6a} can be seen in figure \ref{fig:p6-improved-LIME}. From both figures, we can see that the benign accuracy has decreased by about 2\%, but the malicious accuracy has increased dramatically. As discussed previously, preset 6, and inherently 6a, is a simple, reducing convolutional network, and is used for baseline comparison with the LLC-VAE performance. The LLC-VAE performed less than 1\% worse in terms of benign accuracy, but almost 5\% better in terms of malicious accuracy. Overall the LLC-VAE performed better for this test, but could still improve with some fine tuning.

\begin{table}[htbp]
    \begin{subtable}[b]{0.4\textwidth}
        \caption{Preset 4a}
        \label{tab:p4a}
        \centering
        \arrayrulecolor{black}
        \begin{tabular}{l|r}
            \hline
            Parameter & Value                                             \\
            \arrayrulecolor{black}\hline
            Preset    & 4                                 \\
            CT        & Binary                                                \\
            Steps     & 30,000                                            \\
            Features  & 40                                              \\
            KS        & 5                                              \\
            Stride    & 1-1-1                                            \\
        \end{tabular}
    \end{subtable}
    \hfill
    \begin{subtable}[b]{0.4\textwidth}
        \caption{Preset 6a}
        \label{tab:p6a}
        \centering
        \arrayrulecolor{black}
        \begin{tabular}{l|r}
            \hline
            Parameter & Value                                             \\
            \arrayrulecolor{black}\hline
            Preset    & 6                                 \\
            CT        & Binary                                                \\
            Steps     & 30,000                                            \\
            Features  & 40                                              \\
            KS        & 5                                              \\
            Stride    & 1-1-1                                            \\
        \end{tabular}
    \end{subtable}
    \caption[Preset 4a and Preset 6a]{Modified preset 4 \ref{tab:es-p4} and preset 6 \ref{tab:es-p5}. The parameters are as follows; \texttt{Preset} is the base preset, \texttt{CT} is short for classification type, \texttt{Features} specifies the number of input features, \texttt{KS} is short for kernel size. \texttt{Stride} specifies the stride size in the format $i_{1}-i_{2}-i_{3}$, where $i$ is the size of the first, second, and third layer respectively.}
    \label{tab:presets-a}
\end{table}


\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[scale=0.4]{img/cm/p4_te_modified_19_numbers.pdf}
        \caption{Amount of flows for each classification.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[scale=0.4]{img/cm/p4_te_modified_19.pdf}
        \caption{Accuracy values for each classification.}
    \end{subfigure}
    \caption[Confusion Matrix of Test Dataset on Preset 4a]{Confusion matrix of the test results on preset 4a.}
    \label{fig:p4-improved-LIME}
\end{figure}

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[scale=0.4]{img/cm/p6_te_modified_17_numbers.pdf}
        \caption{Amount of flows for each classification.}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[scale=0.4]{img/cm/p6_te_modified_17.pdf}
        \caption{Accuracy values for each classification.}
    \end{subfigure}
    \caption[Confusion Matrix of Test Dataset on Preset 6a]{Confusion matrix of the test results on preset 6a.}
    \label{fig:p6-improved-LIME}
\end{figure}
\FloatBarrier

From earlier, when we trained the six presets \ref{analysis-preset-performance}, reducing the KL-Loss multiplier showed some improvement on overall model performance. We tried to reduce it even further with preset 4b \ref{tab:p4b}, changing the multiplier to $1 \cdot 10^{-6}$ and number of steps to 50,000. The result of doing so can be seen in figure \ref{fig:p4-improved-kl}. The benign accuracy remained mostly the same as when using a KL-Loss multiplier of $1 \cdot 10^{-4}$, but the malicious accuracy increased by more than 3\%, compared with the results of preset 4a \ref{fig:p4-improved-LIME}. Further reducing the KL-Loss multiplier caused the LLC-VAE model performance to degrade, pointing to a multiplier of $1 \cdot 10^{-6}$ to provide the best results.

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.4]{img/cm/p4_te_kl_26.pdf}
    \caption[Confusion Matrix of Test Dataset on Preset 4a With Reduced KL-Loss Multiplier]{Confusion matrix of the test results on preset 4b, after adjusting the KL-Loss multiplier from $1 \cdot 10^{-4}$ to $1 \cdot 10^{-6}$.}
    \label{fig:p4-improved-kl}
\end{figure}

\subsubsection{Adjusting Receptive Field}

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.5]{img/figures/receptive_field_3x13-2x2-1x1.pdf}
    \caption[Receptive Field Example]{Example figure of the receptive field size for a model using three layers, a kernel size of 13, and the first two layers having a stride size of 2.}
    \label{fig:receptive-field}
\end{figure}

The tuning presets that were used to train the LLC-VAE worked as a way to try different methods for improving the model, as well as to see which settings worked, and which settings did not. Both preset 4a \ref{tab:p4a} and preset 6a \ref{tab:p6a} used convolutional layers for the encoder and decoder. Within convolutional layers, it is possible to adjust the kernel size and the stride size of the sliding window, as discussed in \cref{methodology-conv-layers}. By doing so, we can adjust the effective size of the receptive field of the latent layer, to make it learn an abstraction of the relations between a larger or smaller number of features in the input layer.

All of the original six presets \ref{tab:es-presets} uses a kernel size of 5, where the first layer has a stride size of 2, which leads the latent layer to have an effective receptive field size of 21. This means that each latent layer node is able to learn relations between 21 adjacent input features. In order for each node in the latent layer to learn from the relations between all the original 76 input features, as seen in table \ref{tab:methodology-features}, the kernel size of each layer needs to be set to 13, and the first two layers need a stride size of 2. A figure showing how the theoretical receptive field increases in this case, can be seen in \ref{fig:receptive-field}.

\begin{table}[htbp]
    \begin{subtable}[b]{0.4\textwidth}
        \caption{Preset 4b}
        \label{tab:p4b}
        \centering
        \arrayrulecolor{black}
        \begin{tabular}{l|r}
            \hline
            Parameter & Value                                             \\
            \arrayrulecolor{black}\hline
            Preset    & 4a                                 \\
            KLM       & $1 \cdot 10^{-6}$                                                \\
            Steps     & 50,000                                            \\
            Features  & 40                                              \\
            KS        & 5                                              \\
            Stride    & 1-1-1                                            \\
        \end{tabular}
    \end{subtable}
    \hfill
    \begin{subtable}[b]{0.4\textwidth}
        \caption{Preset 4c}
        \label{tab:p4c}
        \centering
        \arrayrulecolor{black}
        \begin{tabular}{l|r}
            \hline
            Parameter & Value                                             \\
            \arrayrulecolor{black}\hline
            Preset    & 4a                                 \\
            KLM       & $1 \cdot 10^{-6}$                                                 \\
            Steps     & 140,000                                            \\
            Features  & 40                                              \\
            KS        & 7                                              \\
            Stride    & 2-2-1                                            \\
        \end{tabular}
    \end{subtable}
    \caption[Preset 4b and Preset 4c]{Two modifications on preset 4a \ref{tab:p4a}. As from earlier, \texttt{KLM} is short for KL-Loss multiplier.}
    \label{tab:presets-bc}
\end{table}

The best results has thus far been achieved after training the model on preset \textbf{4b} \ref{tab:p4b} with a KL-Loss multiplier of $1 \cdot 10^{-6}$, as seen in figure \ref{fig:p4-improved-kl}, with the reduced input feature set from table \ref{tab:lime_top}. To achieve an effective receptive field size that covers all the 40 features from the reduced input feature set, we adjusted the kernel size of the convolutional layers to 7, and the first and second layer to have a stride size of 2, as seen in preset \textbf{4c} \ref{tab:p4c}. This gives the latent layer nodes a theoretical receptive field size that covers 43 features. From figure \ref{fig:p4-latent-left}, we see the accuracy plot of the LLC-VAE performance using preset 4b on the validation set. From figure \ref{fig:p4-latent-right}, we see the accuracy plot of the LLC-VAE performance using preset 4c on the same set. We can see from figure \ref{fig:p4-modified-latent-26-35} that increasing the receptive field size did not improve the validation accuracy, but rather degraded it. The model converged to a solution at about step 130,000.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p4_modified_26_va_acc.csv}{Accuracy}{scale=0.6}
        \caption{Preset 4b}
        \label{fig:p4-latent-left}
    \end{subfigure}
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard/p4_modified_35_va_acc.csv}{Accuracy}{scale=0.6}
        \caption{Preset 4c}
        \label{fig:p4-latent-right}
    \end{subfigure}
    \caption[Validation Accuracy When Changing Receptive Field Size]{Comparison of the validation accuracy when using two different receptive field sizes with the LLC-VAE on preset 4b and 4c.}
    \label{fig:p4-modified-latent-26-35}
\end{figure}
\FloatBarrier

\subsubsection{Other Changes}

To better understand what works well and what does not, for the LLC-VAE, we have tried further fine tuning of the model based on preset 4, as well as the improvements done with LIME and the modifications on the convolutional layers. We have tried to adjust the KL-Loss multiplier, and ended up with a multiplier of $1 \cdot 10^{-6}$, as seen in preset 4b \ref{tab:p4b}, to show the best performance. Adjusting the P-Loss or R-Loss multipliers showed no improvements. Further adjustments of the convolutional layers showed that the optimal settings for the kernel sizes were 5 with a stride size of 1 for all layers, leading to a latent layer size of 28. Both larger and smaller latent layer sizes showed worse end results, even though larger latent layer sizes caused the model to converge faster.

Earlier, when discussing the datasets, we could see that some of the malicious traffic flows from the training set CSECICIDS2018 had few samples, see \cref{methodology-2018}. The attacks \texttt{DoS Slowloris}, \texttt{DoS Goldeneye}, and \texttt{DDoS LOIC-UDP} had relatively few samples compared to the other attack classes. To test whether this negatively impacted the training process, we removed them for a training run. Contrary to our initial beliefs, removing these attacks from the training set decreased model accuracy. The training and validation accuracy remained the same as before, but the test accuracy degraded. This could point to the model generalizing better when subjected to a variety of different attack types with few samples.

Amongst the features that were removed after using LIME, the source IP and destination IP addresses were also removed. It is common for mitigation systems, when determining whether a network packet or flow is an attack or not, to analyze the source and destination IP addresses. By doing so, a mitigation system can determine the intent of the source by connecting their IP address to their behavior and traffic frequency. The LLC-VAE however, performed better after removing the IP addresses, improving overall model performance for the test dataset. We performed a training run on the settings used with preset 4 \ref{tab:es-p4} where we removed the IP address input features, and got the test results seen in figure \ref{fig:p4-noip}. Figure \ref{fig:p4-ip} shows the confusion matrix for preset 4 when performing binary classification, which used the IP addresses during training. The benign detection accuracy decreased by about 1\% when removing the IP addresses. The malicious detection accuracy increased by about 16\%, which is a significant leap in overall model performance. This points to the LLC-VAE overfitting on the IP address input features, learning specific IP addresses instead of the relationships between the IP addresses and the other input features. More about this in \cref{discussion-simulated}.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[scale=0.4]{img/cm/p4_te_anomaly.pdf}
        \caption{With IP addresses.}
        \label{fig:p4-ip}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[scale=0.4]{img/cm/p4_te_noIP.pdf}
        \caption{Without IP addresses.}
        \label{fig:p4-noip}
    \end{subfigure}
    \caption[Preset 4 Test Results Comparison, With and Without IP Addresses]{Comparison of test results of preset 4, with and without IP addresses.}
    \label{fig:p4-ip-and-noip}
\end{figure}

\section{LBD-VAE Results}
\label{analysis-lbd-results}

The second approach, LBD-VAE, will use similar tuning settings to the first approach. The presets will not be used directly, but variations will be tested, based on the findings of what worked well for the LLC-VAE, these new settings can be seen in table \ref{tab:lbd-settings}. The LBD-VAE consists of two different models that need to be trained in order, where the first model is trained in isolation from the second one, as seen in figure \ref{fig:methodology-lbd}. As was done previously, all training runs will use the CSECICIDS2018 dataset with a 60-40 split between the training set and the validation set respectively. The training set has been modified to contain an equal amount of benign and malicious flows, to prevent learning bias.

\subsection{Performance}

\begin{table}[htbp]
    \begin{subtable}[b]{0.4\textwidth}
        \caption{LBD-preset 1}
        \label{tab:lbd-s1}
        \centering
        \arrayrulecolor{black}
        \begin{tabular}{l|r}
            \hline
            Parameter & Value                                             \\
            \hline
            LR        & $1 \cdot 10^{-4}$                                 \\
            KLM       & 1                                                 \\
            Steps 1   & 20,000                                            \\
            Steps 2   & 30,000                                            \\
            ST        & Log                                               \\
            LT        & Conv                                              \\
            RLT       & Batch                                             \\
            Features  & 76                                                \\
            KS        & 5                                                 \\
            Stride    & 2-1-1                                             \\
        \end{tabular}
    \end{subtable}
    \hfill
    \begin{subtable}[b]{0.4\textwidth}
        \caption{LBD-preset 2}
        \label{tab:lbd-s2}
        \centering
        \arrayrulecolor{black}
        \begin{tabular}{l|r}
            \hline
            Parameter & Value                                             \\
            \hline
            LR        & $1 \cdot 10^{-4}$                                 \\
            \rowcolor{Gray}
            KLM       & 4                                                 \\
            Steps 1   & 20,000                                            \\
            Steps 2   & 30,000                                            \\
            ST        & Log                                               \\
            LT        & Conv                                              \\
            RLT       & Batch                                             \\
            \rowcolor{Gray}
            Features  & 40                                                \\
            KS        & 5                                                 \\
            \rowcolor{Gray}
            Stride    & 1-1-1                                             \\
        \end{tabular}
    \end{subtable}
    \hfill
    \begin{subtable}[b]{0.4\textwidth}
        \caption{LBD-preset 3}
        \label{tab:lbd-s3}
        \centering
        \arrayrulecolor{black}
        \begin{tabular}{l|r}
            \hline
            Parameter & Value                                             \\
            \hline
            LR        & $1 \cdot 10^{-4}$                                 \\
            \rowcolor{Gray}
            KLM       & $1 \cdot 10^{-6}$                                 \\
            \rowcolor{Gray}
            Steps 1   & 1,500                                             \\
            Steps 2   & 30,000                                            \\
            ST        & Log                                               \\
            LT        & Conv                                              \\
            RLT       & Batch                                             \\
            Features  & 40                                                \\
            KS        & 5                                                 \\
            Stride    & 1-1-1                                             \\
        \end{tabular}
    \end{subtable}
    \hfill
    \begin{subtable}[b]{0.4\textwidth}
        \caption{LBD-preset 4}
        \label{tab:lbd-s4}
        \centering
        \arrayrulecolor{black}
        \begin{tabular}{l|r}
            \hline
            Parameter & Value                                             \\
            \hline
            LR        & $1 \cdot 10^{-4}$                                 \\
            KLM       & $1 \cdot 10^{-6}$                                 \\
            \rowcolor{Gray}
            Steps 1   & 100,000                                           \\
            Steps 2   & 30,000                                            \\
            ST        & Log                                               \\
            LT        & Conv                                              \\
            RLT       & Batch                                             \\
            Features  & 40                                                \\
            \rowcolor{Gray}
            KS        & 7                                                 \\
            \rowcolor{Gray}
            Stride    & 2-2-1                                             \\
        \end{tabular}
    \end{subtable}
    \caption[Settings for the LBD-VAE Model]{Settings for the LBD-VAE Model. Steps 1 is the number of iterations for "model 1", steps 2 is the number of iterations for "model 2".}
    \label{tab:lbd-settings}
\end{table}
\FloatBarrier

For the first training run, we used all the original 76 input features from table \ref{tab:methodology-features}. The first model was trained exclusively on benign traffic flows, so that the reconstruction loss would become low for benign traffic, and higher for malicious traffic. The second model was trained on a combination of benign and malicious traffic, so the linear classifier could find a threshold value that separates the two flow traffic types. For the convolutional layers, the kernel size was set to 5 for all three layers, the first layer had a stride size of 2, while the second and third layer had a stride size of 1, leading to a latent layer size of 30 nodes. The settings for LBD-preset 1 can be seen in full at table \ref{tab:lbd-s1}. Since the LBD-VAE trains two models separately from each other, there will be two different iteration counters, steps 1 and steps 2. When showing the results, some of the graphs have been cropped to only show what is relevant. I.e.\ if presenting the LBD-VAE accuracy, which does not improve until model 2 starts training, the graph is cropped to only show that part.

When the training was stopped for the first model, at 20,000 steps, the R-Loss mean value had become about 16 for benign data, as seen in figure \ref{fig:1a}. For the second model, training stopped at 30,000 steps, and the R-Loss mean value ranged from 30-40, as seen in figure \ref{fig:1b}. These results acknowledges that benign traffic flows have lower R-Loss when compared to malicious traffic, since the benign data was the same for both training sessions, but the second model had malicious data as well. The overall accuracy scores showed poor performance, achieving an average accuracy of about 63\%. Notice the development seen in figure \ref{fig:1c}, which is a validation set containing only benign flows, and figure \ref{fig:1d}, which is a validation set containing exclusively malicious flows. The two graphs grow in inverse directions of each other. When the benign accuracy increases, the malicious accuracy decreases by almost as much. This is a sign of the benign and malicious probability distribution functions being too similar, so that the Loss Based Detector is unable to classify them properly.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard2/46_tr1_rloss.csv}{Value}{scale=0.6}
        \caption{Model 1 training R-Loss}
        \label{fig:1a}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard2/46_tr2(1)_rloss.csv}{Value}{scale=0.6}
        \caption{Model 2 training R-Loss}
        \label{fig:1b}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard2/46_va_benign_acc.csv}{Value}{scale=0.6}
        \caption{Benign validation accuracy}
        \label{fig:1c}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard2/46_va_malicious_acc.csv}{Value}{scale=0.6}
        \caption{Malicious validation accuracy}
        \label{fig:1d}
    \end{subfigure}
    \caption[LBD-preset 1 Training Run]{Results from the LBD-preset 1 training run.}
    \label{fig:lbd-1}
\end{figure}

After running another session, this time on LBD-preset 2 \ref{tab:lbd-s2}, with a kernel size of 5 and stride size of 1 for all layers, the results showed the same pattern as when running on LBD-preset 1, with no improvements. The KL-Loss multiplier was set to 4, increasing its impact, and using the reduced amount of input features after applying LIME, from table \ref{tab:lime_top}. This could mean that the KL-Loss should have less significance, or that the VAE is unable to separate the flow traffic classes properly.

A run done with LBD-preset 3 \ref{tab:lbd-s3}, as shown in figure \ref{fig:lbd-2}, was done with a KL-Loss multiplier of $1 \cdot 10^{-6}$, as well as using the reduced input feature set \ref{tab:lime_top}. For this training run, we also reduced the amount of training steps for model 1, the model that trains on benign data, to 1,500. This will prevent the model from converging on a R-Loss value. From figure \ref{fig:2a}, the LBD-VAE converged on an accuracy score of about 64\%, but there was a positive spike early on in the training of model 2. Looking at figure \ref{fig:2b}, the validation accuracy on benign data, and figure \ref{fig:2c}, the validation accuracy on malicious data, we see that at around total step 8,000, the benign accuracy was at a mean value above 70\%, and the malicious accuracy was at a mean value above 88\%. These accuracies are still far from good, but it is a sign that the VAE is able to separate the traffic flows well enough for the LBD to classify them, given the right tuning settings.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard2/44_tr_acc.csv}{Accuracy}{scale=0.6}
        \caption{Model 2 training accuracy}
        \label{fig:2a}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard2/44_va_benign_acc.csv}{Accuracy}{scale=0.6}
        \caption{Benign validation accuracy}
        \label{fig:2b}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard2/44_va_malicious_acc.csv}{Accuracy}{scale=0.6}
        \caption{Malicious validation accuracy}
        \label{fig:2c}
    \end{subfigure}
    \caption[LBD-preset 3 Training Run]{Results from the LBD-preset 3 training run.}
    \label{fig:lbd-2}
\end{figure}

The results from using the LBD-VAE on LBD-preset 4 \ref{tab:lbd-s4}, can be seen in figure \ref{fig:lbd-3}. The kernel size of all three convolutional layers were set to 7 and the first two layers had a stride size of 2, leading to a latent layer size of 4, and a theoretical receptive field size of 43. Since there were so few nodes in the latent layer, model 1 required a longer training run compared to the previous runs, hence the number of steps were set to 100,000. As with the previous runs, the VAE still had trouble separating benign from malicious traffic flows. The overall accuracy was slightly better, but still more tuning is required if the LBD-VAE is to be used as a part of a mitigation system. As seen in figure \ref{fig:3a}, the benign accuracy was prioritized when using the current settings, although at the cost of a lower malicious accuracy, as seen in figure \ref{fig:3b}.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard2/50_va_benign_acc.csv}{Accuracy}{scale=0.6}
        \caption{Benign validation accuracy}
        \label{fig:3a}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.4\textwidth}
        \centering
        \tfFromcsv{img/tensorboard2/50_va_malicious_acc.csv}{Accuracy}{scale=0.6}
        \caption{Malicious validation accuracy}
        \label{fig:3b}
    \end{subfigure}
    \caption[LBD-preset 4 Training Run]{Results from the LBD-preset 4 training run.}
    \label{fig:lbd-3}
\end{figure}

\section{Comparison of Results}
\label{analysis-comparison}

At the currently best settings, using preset 4b \ref{tab:p4b}, the LLC-VAE achieved a benign accuracy of 99.59\% and a malicious accuracy of 99.98\% on the validation set\footnote{We use validation set here for comparison between the LLC-VAE and the LBD-VAE, since we did not do any test runs using the LBD-VAE because of poor training performance.}, as seen in figure \ref{fig:llc-validation}. This means that based on the validation set, 4 out of every 1,000 legitimate flows, and the corresponding source IP addresses, would be blocked. At the same time, only 2 out of every 10,000 malicious flows would be let through the LLC-VAE. The LBD-VAE prioritized benign accuracy, which is better than prioritizing malicious accuracy. More on this will be discussed in \cref{discussion-partial}. However, the overall accuracy, as seen in \ref{fig:lbd-validation}, was much lower compared to the accuracy of the LLC-VAE.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[scale=0.4]{img/cm/p4_va_kl_26.pdf}
        \caption{LLC-VAE validation accuracy.}
        \label{fig:llc-validation}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[scale=0.4]{img/cm/s2_run3_va_50.pdf}
        \caption{LBD-VAE validation accuracy.}
        \label{fig:lbd-validation}
    \end{subfigure}
    \caption[LLC-VAE and LBD-VAE Validation Accuracy Comparison]{Validation accuracy comparison.}
    \label{fig:analysis-llc-lbd-validation}
\end{figure}

Compared with the simple convolutional neural network, the LLC-VAE performed better overall on the test set. The best test results for the LLC-VAE was on preset 4b \ref{tab:p4b}, as can be seen in figure \ref{fig:llc-test}. The best test results for the simple convolutional network was on preset 6a \ref{tab:p6a}, as can be seen in figure \ref{fig:cnn-test}. The LLC-VAE had less than 1\% worse benign accuracy, but substantially increased malicious accuracy, at about 7.5\% higher. For both models the validation accuracy was significantly higher, but ultimately, the test accuracy gives a better understanding of how the models would perform in general, since the test set comes from a different computer network. Hence, there are fewer similarities that could cause overfitting, as the datasets are internally correlated to a large degree.

Using the LLC-VAE as a part of a mitigation system is within reason, even though 3 in every 100 benign flows would be blocked. Although, relying solely on the detection capabilities of the LLC-VAE would not be a good solution. Instead, it should be incorporated as a part of a larger mitigation system.

\begin{figure}[htbp]
    \centering
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[scale=0.4]{img/cm/p4_te_kl_26.pdf}
        \caption{LLC-VAE test accuracy.}
        \label{fig:llc-test}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.4\textwidth}
        \includegraphics[scale=0.4]{img/cm/p6_te_modified_17.pdf}
        \caption{CNN test accuracy.}
        \label{fig:cnn-test}
    \end{subfigure}
    \caption[LLC-VAE and Simple CNN Test Accuracy Comparison]{Test accuracy comparison.}
    \label{fig:analysis-llc-cnn-test}
\end{figure}

\subsection{Flow Processing Time}

After fully training the LLC-VAE on the best preset, preset 4b \ref{tab:p4b}, we measured the speed of the model. The LLC-VAE was estimated to be able to process one batch in about 10.8 ms $\pm$ 0.3 ms, where one batch contains 1,024 flows. This is between 90 - 95 batches per second, which translates to about 92,000 - 97,000 traffic flows per second. These measurements are only from the LLC-VAE, and does not include time taken for data transformations. Furthermore, the model has not been optimized for speed either. If this approach were to be added as a part of a full mitigation system, the overall flow processing time would be expected to increase, so these measurements only give an indication of what to expect from the LLC-VAE.




\end{document}


==> parts/background.tex <==
\begin{document}

\chapter{Background}
\label{background}

DDoS and DoS attacks come in many shapes and forms. Both DDoS and DoS are very similar in intent, and can be similar in execution. The goal for both types of attacks is to cause a denial of service for their victim. Successful attacks can last for extended periods of time, potentially causing large amounts of damage to a victim, both financially and in regards to working hours wasted. Multiple proposed solutions already exist, both on a theoretical and production level. Some solutions are based on stateless network traffic, and others are based on stateful network traffic. In more recent times, more and more detection and mitigation systems have been proposed using machine learning. With the potential for detecting and categorizing different types of data at a much higher precision than humans in some cases, and its success in other problem domains, machine learning could very well prove to be effective at combating malicious computer network traffic as well.

In order to understand how we can use the two proposed approaches, the LLC-VAE and the LBD-VAE, to classify and potentially mitigate network intrusion in the form of DDoS and DoS attacks, it is important to understand the nature of the attacks. In this chapter, we will attempt to give the reader an extensive understanding of the problem domain. We will explore where DDoS and DoS attacks typically occur, what the aim of different attacks are, how they try to achieve their goal, and to what degree the different types of attacks have been popular in recent years. There exists a multitude of different attack vectors, including but not limited to, application layer attacks such as HTTP GET and POST\footnote{Hyper Text Transfer Protocol. Application level protocol for data communication.} flooding, or network layer attacks such as ICMP\footnote{Internet Control Message Protocol, a network layer protocol to send messages between network devices.} amplification. Several types of machine learning techniques have the potential to be used for the task of mitigating DDoS and DoS attacks. This chapter will be used to highlight relevant techniques, specifically in the domain of deep learning, before going into detail about Variational Autoencoders.

\section{Network Intrusion and Exploited Vulnerabilities}

In networking, there exists multiple different types of attacks. There are attacks that spy on a network such as a "man-in-the-middle attack", that is able to read and control traffic between two parties. "Eavesdropping", where a third-party is able to read or listen in on communication between two devices. "Password-based attacks", where an attacker tries to retrieve passwords, or brute-force them to gain access to certain parts of a server or website. These are just some examples of network intrusions. The focus of this thesis will be on DDoS and DoS attacks. The idea behind DDoS and DoS attacks is to deny one or more services provided by a website or server to other users. Services such as video browsing, login or any other form of service a website or server might offer. Part of what makes DDoS and DoS mitigation a difficult problem is how hard it is to differentiate between normal traffic, and malicious traffic. After all, a network does not see the difference between a thousand normal users trying to connect to the site, and a thousand bots trying to connect. All the network sees is the information for each individual package, not the intent of whoever is sending the packages. In the following sections we will detail how different types of DDoS and DoS attacks operate and what their typical goal is. After that we will look at how we can detect and classify them.

\subsection{Brute Force Attacks}

Brute force attacks, also called flooding attacks, is a type of DDoS attack that attempts to spend all the bandwidth of the networking system they are focusing on. Whenever a network connection is established and data is transferred between two systems, a certain amount of bandwidth is spent from the hosting server to accommodate for the incoming connection. How much bandwidth is available varies for each server, and the attack sizes vary accordingly. The goal of a brute force attack is to establish an overwhelming amount of connections, making the hosting server unable to handle all the network traffic. The bandwidth can be exploited through UDP, ICMP, TCP or DNS\footnote{Transmission Control Protocol (TCP), User Datagram Protocol (UDP), are transport layer protocols. Domain Name System (DNS) is an application layer naming system.}\cite{Asosheh-and-Ramezani-2008}, and also HTTP, which are legitimate services to anyone with access to the server. This is part of the reason why brute force attacks can be so hard to prevent. In the taxonomy of Mirkovic and Reiher\cite{Mirkovic-and-Reiher-2004}, certain types of brute force attacks are categorized as "non-filterable", meaning that you cannot differ them from normal traffic. An example of this is DNS request flooding\footnote{The content of a legitimate DNS request packet and a malicious one are indistinguishable. They only differ by the intent of the sender.}.

\subsection{Amplification Attacks}

An amplification attack is another form of bandwidth depletion, like flooding. The major difference lies in how the attacker occupies the bandwidth. A brute force attack sends traffic directly to the victim server, while an amplification attack relies on secondary sources. This kind of attack falls under the category of reflection based attacks. The main advantage of using this technique is that it does not require as many machines as a brute force based attack. To deplete the bandwidth of their victim, an amplification attack will broadcast messages and send a spoofed return address which is set to be the victim’s IP address. This will bring each system in the subnet which received the broadcast to initiate replies to the given IP address, thus causing an amplified amount of reply packets being sent to the victim, effectively clogging their network.

From the taxonomy of Specht and Lee\cite{Specht-and-Lee-2003}, we are given two common examples of amplification attacks, "Smurf" and "Fraggle". We will only explain the first one as they are both similar. A Smurf attack works by sending an ICMP ECHO\footnote{An ICMP ping. A short message sent to a network device to check reachability.} request to all hosts within the broadcast address range with a spoofed IP address. Each host will then individually send an ICMP ECHO REPLY packet to the targeted IP address. One such reply does not require much bandwidth, but due to the nature of amplification attacks, it is a trivial issue to generate an attack on a large enough scale to disrupt the victim server.

\subsection{Resource Depletion}

Attacks that aims for bandwidth depletion often tries to overwhelm the victim with packets and requests to disrupt a service. Some attacks however, will focus on exploiting design deficiencies or software bugs on the targeted server. These types of attacks are called resource depletion attacks, or resource exhaustion attacks. The end goal is much the same as with bandwidth depletion but varies slightly in methods used.

A protocol exploit attack is a form of resource depletion that aims to deplete the resources of a victim server by abusing faults in common network protocols through brute force. One such exploit is a TCP SYN attack that abuses the three-way handshake\footnote{In a three-way handshake, a SYN message is sent from the connecting system to the server, which is then answered by a SYN-ACK, and finally this is responded to with an ACK from the connecting system back to the server.} used to initiate a connection between two systems. The exploit focus is on bombarding the server with SYN messages and typically spoofing the return address so that the server sends a number of SYN-ACK messages and waits for the final ACK, which is never received. There is a timeout on a three-way handshake, so this exploit must send a lot of SYN messages within this time window. The effect of this attack is that the server’s processor and memory resources are spent trying to establish connections with fake IP addresses.

Malformed packets is another form of attack which aim is to deplete the resources of their victim. When a connection has been established between two systems, and packages can be transferred between them, the receiver needs to process the packages sent, usually from multiple clients at the same time. A package can be changed, or malformed, to make the victim server waste resources attempting to parse it. An example of an attack using malformed packets is IP fragmentation. It is a type of attack that aims to abuse the limit for the size of datagrams, controlled by the maximum transmission unit (MTU). E.g.\ an attack sends a packet larger than the MTU limit of 1500 bytes, it then needs to be fragmented and sent separately. When a server receives a packet that needs to be fragmented, but can not be reassembled because it has been malformed to contain faulty or fake data, the server wastes resources. This is because it is attempting to parse multiple message parts before realizing that the message is malformed. Given an overwhelming amount of malformed packets, the server will waste all its resources handling them, causing resource depletion.

\section{Trends and Statistics}

This section will present the different attack vectors of DDoS and DoS attacks and how big of a problem these attacks are today, as well as how the problem is expected to develop over time.

Cisco has an ongoing initiative to track and forecast the impact of visual networking applications. The latest edition of this forecast makes an attempt to predict the global data usage, and the trends of network attacks\cite{Cisco-forecast-2019}. In 2017 the number of network devices was around 18 billion, and this number is predicted to increase to about 28.5 billion by the year 2022. From this we can see that the amount of devices that can be used for and is susceptible to attack is increasing, making the need for good network intrusion detection and mitigation systems increasingly important as time passes. A network device in this context is not restricted to personal computers, but can also be a cellphones, cars, printers, or any other device that are able to connect to other devices through networking protocols. This makes the work of protecting against network intrusions even harder, as the amount of devices that can potentially be used for an attack is already very large, and is predicted to grow substantially\cite{Cisco-forecast-2019}. If someone wants to deploy a DDoS attack by hijacking and clustering other devices in a botnet, they do not need to restrict themselves to hijacking personal computers. On the contrary, other network capable devices such as IoT appliances has historically had a lesser focus on security, making them a prime target and an easy way to increase the size of the botnet.

As discussed earlier, the Cisco initiative reported the largest DDoS attack size to date, at a size of 1.7 Tbps in the first half of 2018. This is almost three times the peak size of 2017 which was at 600 Gbps. These attacks sizes are not a common occurrence, an average attack will not be as large as these sizes. Still it is important to keep in mind when developing a mitigation system the potential attack sizes one might face. In 2017 the average size was 990 Mbps, roughly a 10\% decrease from 2016. In 2018 the size of an average attack increased by 37\%, which were likely related to the exposed Memcached vulnerability. Cisco predicts that DDoS attack occurrences and sizes will increase, and believe that out of the total usage of a country’s Internet traffic, DDoS attacks could represent up to 25\%\cite{Cisco-forecast-2019}. This gives an indication of how large a problem DDoS attacks represent.

In a security report by Kaspersky in 2017\cite{Kaspersky-risk-report-2017}, 19\% of businesses experienced some form of DDoS or DoS attack. Amongst the organizations surveyed, 46\% believed cyber threats will be one of the top three developing risks in the next two years. This includes other forms of cyber crime, as well as DDoS and DoS.

\subsection{Attack Cost}

A DDoS attack against a website or server not only affects their ability to provide services to their users, but in many cases also affects their income and security expenditure. Online stores relies on their ability to provide sale services to their customers, and any downtime will lead to money lost and a tarnished reputation. Websites or servers that provide a paid service will also be greatly affected by downtime, in the form of lost customers and reparation costs. There is also indirect economic effects of downtime in certain organizations such as wasted work hours of employees, and because of dependency on certain network services to be able to fulfill their tasks efficiently.

In a threat evaluation report of DDoS attacks by Kaspersky from 2015\cite{Kaspersky-risk-report-2015}, derived from their survey on global IT security\cite{Kaspersky-risk-report-2015-original}, it was found that 50\% of attacks causes a noticeable disruption of service such as increased web page loading times, while 24\% lead to a complete denial of service. The attack length of DDoS attacks vary greatly, depending on the perpetrator’s motivation for the attack. About one third of attacks lasts less than an hour, one third lasts several hours, and one third lasts a day or more, with some lasting up to several weeks. With this in mind it is easy to picture how great the loss of money could be for websites and service providers, considering their dependency on their services to stay up to earn revenue. According to the threat report, enterprises lost \$417.000 on average as a result of a successful DoS attack in 2015. With these kinds of sums lost due to downtime, it is easy to imagine that there is a market for better defense systems, and to find solutions that are easy to implement, saving companies time and money in setting up a defense system.

\subsection{Computer Network Attackers}

The reasons to launch DDoS or DoS attacks against a website or server varies greatly. It could simply be an amateur experimenting with techniques, or seeking a sense of thrill. At the other end of the scale however, we find more dangerous and more determined hackers that have access to large infrastructures of machines ready to launch attacks, as well as access to large scale financial and resource backing.

Attackers could deploy an attack as a decoy to launch another form of attack, or the attack itself could be used to hold an organization hostage for ransom. Maybe the attackers come from, or are hired by a competing firm which have something to gain from causing a denial of service. Then there are politically motivated attacks. E.g.\ if an article is uploaded to a news page and there are some external parties that have an interest in discrediting or suppressing the article. They might resort to causing a denial of service to prevent others from accessing it, or forcing the website to remove the article.

\subsubsection{Attack Vectors}

As with the background and reasons for launching a DDoS or DoS attack, the methods used can also vary greatly. In Cisco’s annual report on cyber security from 2018\footnote{Previous reports can be seen in 2017\cite{Cisco-report-2017}, and 2016\cite{Cisco-report-2016}}\cite[p.~31]{Cisco-report-2018}, HTTP flood attacks were the most common application layer attack in 2017. Out of the organizations surveyed, 37\% claimed to have been a victim of this kind of DDoS attack. SMTP\footnote{Simple Mail Transfer Protocol.}, DNS and HTTPS attacks were each reported to have affected more than 20\% of the organizations. In total, 64\% had experienced some form of application layer attack that year. About half of the surveyed organizations also reported to have been attacked at the network layer, where TCP SYN attacks were the most common at 35\%, and UDP the second most common at 23\%.

This conceptualization is supported by Kaspersky in a report on DDoS attacks released quarterly\cite{Kaspersky-quarterly-reports-1, Kaspersky-quarterly-reports-2, Kaspersky-quarterly-reports-3, Kaspersky-quarterly-reports-4}. We can compare some of the data from Cisco’s annual report. In Q4 2016 and Q1 2017, the most common attack vectors where TCP SYN, TCP, UDP, HTTP and ICMP respectively, with TCP SYN at a 75\% share in Q4 2016 and down to 48\% in Q1 2017. In Q3 2017 we can see that the most common forms of attack vectors remain the same, with TCP SYN at a 60\% share, and TCP, UDP and HTTP laying at between 10-11\%. Q1 2018 shows much of the same statistics, and Q3 2018 have the same top five attack vectors, with TCP SYN taking up an overwhelming 83\% of the distribution. The data reviewed from Kaspersky and Cisco suggests that the most common attack vectors in the last couple of years have been HTTP/HTTPS, DNS, TCP SYN, TCP and UDP, and that the most common forms of attack is some method of flooding or amplification attack.

Knowing what attack vectors are the most common and what type of attack a mitigation system can expect to see, will help greatly in understanding the performance of the two proposed approaches when applied to the datasets at our disposal. A potential danger with only training the models on the current datasets, is that the approaches might become too specialized, only working against the learned attacks. Further discussion in \cref{discussion-datasets}. It is important to make the proposed approaches easily trainable, or alternatively make them robust to unseen attacks. The LBD-VAE could become a viable solution to this problem, since it will filter traffic based on the model loss functions, more about this approach in \cref{methodology-lbd-vae}.

\subsubsection{Attack Motivation}

The motivations for an attack are not always obvious, as the ultimate goal is not necessarily apparent in the method of attack. It is possible to make deductions based on what was targeted when the attack happened and what it achieved. Take for example an attack in 2014 where attackers targeted websites owned by NATO, after they became involved with the conflict happening at the time in Ukraine\cite{Wueest-2014}. In this case it may be safe to assume that the hackers were politically motivated. Amongst other types of common motivations, there is extortion, diversion, disputes, and collateral damage. Extortion is to use the looming threat of a DDoS or DoS attack to get what you want from the victim. To prove to the victim that the attacker has the capability of such an attack they might demonstrate on a random target, which would then fall under the category of collateral damage. DDoS and DoS attacks motivated by disputes can be similar to politically motivated attacks, or it can be motivated by wanting to remove competition. A DDoS or DoS attack can also be used as a diversion for something more threatening. If an organization is targeted by a large enough DDoS or DoS attack, which they are unable to handle, their network will crash. In the downtime window, the attackers can then launch a secondary attack, such as a virus, which now has a larger chance of going undetected because the system administrators are busy handling the DDoS or DoS attack.

Who exactly initiated an attack can be harder to deduce than the reasons for it, although it is possible to find out the general geographical region the attack originated from. In many cases hackers use spoofed IP addresses, VPNs, several layers of indirection, hacked hardware etc. making it hard to pinpoint where an attack originated. According to the quarterly reports of Kaspersky\cite{Kaspersky-quarterly-reports-1, Kaspersky-quarterly-reports-2, Kaspersky-quarterly-reports-3, Kaspersky-quarterly-reports-4}, the most prevalent countries that initiated DDoS attacks, from Q4 in 2016 to Q3 in 2018, were China, USA, and South Korea. China was reported as the source of attacks from 55\% to 77\% of the time, in terms of number of attacks. From this data alone it is easy to believe that a DDoS attack can be prevented in the majority of cases simply by looking at source countries through their IP address. If a Norwegian website written in Norwegian is experiencing a spike in the number of connections from one of the aforementioned countries, it may be safe to assume that it is a DDoS attack. This data however, must be viewed in correlation with the report on what countries were most often the victim, so as to not get a skewed view of where we can anticipate attacks from. Three notable countries from the same reports show China, USA and South Korea as some of the most targeted countries with roughly the same proportions of being targeted as those of sending attacks. This conceives the idea that a portion of the DDoS attacks might be internal to each individual country. To analyze attack motivations and sources is a difficult challenge, and statistical data should be considered, but not depended on fully.

\section{Classifying DDoS and DoS Attacks}

In this section we will look at how network packets are processed, and how they can be transformed and handled to suit our purposes. Then we will explore different machine learning techniques, how they work and for what purposes they are typically used. Then the paper will move on to autoencoders, one of the main algorithms used in this thesis, how they work, and why a Variational Autoencoder might be a well suited deep learning technique for mitigating DDoS and DoS attacks.

\subsection{Stateless and Stateful Packet Processing}
\label{background-packet-state}

There are two ways of processing packets going through a network. One is stateful or flow-based, the other is stateless or per packet-based. The terms stateful and stateless packet processing is typically used for describing two types of firewall filtering methods, but can also be used to describe the concept itself. We will talk about the concept, and also give examples of how they work using firewalls.

\subsubsection{Stateless}
Stateless packet processing or filtering, is when a packet is handled in isolation of other packets. Network traffic is by default processed in this manner, and on the most basic level, will simply be forwarded through the network by the network routers and switches. A packet moving through the network contains information such as source and destination IP, source and destination port, payload, payload length, and traffic type, specifically TCP or UDP. A firewall that utilizes stateless packet filtering will block or allow packets based on the static information available, or using deep packet inspection (DPI)\cite{Alaidaros-et-al-2011}. Keeping track of what connections are allowed or denied entry is called whitelisting and blacklisting respectively. When a stateless firewall sees an incoming packet, and the firewall has been programmed to block all incoming connections trying to reach port 80, that packet will be dropped if the destination port is set to 80. This kind of packet processing is both quick in execution, and easy to implement. As such, it scales well, because there is less overhead and minimal pre-processing required before allowing or dropping a packet. Stateless filtering can handle large amounts of traffic without much issue, because of the simple way it handles packets. However, if using a stateless firewall, there is still a limitation to scaling, because of sequential nature of firewalls. There are multiple solutions to fixing this particular problem, e.g.\ as a tree-rule setup. An example can be seen in the paper by Al-Shaer and Hamed\cite{Al-Shaer-and-Hamed-2003}. There they proposed a rule based tree rather than a list, to speed up lookup time and reduce rule conflicts and anomalies.

\subsubsection{Stateful}
Stateful packet processing or filtering, is when all packets moving through a network are analyzed and grouped in different flows based on previous knowledge. This is done through the creation of sessions\cite[p.~55]{Noonan-and-Dubrawsky-2006}. Whenever a packet is moving through the stateful filtering mechanism, for example a stateful firewall, the firewall will try to match it with already existing sessions based on information such as source and destination address, source and destination port, and protocol. The first packet in a flow will be used for the creation of the session. Information about a session is typically stored only for a given period of time. If no packets have moved over the connection for a time, then the session will be timed out. It is possible to store each session indefinitely, and this would give a much more detailed picture of each connection, but would be impractical on a larger scale because of limitations to system resources. The benefit of using stateful packet processing and creating sessions based on flows of packets between connections, is the meta information that could be gathered. When looking at packets in isolation, it is in many cases impossible to differentiate between normal and malicious traffic, because malicious traffic typically tries to masquerade as normal traffic. With the meta information gained from stateful packet processing, we are able to look at previous packets from the same source and with the same destination. Using that information, it is possible to analyze useful information such as flow duration, average packet size, packet count of packets transferred in a given time window, and so on. In other words, the use of flows allows analysis of the context in which the packets are transferred.

\subsection{Machine learning}

"A computer program is said to learn from experience E with respect to some class of tasks T and performance measure P, if its performance at tasks in T, as measured by P, improves with experience E." This is how Tom Mitchell in his book about machine learning from 1997, defined the concept of machine learning\cite[p.~2]{Mitchell-1997}. It has been used since as an informal definition. At the most basic level, machine learning is just that, an iterative program that can improve, learn, and generalize from experience. There are three major approaches within the world of machine learning, used to describe the different categories machine learning algorithms fall into: These are supervised, unsupervised, and reinforcement learning. These three categories each learn from experience E, and each of them will be presented here, as well as some of their use-cases.

\subsubsection{Supervised Learning}
Supervised machine learning is when the learning experience of an algorithm is allowed to improve itself on predetermined, desired data, already labeled with their desired output, also called target values. As training of a new model begins, it will perform predictions on what it thinks is the correct output, which is usually a random guess, since the model has yet to learn the posterior. The labels are used as a ground truth for comparing the validity of these predictions, and if the guess is wrong, the model can adjust itself. This process is repeated using a quantity of different, labeled data, until the model's predictions are mostly right. In general it is desired to have large amounts of data one can train a machine learning model on, so as to have it learn from a variety of examples, hopefully spanning a large part of the expected real world input. After a model has been trained, it is common to perform an evaluation on an unseen dataset, often referred to as the test set. The model will not be allowed to learn from this dataset. Instead it will be used to extract performance statistics to allow the developers to analyze how well it was trained and designed. If a model is allowed to train for too long on a too narrow dataset, it is in danger of learning qualities explicit to the training dataset. We want a machine learning model to generalize because it needs to perform well on real world input. The training performance in itself is secondary, as it is only a stepping stone to achieve good real world performance. One of the major drawbacks of supervised learning is the need for labeled data. Because a machine learning model requires extensive amounts of data, we also need equally large amounts of labels. The labels must often be manually annotated for each data point in a dataset. An image dataset with millions of images of animals that needs to be labeled by people, is an enormous and expensive task. Unlabeled data sometimes provide degraded performance in terms of classification, but labeled data is both more expensive and harder to acquire\cite{Chapelle-et-al-2010}.

\subsubsection{Unsupervised Learning}

Unsupervised machine learning is similar to supervised, in that they both attempt to predict an output, given an input. The major difference being that when a supervised learning model is told when something is wrong or correct, unsupervised learning is not told, as there are no labels. Because of this, an unsupervised model is forced to group outputs by similar qualities, and not by what it is told to group them by. In other words, supervised learning aims to learn the probability of output $y$ from input $x$, by estimating $p(y | x)$\footnote{This syntax comes from statistics. $p$ stands for "probability", and $p (h | x)$ can be read as "The probability of $h$ given $x$".}, while unsupervised learning aims learn the probability distribution $p(x)$ where $x$ represents several examples of random vectors.

\subsubsection{Reinforcement Learning}
\label{background-reinforcement}

Reinforcement learning is more about learning to interact in an environment. Similarly to unsupervised learning, there is a sequence of desired outputs, but nothing telling the model what is correct. Instead, a reinforcement model has a feedback loop between the learning system and its experiences. The model is set to discover new solutions and actions within the environment, which is called exploration. A developer can use both rewards and punishments to adjust the model behavior, so as to have the model perform preferred actions, as well as discredit bad ones. When a model performs actions based on immediate rewards and punishments, it is called exploitation. Making a good reinforcement learning model requires constant balancing of exploitation and exploration, lest we end up with a model that gets stuck in a local optima, or a model that never finds a solution, respectively\footnote{Balancing exploitation and exploration is generally important for machine learning algorithms, including supervised and unsupervised models, not just for reinforcement learning.}.

\subsubsection{Deep Learning}

Deep learning, short for deep structured learning, is a subfield of machine learning. An artificial neural network (ANN), as can be seen in figure \ref{fig:background-ann}, is a visualization of the neural network (NN) framework. A normal NN can be called shallow\footnote{Shallow is not a formal definition, and it can be used differently, but in general it is a term used to describe neural networks with one or relatively few hidden layers.}. The simplest form of a NN has an input layer used to feed data into the network. The intermediate layer, also called the hidden layer, is a grouping of the input features from the input layer into a new combination of features. Finally we have the output layer that gives a classification or category of where to place the given input. The difference between deep learning and normal machine learning in this context, is that a deep learning algorithm uses multiple hidden layers for the model instead of only one like a simple neural network. Deep learning can be used for supervised, unsupervised, and reinforcement learning, and while there is some overlap between these three categories, supervised is generally for classification, unsupervised for clustering, and reinforcement for learning from an environment.

Neural networks learn by being fed data through the input layer and adjusting the values of the network. In the case of a feedforward NN, input data propagates through the network from beginning to end. An activation function\footnote{Activation functions are nonlinear in nature. They make a NN able to express nonlinearities in the input data.} is applied to the outputs of each hidden layer, which is used as inputs to the following hidden layer. After the data has moved through the network, a backpropagation algorithm is used to update the values of the nodes and connecting weights based on the output of an iteration. Backpropagation follows a gradient descent approach, which is an optimization algorithm used to find the minimum of a function. Backpropagation is iterative and recursive.

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.7]{img/figures/ANN.pdf}
    \caption[Artificial Neural Network]{Fully connected feedforward artificial neural network. Squares represents input and output features, circles represent hidden layer feature nodes, and the lines between the nodes represent weights.}
    \label{fig:background-ann}
\end{figure}

Many classification problems can be solved by shallow machine learning algorithms, and are often faster than deep learning algorithms, as well as being just as accurate. When classifying problems with a linear or low dimensional solution space, e.g.\ the difference between the colors black and white, shallow neural networks could be a better fit. Deep learning is however better at learning complex abstractions of features from simpler abstractions\cite[p.~163]{Goodfellow-et-al-2016}. A problem with shallow neural networks is their inability to extract and make sense of data that have many similar features to other types of data. Each hidden layer in a neural network adds a level of complexity to the features from the input layer. If there is only one layer, as in the case of shallow neural networks, the model might not be able to understand less obvious differences in the data.

Take for example an image of a cat, a shallow neural network might not be able to recognize the same cat if the image was taken from a different angle, or if the first was taken during day, and the second during night, darkening the pixels values. A deep neural network does not simply look at the input data as is, but iteratively abstracts features into higher level representations, learning multiple representations. Given how similar DDoS and DoS attacks can be to normal computer network flows, and the many shapes and forms the attacks can take, we will attempt to solve this particular problem using the framework of a deep neural network.

\subsection{Autoencoders}
\label{background-autoencoders}

An autoencoder is a deep learning framework that utilize an NN framework to perform a variety of different tasks, primarily for unsupervised learning, where the backpropagation target values are set to be equal to the input. Variations of an autoencoder allows for classification, anomaly detection, and generative tasks, amongst other uses. Autoencoders are feedforward networks, meaning that the representative ANN is a directed acyclic graph, and that they use back-propagation for training. The composition of an autoencoder always has at least two parts, an encoder and a decoder. The encoder encodes the input $x$ to a hidden layer $h$, selecting which dimensions to learn from with the function $h = f(x)$. The decoder tries to make a reconstruction, $r$, of the input from the hidden layer, with the function $r = g(h)$. The concept of autoencoders have been around for over a decade, with one example dating back to 1988 by Bourland and Kamp\cite{Bourlard-and-Kamp-1988}. Historically the hidden layer mapping has been deterministic, but more modern solutions use stochastic mapping, with the functions $p_{encoder}(h | x)$ and $p_{decoder}(x | h)$\cite[p.~499]{Goodfellow-et-al-2016}.

The reconstruction of the hidden layer is not a perfect replication, nor should it be, and is recipient to noise. For an autoencoder model to be useful, it needs to generalize over training data, lest we end up with a model that performs poorly on foreign data, as we will see later in \cref{analysis}, \nameref{analysis}. One of the major pros to using this kind of model is its capability to determine which parts of the input are important, by forcing it to learn the useful properties of the data it is given during training. In a way, when using an autoencoder we are often more interested in the encodings of the data and the latent layer representations, than we are of the actual reconstruction of the decoder. A good autoencoder is one that is able to properly select which dimensions from the input to use in the hidden layer and to what degree. In such a way that the decoder is able to produce a good approximation on as few dimensions as possible. There are mainly two methods for dimension selection used in autoencoders, dimensionality reduction and regularization. Dimensionality reductions is when each hidden layer in the model contains fewer nodes than the preceding layer. This forces the model to select the most important features from the previous layer, and throw away the least important ones. Regularization selects the nodes with the greatest positive impact on the model's result, and lessens the impact of the other nodes. There are multiple, different regularization techniques, and some of them will be discussed in the following sections.

The imperfect reconstruction of the input data can be both an advantage and a disadvantage in machine learning. Autoencoders, like other machine learning algorithms, must be applied to problems they are fit to solve. Reconstructing the input is only possible if the model has seen similar data during training. If an autoencoder is only given images of cats during training, it will not be able recognize images of e.g.\ birds. For this thesis, it means that the model will not be able to classify a DDoS or DoS attack if we only train it on normal data. However, because of this exact property, an autoencoder could be used as an anomaly detector, essentially differing the two classes by only recognizing normal data, and unable to recognize anomalies.

\begin{algorithm}[htbp]
\SetAlgoLined
    \For {each input $x$}{
        Feedforward $x$ and compute activations for each layer\;
        Sample the hidden layer $z$\;
        Obtain output $y$\;
        Measure deviation of $y$ from $x$\;
        Backpropagate to update weights and node values\;
    }
    \caption{A simple autoencoder}
\end{algorithm}

\subsubsection{Sparse Autoencoder}
\label{sparse-autoencoder}
A sparse autoencoder (SAE) is a regularized variation of an autoencoder with potentially more nodes in the hidden layer than in the input layer. This means that to extract useful features to learn from at the input layer, the SAE appends a regularizing function to the normal loss function of an autoencoder\cite{ng-et-al-2011}\cite[p.~502]{Goodfellow-et-al-2016}. Because of this, the hidden layer only has a few select nodes active at a time, forcing the SAE to learn the most useful properties of the input. Furthermore, each type of input activates different nodes in the hidden layer. There is normally overlap between properties of for example network packets, hence they would often activate some of the same nodes, but the point of a SAE is to only activate the relevant nodes in the hidden layer, customized for those types of input. This is called the sparsity constraint. In theory, this means that the total amount of active nodes in the hidden layer could be as large as the different properties of the input, leading to some SAEs to have larger hidden layers than input.

The loss function of an autoencoder can be described as $L( x, g( f(x) ) )$, where $f$ is an encoder and $g$ is a decoder. The goal is to minimize the difference between the input and the output. This is done by penalizing $g( f(x) )$ for being dissimilar from the input x. A sparse autoencoder adds a sparsity penalty to the loss function, which is commonly done in one of two ways. One way is to use L1 regularization, also called Lasso Regression\footnote{From statistics. Lasso Regression shrinks the coefficient of less important features, reducing their impact.}, which ends up looking like this, $L( x, g( f(x) ) ) + \Omega( f(x) )$ where $\Omega( f(x) )$ is the regularization term. Note that regularized networks typically regularize the weights that connects the nodes. SAEs however, apply regularization on the activations of the nodes. The term $\Omega( f(x) )$ where $f(x)$ is the hidden layer $h$, can be simplified as $$\Omega(h) = \lambda \displaystyle\sum_{i} |h_i|$$

Here $\lambda$ is a hyperparameter, and the following formula is the absolute sum of all activations of the nodes $i$ in the hidden layer.

Another way to apply a sparsity penalty is by using Kullback-Leibler divergence, or KL-Divergence for short. KL-divergence is a measure of the divergence between two probability distributions, used to measure their similarities, or dissimilarities. Given the probability distributions $p$ and $q$, KL-divergence is a measure of how well $q$ approximates $p$, by calculating the cross-entropy $H(p, q)$ minus the entropy $H(p)$, to get the KL-term $D_{KL}(p || q) = H(p, q) - H(p)$. The KL-divergence is a central part of the Variational Autoencoder, which will be explained in detail in \cref{background-vae}. Niyaz et al. proposed using a stacked sparse autoencoder in order to detect DDoS attacks in software defined networking (SDN)\cite{Niyaz-et-al-2016}. In their paper they use KL-divergence for their sparse autoencoders to put a constraint on the hidden layer to maintain low average activation values. They also present a method for layering the sparse autoencoders to use as a classifier. The sparsity penalty term can be written as $$\beta\displaystyle\sum_{j=1}^{N} KL(p||\hat{p}_{j})$$

Where $\beta$ is a hyperparameter to adjust the sparsity penalty term. $\hat{p}_{j}$ is the average activation value of a hidden node $j$ over all the training inputs, and $p$ is a Bernoulli random variable\footnote{From statistics, a Bernoulli distribution is the discrete probability distribution of a random variable with boolean values.} that represents the ideal value distribution. The KL-loss is at a minimum when $p=\hat{p}_{j}$.

\subsubsection{Denoising Autoencoder}

The principle of a denoising autoencoder (DAE) is simple. As was explained earlier, an autoencoder aims to optimize the loss function by minimizing the difference between the input and the reconstructed output. A DAE is regularized and can be overcomplete, meaning it uses regularization to extract useful features. Differing from a SAE, a DAE does not apply a penalty to the loss function, but instead changes the reconstruction error term. The loss function is changed from the vanilla version $L( x, g( f(x) ) )$ to $L( x, g( f(\tilde{x}) ) )$, trying to optimize on $f(\tilde{x})$ instead of $f(x)$, where $\tilde{x}$ is a corruption of the input. The output is then compared to the uncorrupted input. DAEs differ only in a minor way from vanilla autoencoders. By adding noise to the input data, a DAE is forced to learn the most prominent features to be able to reconstruct the original input, essentially learning to remove the noise.

A DAE is generally used for creating outputs free of noise. If applied to images, it is possible to reconstruct missing parts, for example if there is a lens-flare covering part of the image, the DAE could provide a copy of the image without the flare. A DAE could also be used to restore missing or hard to read letters and words in a text, or unclear sound could be repaired to sound cleaner. Vincent et al.\cite{vincent-et-al-2010} presented a simple stacked DAE and tested it on a variety of different datasets, including the MNIST image dataset\cite{MNIST}. What they showed us is that by using a denoising criterion, we can learn useful higher level representations of the input data. In the paper by Vincent et al.\cite{vincent-et-al-2010}, the input is corrupted with simple generic corruption processes, and they mainly perform tests on image and audio samples. A denoising criterion could be useful to help the learning process of an autoencoder, to perform DDoS and DoS classification based on the output loss function.

\subsection{Variational Autoencoder}
\label{background-vae}

The Variational autoencoder (VAE) introduced by Kingma and Welling\cite{Kingma-and-Welling-2013} is a generative model and use the same encoding as a normal autoencoder, the difference being in how the latent variables are handled. It is based on variational Bayes\footnote{Bayes is here referring to Bayesian inference. Variational Bayes methods are used for approximating intractable integrals arising from Bayesian inference.} which is an analytical approximation to the intractable posterior distribution of the latent variables. It is used to derive a lower bound for the marginal likelihood of the observed data. The VAE present a change to variational Bayes, by reparameterization of the variational lower bound, which is called the Stochastic Gradient Variational Bayes (SGVB) estimator. Since the VAE is a generative model, its primary strength lies with how well it can create new outputs based on learned features from training. It is in addition to this also possible to extend on a VAE to use it for data classification. An example of this can be seen in the VAE of Y. Pu et. al.\cite{Pu-et-al-2016} using convolutional layers of the encoder and decoder to perform semi-supervised learning on image datasets.

The main difference between a traditional autoencoder and a VAE is how they use the layer between the encoder and the decoder, commonly referred to as the latent layer. An autoencoder use the latent variables directly and decode them to use for comparison between the input and output. A VAE will instead encode into two vectors of size $n$, the vector of means $\mu$, and the vector standard deviations $\sigma$. A sampled vector is created from a collection of elements $z_{i}$ that is assumed to follow a Gaussian distribution\footnote{A Gaussian distribution, also called a normal distribution, is a function that represents the distribution of a group of random variables as a symmetrical bell-shaped graph with the mean value at the center.}, where each element $i$ comes from the $i$-th element in $\mu$ and $\sigma$. Thus we can write each element in the sampled vector as $z_{i}\sim{\mathcal{N}(\mu_{i}, \sigma_{i}^{2})}$\footnote{From statistics. It reads: "z drawn from a normal distribution with mean $\mu$ and standard deviation $\sigma$"}.

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.45]{img/figures/fcVAE.pdf}
    \caption[Variational Autoencoder With Fully Connected Layers]{A VAE with fully connected layers. Each vertical line of nodes represent one layer. The latent mean and latent variance layers are two separate layers, which the layer z sample from. All nodes in a layer have weights connected to the nodes in the adjacent layer, like seen in the first two encoding layers. (For simplification, only some of the weights are drawn in this figure).}
    \label{fig:background-fcvae}
\end{figure}

\subsubsection{VAE in Detail}
\label{background-vae-detail}

Let $z$ be a latent representation of the unobserved variables, and $g(z)$ a differentiable generator network. $x$ is sampled from a distribution $p(x; g(z))$, which can be written as $p(x|z)$. Here $p(x|z)$ represents a probabilistic decoder presenting a distribution over the possible values of $x$ given $z$. When using the probabilistic decoder, we get an observation $x$ from the hidden variable $z$. However, what we want is to infer the characteristics of $z$, thus we need $p(z|x)$ and the integral marginal likelihood $p(x)$. The problem is that $p(x)$ is intractable, meaning that we cannot evaluate or differentiate the marginal likelihood\footnote{For further details about this problem, see the original paper by Kingma and Welling\cite{Kingma-and-Welling-2013}.}. The solution to this is to create an approximation of the true posterior with another distribution $q(z|x)$, which will be the recognition model, a probabilistic encoder. We can use KL-divergence to measure the difference between these two probability distributions, as discussed earlier in \cref{sparse-autoencoder}. The goal is to minimize the difference in order for the two distributions to be as similar as possible, we then get $\min{KL}(q (z|x) || p (z|x) )$. This can be used to maximize the lower bound $\mathcal{L}(q)$ of the marginal likelihood of the observed data, so that we get $\mathcal{L}(q) = E_{z\sim{q(z|x)}} \: log \: p(x|z) - D_{KL} (q (z|x) ) \, || \, p (z) )$. The first term $E_{z\sim{q(z|x)}} \: log \: p(x|z)$ represents the reconstruction term, and $D_{KL} (q (z|x) ) \, || \, p (z) )$ represents the Kullback-Leibler (KL) term. It ensures that the approximate posterior q is similar to the true posterior p.

\subsubsection{Reparameterization Trick}

We have now seen the basic explanation of how a VAE works, and the math behind it. To fix the problem with the integral marginal likelihood $p(x)$, the "reparameterization trick" is introduced.

Since an autoencoder relies on a NN to forward data and backpropagate for training, we should not have a latent variable $z$ be a random variable sampled from $q(z|x)$. A NN generally has poor performance when performing backpropagation on random variables. This would lead to the decoded output being too different from the input. We know that the probabilistic encoder $q(z|x)$ is Gaussian, because it produces a distribution over the possible values of $z$ from a data point $x$. In other words, $q(z|x) = {\mathcal{N}(\mu, \sigma^{2})}$. Now let $\varepsilon$ be an auxiliary noise variable $\varepsilon \, \sim{\mathcal{N}(0, 1)}$. We can reparameterize the encoder $q(z|x)$, so we get $z = \mu + \sigma \cdot \varepsilon$ as seen on the right hand side of figure \ref{fig:background-repa}.

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.8]{img/figures/reparameterization.pdf}
    \caption[Reparameterization Trick]{Diamond shapes represent deterministic dependencies, and oval shapes represent random variables.}
    \label{fig:background-repa}
\end{figure}

\subsubsection{Motivation}
As we have mentioned earlier, network packets moving between a client and a server can vary greatly in shape and form even though they follow the same protocols. Likewise many network packets can be very similar, with only small differences separating them. The same goes for packets belonging to DDoS and DoS attacks, they can be very similar to other attack packets, and normal packets. One of the things we aim at achieving in this thesis, is to be able to efficiently separate DDoS and DoS attacks from normal traffic. An autoencoder, particularly a VAE, could be a well suited tool for this. It is a challenging problem to separate malicious and normal traffic, sometimes with no more than minute differences separating them, hence we need a tool that is able to find small details and differences, as well as finding features that are important. Standard autoencoders, and other implementations of autoencoders, learn features from input data in a discrete fashion when encoded to the latent layer. A VAE on the other hand encode features as probability distributions with the use of variational inference\cite{Kingma-and-Welling-2013,blei-et-al-2017}, in our case causing similar packets to be encoded and decoded in a similar manner. We sample from this distribution to get the latent attributes.

A common problem with machine learning in general is gathering reliable data to train and test on. What is more, deep learning algorithms require large amounts of data to generalize and train robust and deep features. While a VAE need large amounts of data just like many other deep learning methods, one of its strengths is in its ability to generalize over similar features, and ignore noise. With a VAE, one can create a model capable of learning smooth latent state representations of the input. There are two parts to the learning process of a VAE, the reconstruction loss and the KL-divergence loss. Using purely reconstruction loss causes it to behave like a normal autoencoder, simply reconstructing the input to the output, with potentially large gaps in between different classes. Using purely KL-divergence loss we end up with outputs which all use the same unit Gaussian, causing different classes of data to be grouped and mixed between each other. Other autoencoders which do not rely on variational inference have been used for both DDoS and DoS detection, and will be discussed later in \cref{related-work}, \nameref{related-work}. Because the VAE combines these two loss terms into one, a potential use for it is to group different classes of data with similar features close to each other. This is one of the reasons why a VAE is a generative model, since it can extract and generate new data based on data points with likeness to each other. For detecting and classifying DDoS and DoS, the generative part can be ignored, instead using the VAE to remove noise, and generalizing over similar features in a manner that allows understanding of data not included during training of the model.

Generating new samples using a VAE is straightforward. One simply removes the encoder part after training, leaving $z$ to sample from $\mathcal{N}(0, 1)$\cite{Doersch-2016}. We do not need to generate new data from the learned features of DDoS, DoS and normal data since we are using it for detection and mitigation. However, it should be noted that a general problem with the VAE architecture is that the normal and generated outputs come out blurry, or noisy\cite{Kingma-and-Welling-2013,Doersch-2016}. The model will sometimes ignore less prevalent features of the input, potentially causing this blurriness. This weakness is most obvious when looking at images as outputs. How much this affects datasets consisting of network packets, and how important it is for training and testing is difficult to tell.



\end{document}


==> parts/conclusion.tex <==
\begin{document}

\chapter{Conclusion}
\label{conclusion}

This thesis has presented two different approaches for DDoS and DoS mitigation using deep learning. Both approaches build on the framework of a Variational Autoencoder, using pre-generated datasets to classify different types of computer network traffic. These datasets provide the two approaches with input features from network traffic flows, allowing them to learn to filter normal and malicious traffic.

The first approach, LLC-VAE, is a latent layer classification network that utilizes the latent layer encodings of a Variational Autoencoder. The LLC-VAE showed clear signs of overfitting towards the training dataset in the beginning, but the generalization capabilities has been greatly improved through various tunings. The improved generalization has in large part been achieved by adjusting the KL-Loss weight, manual feature selection, and tuning of the convolutional layers.

The performance of the LLC-VAE has been tested on two different datasets, split into a training set, a validation set, and a test set. The training and validation sets have data that are internally correlated, hence we use the test set to record model results. When we compared the LLC-VAE performance with a simple convolutional network of a similar structure, the LLC-VAE was overall better at generalizing, achieving better results on the test set.  At the core of the VAE is the KL-Loss value, which regulates the latent layers. Lowering the KL-Loss weight improved the overall model performance. When the weight was lowered past a certain point however, the overall performance of the LLC-VAE declined. Acknowledging that using a Variational Autoencoder over a standard autoencoder had a positive impact on the ability of the model to classify normal and malicious traffic flows.

The second approach, LBD-VAE, relies on the VAE to separate normal and malicious traffic flows into two different probability distributions. A Loss Based Detector is applied to the reconstruction loss, classifying traffic flows using a linear classification layer. The VAE is trained exclusively on normal traffic, and the LBD is trained on a combination of normal and malicious traffic. Since the VAE is only trained using normal traffic, the LBD-VAE is theoretically capable of classifying DDoS and DoS attack types not seen during training. This is because malicious flows would not fit into the probability distribution of the normal flows. The results from the training runs using the LBD-VAE showed that it is currently unable to be used as a part of a mitigation system. The VAE had difficulty with separating the two probability distributions, hence the classifier achieved unsatisfactory results. Still, if the LBD-VAE were to be tuned further, it has the potential of becoming a viable method for mitigation.

This thesis has proven that deep learning based techniques can be effective at countering DDoS and DoS attacks. The second approach, LBD-VAE, currently does not perform well enough to be used as a mitigation system, but is theoretically promising. More research should be executed to explore other possibilities. The overall best test results was achieved by the LLC-VAE, being able classify benign and malicious traffic at upwards of 97\% and 93\% accuracy respectively, on simulated data in the generalized case. The LLC-VAE has proven itself capable of competing with traditional mitigation methods, but will need further tuning to ensure even better performance.



\end{document}


==> parts/discussion.tex <==
\begin{document}

\chapter{Discussion}
\label{discussion}

This chapter will discuss strengths and weaknesses of the used datasets, as well as the two proposed approaches, the LLC-VAE and the LBD-VAE. Future work and changes that could be applied to the current approaches to ensure an optimal solution, are discussed towards the end of the chapter.

\section{Proposed Approaches}

This thesis proposed two approaches for creating a detection system that could be used as a part of a mitigation system against DDoS and DoS attacks. The first approach, LLC-VAE, is based on two ideas. First, that an autoencoder framework learns useful representations of the input data at the latent layer. Second, that a VAE  separates different flow types, as well as gathering similar flow types, through the latent layer node probability distributions.The latent layer classificator is made with a single hidden layer, but it is not a linear classifier. By combining the LLC with the VAE, the LLC-VAE backpropagate on the weights and node values of the encoder, in addition to the classification layer, turning it into a non-linear classifier. Moreover, after training the model to completion, it relies completely on the encoder, allowing for the removal of the decoder, ensuring increased traffic flow processing speed.

The best presented validation results, as seen in figure \ref{fig:llc-validation} on preset 4b \ref{tab:p4b} from \cref{analysis}, \nameref{analysis}, shows that the VAE was able to separate the input data to such a degree that the LLC was able to detect benign and malicious data at a high accuracy for both the training and the validation set. The LLC-VAE suffered in performance when the test data was used, as seen in figure \ref{fig:llc-test}, acknowledging that this approach overfits to some extent on the training data when using preset 4b.

When compared with a simple baseline convolutional network, as seen in figure \ref{fig:cnn-test} on preset 6a \ref{tab:p6a}, the LLC-VAE performed better overall. Further tuning of the LLC-VAE could increase the performance.

The main contribution of this thesis is the LLC-VAE, the Loss Based Detection model was meant as an alternative, to explore the ability of the VAE to detect traffic flow anomalies. Similarly to the first approach, the LBD-VAE builds on the idea that a VAE can effectively group similar traffic flow types. The results proved the current implementation of the LBD-VAE to be insufficient in terms of anomaly detection. We do not disprove it as a potential solution, but it will require more work and tuning if it is to perform competitively. This could be a potential avenue for future work. The Loss Based Detector is a linear classifier, that depends heavily on the VAE to create distinct probability distributions for the benign and malicious traffic flows, based on the  reconstruction loss. Because of this, the LBD-VAE relies more on the VAE part than the first approach. Further changes would thus need to be applied to the VAE framework.

\section{Partial Mitigation}
\label{discussion-partial}

DDoS and DoS attacks are not in themselves harmful to a victim server or website. An overwhelming amount can cause harm, but there is no issue with letting some through, as long as the victim can handle the traffic load. E.g.\ if a server can handle 500 Mbps of network traffic, and there is an attack of size 1 Gbps, a mitigation system could allow 50\% of the attack traffic to pass, ignoring normal load on the server. For this reason, a high benign accuracy is more important than the malicious accuracy for the two proposed approaches, if implemented as parts of mitigation systems. Ideally, both benign and malicious accuracy should be as high as possible, but occasionally it is necessary to decrease one in the favor of the other. When tuning either of the proposed approaches, if increasing the malicious accuracy causes the benign accuracy to decline, one should reconsider the tuning. On the other hand, it might be worthwhile to choose tuning settings that favor small increments in benign accuracy, even if the malicious accuracy declines. A benign accuracy of 99\% and a malicious accuracy of 90\% is better than 98\% and 97\% respectively. This is because blocking 1 less legitimate user in every 100 is generally more important than blocking 7 extra illegitimate users in every 100. Balancing the benign and malicious accuracy is a problem that would need due consideration, and might need to be tuned specifically for the server or website that implements a mitigation system using the LLC-VAE. Sometimes it might even be necessary to block a certain amount of legitimate users if it means stopping a larger part of a DDoS or DoS attack. E.g.\ if a victim server barely has enough capacity to handle a few percent of an attack, then it is preferable to block a few legitimate users, rather than having all of them losing access to the server.

\section{Datasets}
\label{discussion-datasets}

A problem for any machine learning algorithm, is the challenge of making a dataset that represents the problem domain in a realistic manner, and at the same time being in a format that is usable by the algorithm. Creating a dataset that needs to contain benign computer network traffic, as well as DDoS and DoS traffic, can be very time consuming, and comes with multiple pitfalls. One of the most difficult problems, is to gather or create traffic data that properly captures a representative dataset, and spans the expected real world data, as well as not making a dataset consisting of artificial correlations. Ideally, the traffic data should be sampled from real world computer network traffic. This becomes increasingly difficult when considering that in many cases, the traffic data needs to be anonymized. As an alternative, it is possible to create a closed environment, so there is no need for anonymization, but then there is a problem of generating a sufficient amount of traffic data, since deep learning algorithms require large amounts of data. If one decides to gather data from real world network traffic, there is also the problem of properly labeling the different traffic types. Labeling data, when there are thousands or millions of samples, is a huge time investment. There is also an element of uncertainty, because it is not always possible to know for certain whether a network traffic packet, or flow, is benign or malicious. Simulating the traffic data overcomes some of these difficulties. There would no longer be a need for anonymization, labeling could be completely automatic, and generating enough traffic data would be trivial. However, the quality is difficult to guarantee, and the data might not be representative of real world traffic.

\subsection{Simulated Datasets}
\label{discussion-simulated}

This thesis utilize two pre-generated datasets, CSECICIDS2018\cite{CSECICIDS2018} and CICIDS2017\cite{CICIDS2017}. They contain benign, and a variety of malicious, computer network traffic flows. Both datasets contain large amounts of data, and most of the feature sets overlap between the two. One is used for training and validation, and one for testing. A drawback in using these datasets, is that the traffic flows are generated from simulated computer network traffic. This is not a problem in regard to the DDoS and DoS attack data, because those are typically computer generated anyway\footnote{Even if real DDoS and DoS attacks are generated, they could be generated in a different manner than in the used datasets.}. In regard to the benign data, simulation could create discrepancies between this data and real world computer network traffic. I.e.\ the proposed approaches could have ended up learning correlations that are not fully applicable to real computer networks. On the flip side, the simulated data could have crippled the performance of the two proposed approaches, by creating benign and malicious data that are too similar.

When the LLC-VAE was applied to the test data, another problem was discovered. Recall back to \cref{experimental-computer-networks}, with the figure of the simulated computer networks \ref{fig:experimental-dataset-network}. Both datasets had very small attack networks and normal networks, with few, unique source and destination IP addresses for each type of DDoS and DoS attack. In some cases, a specific attack type only had one unique source IP address. Intuitively, when making a DDoS and DoS mitigation system with deep learning algorithms, it is logical to have the algorithms learn repeating frequency patterns based on the IP addresses of the network traffic. Especially considering how hard it can be to find other patterns in DDoS and DoS attack traffic, since they are so similar to normal traffic. The problem with this is that it could cause a deep learning model to learn the specific IP addresses, and not the correlation between them and the traffic patterns. This assertion is supported by what was found in \cref{analysis}, \nameref{analysis}, regarding the results from figure \ref{fig:p4-ip-and-noip}. When the LLC-VAE performs better on the test results, it means that it generalizes better, i.e.\ less overfitting. From the analysis, the LLC-VAE performed better on the training and validation set when including the IP addresses, but was worse for the test results. Interestingly, the LLC-VAE performed relatively well on the validation set, even without the use of IP addresses, showing that they are not necessary features for training the model to separate DDoS and DoS attacks from benign traffic.

\subsection{Attack Vectors}

A limitation of the two datasets used for this thesis, is the lack of variation in the attack vectors of the DDoS and DoS attacks. Recall back to \cref{methodology-2018}, all of the attacks from the dataset used for training, except one, used HTTP as the attack vector\footnote{The test set, as explained in \cref{methodology-2017}, also used HTTP as the attack vector for the attacks.}. The only attack class that did not, was the DDoS  LOIC-UDP attack, which had very few traffic flow samples. Exactly how much the lack of variety in the attack vectors affected the two proposed approaches is difficult to tell without further testing on other datasets. It could have caused the LLC-VAE or LBD-VAE to overfit towards the training set. The test set would not have shown any signs of overfitting because of the test set also only had attacks that used HTTP. Even though HTTP is one of the most common attack vectors for DDoS and DoS attacks, the used datasets might have been providing a too limited representation of DDoS and DoS attacks in general.

The LBD-VAE will require some work if it is to be used as a part of a mitigation system. If the malicious accuracy were to be increased by tuning and modifying the model, the LBD-VAE has the potential to mitigate DDoS and DoS attacks that it has never observed during training. The LBD-VAE is initially trained exclusively on benign traffic flows, before training the threshold that separates benign from malicious flows. If the threshold is set correctly, it might not matter that the datasets only have DDoS and DoS attacks that use HTTP as their attack vector. The LBD-VAE would classify attacks as anomalies either way, as long as they do not match the benign traffic signature. That is after all one of the strengths of an autoencoder, the ability to detect anomalies based on obscure data patterns. As a side effect, legitimate connections that does not match the benign traffic signature, could end up being blocked by the LBD-VAE.

\subsection{Validation Set and Test Set}

During the multiple training runs of the two proposed approaches, we used a training set, a validation set, and a test set. All three sets have the same input feature set, as such they can be used for the same model. The deep learning models learn from the training set, and the models are adjusted based on the results from the validation set. This way, overfitting can be prevented, by understanding what model parameters influence the capabilities of the model to generalize and learn. As for the test set, normally one would only use it to assess the performance of a fully specified classifier. For the two proposed approaches however, in \cref{analysis}, \nameref{analysis}, we used the test set to determine what tuning settings were optimal\footnote{Using a test set for tuning is not a preferable approach. This was in part done because of necessity. There are few publicly available datasets containing DDoS and DoS data, and even fewer that are compatible to use with each other.}. From there, we adjusted the models until we found the tuning settings that gave the best test results thus far, see \cref{analysis-comparison}. By doing this, one could argue that the test set is used as a second validation set, and not as an actual test set. In some cases, there was a slight decline in overall accuracy on the validation set, when the tuning settings for the models were changed to improve the test results. It was necessary to do this, however. Without inspecting the test set between tunings, we might not have discovered what input features, and which tuning settings, caused overfitting of the LLC-VAE and the LBD-VAE. In addition, the training set and validation set are internally correlated, which caused the models to learn feature relations specific to those sets. This meant that we could not trust the validation set results alone. That is why using the test set for tuning, in addition to the validation set, was necessary for better understanding of how the models learned. Doing this might have caused overfitting towards the test set, so ideally, other test sets should have been used.



\section{Future Work}

This section will be used to discuss possible future work. Presenting how the two proposed approaches can be improved, and discuss what the best approach is to implement either of them as a part of a complete mitigation system.

\subsection{Implementing a Complete Mitigation System}

In their current state, the two proposed approaches do not explicitly perform mitigation. However, both approaches are able to detect benign and malicious network traffic on a flow level. The step from classifying individual traffic flows, to blocking the flows or the source, is not a big one. The simplest way to mitigate the attack flows, is to block and keep track of the source IP addresses that are associated with the flows that have been classified as malicious. I.e.\ by using a blacklist, alternatively a whitelist, or both. As an improvement, the whitelist or blacklist can be used to keep track of repeating IP addresses. So that the addresses that have been associated with legitimate traffic has a higher chance of being let through. This could potentially improve the overall accuracy of the mitigation system, by adding a second security layer after the LLC-VAE or the LBD-VAE. Although this is outside of the scope of this thesis, as it is not a deep learning problem.

In order to create a complete mitigation system, there needs to be a method for generating flows from network packets. Currently, the two proposed approaches rely on pre-generated datasets. The flow generator would be installed onto a computer network, where it can retrieve packets, transform them to flows, and send the flows to the LLC-VAE or the LBD-VAE. One way to transform the packets to flows, is to keep a table of entries, where each entry represents a communication session that tracks information about the packets sent back and forth between two IP addresses\cite[p.~56]{Noonan-and-Dubrawsky-2006}. See also \cref{background-packet-state}. Adding a pre-processing step like this is not difficult, the problem lies with the added time spent processing the traffic moving in and out of a computer network. Optimizing the time spent on pre-processing network packets is vital to creating an efficient mitigation system. Failing to reduce the pre-processing time sufficiently can lead to the system slowing down incoming and outgoing network traffic, by spending too much time handling the packets. Ideally, the mitigation system would handle packets directly, but the two proposed approaches need traffic flows to function, more about this in \cref{discussion-memory}.

\subsection{Live Training}

To overcome the lack of available DDoS and DoS datasets, and the problems with creating datasets from scratch, it is possible to train the proposed approaches live. That is to say, continuing the training after installing the complete mitigation system on a computer network. The mitigation system could then either be trained continuously, or for a set amount of time.

At the beginning of the training, the mitigation system would not actively filter incoming connections, but first establish a high accuracy by learning from the computer network.

One of the difficulties with live training is that there is no way to know for certain whether the network traffic is of a benign or malicious nature. If the mitigation system were to be pre-trained on datasets, before starting live training, the deep learning models could first learn to recognize traffic types, then adjust itself during live training. Network packets are not labeled, so we would have to assume the nature of the network traffic. Alternatively, we could assume all live traffic to be benign, then simulate DDoS and DoS attacks against the computer network. That way the mitigation system would have some labeled data to learn from\footnote{Important to note, is that if live training the models, there would be much more benign traffic than malicious. This could cause the models to forget the malicious attack patterns, because the weights and node values would be adjusted to fit the benign.}.

Live training is a method to ensure continuous learning for the proposed approaches, but there are some pitfalls we could inadvertently end up falling in. When a deep learning model is set to learn constantly, it might learn from erroneous data. E.g.\ if an attacker has obtained knowledge about the live training, they can condition the mitigation system to let their attack through. This can be done by first transferring legitimate traffic over a period of time, then sending an attack with many of the same patterns. That is to say, attackers could induce erroneous learning in the models\footnote{On the same note, the model weights and node values would need to be kept secret. Lest an attacker train their own machine learning algorithm to generate attack traffic that looks like benign to the mitigation system.}. To overcome this particular problem, the live training could be turned on only at specific time intervals. This will not fix the problem completely, but can diminish it. Also, if we do not want the mitigation system to learn from DDoS and DoS attack traffic, the training could be turned off when it is suspected that an attack is happening.

\subsection{Using Memory Models for Packet Classification}
\label{discussion-memory}

When work started on this thesis, the original plan was to implement a RNN, in the form of a LSTM, in addition to the two proposed approaches. With its memory capabilities, a LSTM could potentially replace the need for a system that store session information to create flows from packets. By directly performing DDoS and DoS mitigation on network packets, the overall time spent processing network traffic with this approach could be greatly reduced. As compared to the two proposed flow based approaches. The LSTM could read information from network packets, and store relevant information relating to the packets transferred between two IP addresses in a connection. Each connection and the information about the packets sent between them, would be stored in individual memory units. One of the major difficulties with using a LSTM for DDoS and DoS mitigation, lies with the issue of keeping relevant feature abstractions in memory. Given a packet that arrives at time step $n$. If there are too many packets in between time step $n$ and $n + k$, the relevant memory unit is likely to have been re-appropriated to store something else. For this thesis, the plan to use a LSTM was ultimately discarded because of time constraints.

As an alternative to utilizing a LSTM for mitigation, it could be implemented as a part of the LLC-VAE or the LBD-VAE. Previously we discussed how the current approaches relies on traffic flows, thus needing a system to create flows from packets. An idea could be to use a LSTM to create flows, or otherwise generate features, that the proposed approaches could use for training and mitigation. Whether this would reduce the pre-processing time, when compared to a simple table storing session information, is difficult to tell without implementing and testing such a system. It could be a potential avenue for future work.

\subsection{Further Feature Selection With LIME}
\label{discussion-selection}

The current results from \cref{analysis}, \nameref{analysis}, showed a significant improvement after manually selecting input features with LIME\cite{Ribeiro-et-al-2016}. This suggests that further research on manual feature selection could lead to even better results. So far, we have only removed the least used input features, or features we suspected to have a negative impact on the training of the models. A possibility is to remove individual features, and train the models on the remaining ones. Doing this would be very time consuming, because the models would need to be trained many times, on a multitude of feature combinations out of the original 76. To reduce the time spent training the models, input features could be removed in groups so there would be fewer possible feature combinations. As an alternative, instead of guessing what input features to remove with LIME, one could also theorize what features might cause overfitting, or reduction of accuracy, in the models. This would be similar to how we theorized, and showed with results, that the IP addresses caused a negative impact on the training of the two proposed approaches. As an added benefit of removing features before model training, it would reduce overall processing time for the complete mitigation system. This is because there would be less features generated by the pre-processing step that turns packets into flows, and the LLC-VAE and the LBD-VAE would train on fewer features.


\chapter{Discussion}
\label{discussion}

This chapter will discuss strengths and weaknesses of the used datasets, as well as the two proposed approaches, the LLC-VAE and the LBD-VAE. Future work and changes that could be applied to the current approaches to ensure an optimal solution, are discussed towards the end of the chapter.

\subsection{Proposed Approaches}

This thesis proposed two approaches for creating a detection system that could be used as a part of a mitigation system against DDoS and DoS attacks. The first approach, LLC-VAE, is based on two ideas. First, that an autoencoder framework learns useful representations of the input data at the latent layer. Second, that a VAE  separates different flow types, as well as gathering similar flow types, through the latent layer node probability distributions.The latent layer classificator is made with a single hidden layer, but it is not a linear classifier. By combining the LLC with the VAE, the LLC-VAE backpropagate on the weights and node values of the encoder, in addition to the classification layer, turning it into a non-linear classifier. Moreover, after training the model to completion, it relies completely on the encoder, allowing for the removal of the decoder, ensuring increased traffic flow processing speed.

The best presented validation results, as seen in figure \ref{fig:llc-validation} on preset 4b \ref{tab:p4b} from \cref{analysis}, \nameref{analysis}, shows that the VAE was able to separate the input data to such a degree that the LLC was able to detect benign and malicious data at a high accuracy for both the training and the validation set. The LLC-VAE suffered in performance when the test data was used, as seen in figure \ref{fig:llc-test}, acknowledging that this approach overfits to some extent on the training data when using preset 4b.

When compared with a simple baseline convolutional network, as seen in figure \ref{fig:cnn-test} on preset 6a \ref{tab:p6a}, the LLC-VAE performed better overall. Further tuning of the LLC-VAE could increase the performance.

The main contribution of this thesis is the LLC-VAE, the Loss Based Detection model was meant as an alternative, to explore the ability of the VAE to detect traffic flow anomalies. Similarly to the first approach, the LBD-VAE builds on the idea that a VAE can effectively group similar traffic flow types. The results proved the current implementation of the LBD-VAE to be insufficient in terms of anomaly detection. We do not disprove it as a potential solution, but it will require more work and tuning if it is to perform competitively. This could be a potential avenue for future work. The Loss Based Detector is a linear classifier, that depends heavily on the VAE to create distinct probability distributions for the benign and malicious traffic flows, based on the  reconstruction loss. Because of this, the LBD-VAE relies more on the VAE part than the first approach. Further changes would thus need to be applied to the VAE framework.

\subsection{Partial Mitigation}
\label{discussion-partial}

DDoS and DoS attacks are not in themselves harmful to a victim server or website. An overwhelming amount can cause harm, but there is no issue with letting some through, as long as the victim can handle the traffic load. E.g.\ if a server can handle 500 Mbps of network traffic, and there is an attack of size 1 Gbps, a mitigation system could allow 50\% of the attack traffic to pass, ignoring normal load on the server. For this reason, a high benign accuracy is more important than the malicious accuracy for the two proposed approaches, if implemented as parts of mitigation systems. Ideally, both benign and malicious accuracy should be as high as possible, but occasionally it is necessary to decrease one in the favor of the other. When tuning either of the proposed approaches, if increasing the malicious accuracy causes the benign accuracy to decline, one should reconsider the tuning. On the other hand, it might be worthwhile to choose tuning settings that favor small increments in benign accuracy, even if the malicious accuracy declines. A benign accuracy of 99\% and a malicious accuracy of 90\% is better than 98\% and 97\% respectively. This is because blocking 1 less legitimate user in every 100 is generally more important than blocking 7 extra illegitimate users in every 100. Balancing the benign and malicious accuracy is a problem that would need due consideration, and might need to be tuned specifically for the server or website that implements a mitigation system using the LLC-VAE. Sometimes it might even be necessary to block a certain amount of legitimate users if it means stopping a larger part of a DDoS or DoS attack. E.g.\ if a victim server barely has enough capacity to handle a few percent of an attack, then it is preferable to block a few legitimate users, rather than having all of them losing access to the server.

\subsection{Datasets}
\label{discussion-datasets}

A problem for any machine learning algorithm, is the challenge of making a dataset that represents the problem domain in a realistic manner, and at the same time being in a format that is usable by the algorithm. Creating a dataset that needs to contain benign computer network traffic, as well as DDoS and DoS traffic, can be very time consuming, and comes with multiple pitfalls. One of the most difficult problems, is to gather or create traffic data that properly captures a representative dataset, and spans the expected real world data, as well as not making a dataset consisting of artificial correlations. Ideally, the traffic data should be sampled from real world computer network traffic. This becomes increasingly difficult when considering that in many cases, the traffic data needs to be anonymized. As an alternative, it is possible to create a closed environment, so there is no need for anonymization, but then there is a problem of generating a sufficient amount of traffic data, since deep learning algorithms require large amounts of data. If one decides to gather data from real world network traffic, there is also the problem of properly labeling the different traffic types. Labeling data, when there are thousands or millions of samples, is a huge time investment. There is also an element of uncertainty, because it is not always possible to know for certain whether a network traffic packet, or flow, is benign or malicious. Simulating the traffic data overcomes some of these difficulties. There would no longer be a need for anonymization, labeling could be completely automatic, and generating enough traffic data would be trivial. However, the quality is difficult to guarantee, and the data might not be representative of real world traffic.

\subsubsection{Simulated Datasets}
\label{discussion-simulated}

This thesis utilize two pre-generated datasets, CSECICIDS2018\cite{CSECICIDS2018} and CICIDS2017\cite{CICIDS2017}. They contain benign, and a variety of malicious, computer network traffic flows. Both datasets contain large amounts of data, and most of the feature sets overlap between the two. One is used for training and validation, and one for testing. A drawback in using these datasets, is that the traffic flows are generated from simulated computer network traffic. This is not a problem in regard to the DDoS and DoS attack data, because those are typically computer generated anyway\footnote{Even if real DDoS and DoS attacks are generated, they could be generated in a different manner than in the used datasets.}. In regard to the benign data, simulation could create discrepancies between this data and real world computer network traffic. I.e.\ the proposed approaches could have ended up learning correlations that are not fully applicable to real computer networks. On the flip side, the simulated data could have crippled the performance of the two proposed approaches, by creating benign and malicious data that are too similar.

When the LLC-VAE was applied to the test data, another problem was discovered. Recall back to \cref{experimental-computer-networks}, with the figure of the simulated computer networks \ref{fig:experimental-dataset-network}. Both datasets had very small attack networks and normal networks, with few, unique source and destination IP addresses for each type of DDoS and DoS attack. In some cases, a specific attack type only had one unique source IP address. Intuitively, when making a DDoS and DoS mitigation system with deep learning algorithms, it is logical to have the algorithms learn repeating frequency patterns based on the IP addresses of the network traffic. Especially considering how hard it can be to find other patterns in DDoS and DoS attack traffic, since they are so similar to normal traffic. The problem with this is that it could cause a deep learning model to learn the specific IP addresses, and not the correlation between them and the traffic patterns. This assertion is supported by what was found in \cref{analysis}, \nameref{analysis}, regarding the results from figure \ref{fig:p4-ip-and-noip}. When the LLC-VAE performs better on the test results, it means that it generalizes better, i.e.\ less overfitting. From the analysis, the LLC-VAE performed better on the training and validation set when including the IP addresses, but was worse for the test results. Interestingly, the LLC-VAE performed relatively well on the validation set, even without the use of IP addresses, showing that they are not necessary features for training the model to separate DDoS and DoS attacks from benign traffic.

\subsubsection{Attack Vectors}

A limitation of the two datasets used for this thesis, is the lack of variation in the attack vectors of the DDoS and DoS attacks. Recall back to \cref{methodology-2018}, all of the attacks from the dataset used for training, except one, used HTTP as the attack vector\footnote{The test set, as explained in \cref{methodology-2017}, also used HTTP as the attack vector for the attacks.}. The only attack class that did not, was the DDoS  LOIC-UDP attack, which had very few traffic flow samples. Exactly how much the lack of variety in the attack vectors affected the two proposed approaches is difficult to tell without further testing on other datasets. It could have caused the LLC-VAE or LBD-VAE to overfit towards the training set. The test set would not have shown any signs of overfitting because of the test set also only had attacks that used HTTP. Even though HTTP is one of the most common attack vectors for DDoS and DoS attacks, the used datasets might have been providing a too limited representation of DDoS and DoS attacks in general.

The LBD-VAE will require some work if it is to be used as a part of a mitigation system. If the malicious accuracy were to be increased by tuning and modifying the model, the LBD-VAE has the potential to mitigate DDoS and DoS attacks that it has never observed during training. The LBD-VAE is initially trained exclusively on benign traffic flows, before training the threshold that separates benign from malicious flows. If the threshold is set correctly, it might not matter that the datasets only have DDoS and DoS attacks that use HTTP as their attack vector. The LBD-VAE would classify attacks as anomalies either way, as long as they do not match the benign traffic signature. That is after all one of the strengths of an autoencoder, the ability to detect anomalies based on obscure data patterns. As a side effect, legitimate connections that does not match the benign traffic signature, could end up being blocked by the LBD-VAE.

\subsubsection{Validation Set and Test Set}

During the multiple training runs of the two proposed approaches, we used a training set, a validation set, and a test set. All three sets have the same input feature set, as such they can be used for the same model. The deep learning models learn from the training set, and the models are adjusted based on the results from the validation set. This way, overfitting can be prevented, by understanding what model parameters influence the capabilities of the model to generalize and learn. As for the test set, normally one would only use it to assess the performance of a fully specified classifier. For the two proposed approaches however, in \cref{analysis}, \nameref{analysis}, we used the test set to determine what tuning settings were optimal\footnote{Using a test set for tuning is not a preferable approach. This was in part done because of necessity. There are few publicly available datasets containing DDoS and DoS data, and even fewer that are compatible to use with each other.}. From there, we adjusted the models until we found the tuning settings that gave the best test results thus far, see \cref{analysis-comparison}. By doing this, one could argue that the test set is used as a second validation set, and not as an actual test set. In some cases, there was a slight decline in overall accuracy on the validation set, when the tuning settings for the models were changed to improve the test results. It was necessary to do this, however. Without inspecting the test set between tunings, we might not have discovered what input features, and which tuning settings, caused overfitting of the LLC-VAE and the LBD-VAE. In addition, the training set and validation set are internally correlated, which caused the models to learn feature relations specific to those sets. This meant that we could not trust the validation set results alone. That is why using the test set for tuning, in addition to the validation set, was necessary for better understanding of how the models learned. Doing this might have caused overfitting towards the test set, so ideally, other test sets should have been used.



\subsection{Future Work}

This section will be used to discuss possible future work. Presenting how the two proposed approaches can be improved, and discuss what the best approach is to implement either of them as a part of a complete mitigation system.

\subsubsection{Implementing a Complete Mitigation System}

In their current state, the two proposed approaches do not explicitly perform mitigation. However, both approaches are able to detect benign and malicious network traffic on a flow level. The step from classifying individual traffic flows, to blocking the flows or the source, is not a big one. The simplest way to mitigate the attack flows, is to block and keep track of the source IP addresses that are associated with the flows that have been classified as malicious. I.e.\ by using a blacklist, alternatively a whitelist, or both. As an improvement, the whitelist or blacklist can be used to keep track of repeating IP addresses. So that the addresses that have been associated with legitimate traffic has a higher chance of being let through. This could potentially improve the overall accuracy of the mitigation system, by adding a second security layer after the LLC-VAE or the LBD-VAE. Although this is outside of the scope of this thesis, as it is not a deep learning problem.

In order to create a complete mitigation system, there needs to be a method for generating flows from network packets. Currently, the two proposed approaches rely on pre-generated datasets. The flow generator would be installed onto a computer network, where it can retrieve packets, transform them to flows, and send the flows to the LLC-VAE or the LBD-VAE. One way to transform the packets to flows, is to keep a table of entries, where each entry represents a communication session that tracks information about the packets sent back and forth between two IP addresses\cite[p.~56]{Noonan-and-Dubrawsky-2006}. See also \cref{background-packet-state}. Adding a pre-processing step like this is not difficult, the problem lies with the added time spent processing the traffic moving in and out of a computer network. Optimizing the time spent on pre-processing network packets is vital to creating an efficient mitigation system. Failing to reduce the pre-processing time sufficiently can lead to the system slowing down incoming and outgoing network traffic, by spending too much time handling the packets. Ideally, the mitigation system would handle packets directly, but the two proposed approaches need traffic flows to function, more about this in \cref{discussion-memory}.

\subsubsection{Live Training}

To overcome the lack of available DDoS and DoS datasets, and the problems with creating datasets from scratch, it is possible to train the proposed approaches live. That is to say, continuing the training after installing the complete mitigation system on a computer network. The mitigation system could then either be trained continuously, or for a set amount of time.

At the beginning of the training, the mitigation system would not actively filter incoming connections, but first establish a high accuracy by learning from the computer network.

One of the difficulties with live training is that there is no way to know for certain whether the network traffic is of a benign or malicious nature. If the mitigation system were to be pre-trained on datasets, before starting live training, the deep learning models could first learn to recognize traffic types, then adjust itself during live training. Network packets are not labeled, so we would have to assume the nature of the network traffic. Alternatively, we could assume all live traffic to be benign, then simulate DDoS and DoS attacks against the computer network. That way the mitigation system would have some labeled data to learn from\footnote{Important to note, is that if live training the models, there would be much more benign traffic than malicious. This could cause the models to forget the malicious attack patterns, because the weights and node values would be adjusted to fit the benign.}.

Live training is a method to ensure continuous learning for the proposed approaches, but there are some pitfalls we could inadvertently end up falling in. When a deep learning model is set to learn constantly, it might learn from erroneous data. E.g.\ if an attacker has obtained knowledge about the live training, they can condition the mitigation system to let their attack through. This can be done by first transferring legitimate traffic over a period of time, then sending an attack with many of the same patterns. That is to say, attackers could induce erroneous learning in the models\footnote{On the same note, the model weights and node values would need to be kept secret. Lest an attacker train their own machine learning algorithm to generate attack traffic that looks like benign to the mitigation system.}. To overcome this particular problem, the live training could be turned on only at specific time intervals. This will not fix the problem completely, but can diminish it. Also, if we do not want the mitigation system to learn from DDoS and DoS attack traffic, the training could be turned off when it is suspected that an attack is happening.

\subsubsection{Using Memory Models for Packet Classification}
\label{discussion-memory}

When work started on this thesis, the original plan was to implement a RNN, in the form of a LSTM, in addition to the two proposed approaches. With its memory capabilities, a LSTM could potentially replace the need for a system that store session information to create flows from packets. By directly performing DDoS and DoS mitigation on network packets, the overall time spent processing network traffic with this approach could be greatly reduced. As compared to the two proposed flow based approaches. The LSTM could read information from network packets, and store relevant information relating to the packets transferred between two IP addresses in a connection. Each connection and the information about the packets sent between them, would be stored in individual memory units. One of the major difficulties with using a LSTM for DDoS and DoS mitigation, lies with the issue of keeping relevant feature abstractions in memory. Given a packet that arrives at time step $n$. If there are too many packets in between time step $n$ and $n + k$, the relevant memory unit is likely to have been re-appropriated to store something else. For this thesis, the plan to use a LSTM was ultimately discarded because of time constraints.

As an alternative to utilizing a LSTM for mitigation, it could be implemented as a part of the LLC-VAE or the LBD-VAE. Previously we discussed how the current approaches relies on traffic flows, thus needing a system to create flows from packets. An idea could be to use a LSTM to create flows, or otherwise generate features, that the proposed approaches could use for training and mitigation. Whether this would reduce the pre-processing time, when compared to a simple table storing session information, is difficult to tell without implementing and testing such a system. It could be a potential avenue for future work.

\subsubsection{Further Feature Selection With LIME}
\label{discussion-selection}

The current results from \cref{analysis}, \nameref{analysis}, showed a significant improvement after manually selecting input features with LIME\cite{Ribeiro-et-al-2016}. This suggests that further research on manual feature selection could lead to even better results. So far, we have only removed the least used input features, or features we suspected to have a negative impact on the training of the models. A possibility is to remove individual features, and train the models on the remaining ones. Doing this would be very time consuming, because the models would need to be trained many times, on a multitude of feature combinations out of the original 76. To reduce the time spent training the models, input features could be removed in groups so there would be fewer possible feature combinations. As an alternative, instead of guessing what input features to remove with LIME, one could also theorize what features might cause overfitting, or reduction of accuracy, in the models. This would be similar to how we theorized, and showed with results, that the IP addresses caused a negative impact on the training of the two proposed approaches. As an added benefit of removing features before model training, it would reduce overall processing time for the complete mitigation system. This is because there would be less features generated by the pre-processing step that turns packets into flows, and the LLC-VAE and the LBD-VAE would train on fewer features.





\end{document}


==> parts/experimental_setup.tex <==
\begin{document}

\chapter{Experimental Setup}
\label{experimental-setup}

This chapter will be used to present the proposed algorithms from the previous chapter. We will explain the specifications of the system used to run the programs, the computer network setup that the datasets came from, and what tools that were used to create the proposed algorithms. Before moving on to the analysis chapter, we will explain how the models can be tuned, and suggest some presets.

\section{System Specifications}

All the experiments were performed on a single system, using the two datasets CSECICIDS2018\cite{CSECICIDS2018} and CICIDS2017\cite{CICIDS2017}. The computer system runs on Windows 10 64-bit version. For deep learning, the most important hardware components are the memory, CPU and GPU. The system has 16GB of RAM, uses a Intel Core i7-5930K CPU with 6 cores at 3.50GHz (stock frequency), and a Nvidia GeForce GTX 1080 graphics card with 8GB of dedicated GPU-memory.

When running the experiments, it is possible to adjust the batch size that is fed to the deep learning models as a hyperparameter. The number of flows in one batch should usually be as high as possible to ensure optimal learning and speed up model convergence time\cite{Smith-et-al-2017, Keskar-et-al-2016}. Because the models mainly run on the GPU, the only limitation on batch size is the dedicated GPU-memory. After running a few experiments, we found a batch size of about 1000 flows per batch to be the optimal amount to ensure stable training. The deep learning models mainly run using the GPU, so the CPU is at about 15\% usage during runtime when the GPU is at max memory load. RAM usage by the model is about 6.5GB during runtime, but it should be noted that this is because we load the whole training dataset into memory to reduce training times. It is possible to rely more on the disk to reduce memory usage, but this would result in slower training times.

\section{Datasets}
\label{experimental-computer-networks}

For the two proposed approaches presented in this thesis, we use the CSECICIDS2018 dataset\cite{CSECICIDS2018} for training and validation, and the CICIDS2017 dataset\cite{CICIDS2017} for testing. The terms validation set and test set, are often used interchangeably to describe the same thing, a dataset for improving a machine learning model. For the remainder of this thesis, when we discuss validation sets, it means flows from the same computer network as the training set. The CSECICIDS2018 dataset will be split into two subsets, one is the training set, and the other the validation set. When discussing test sets, it means flows from a different computer network than the ones featured in the training and validation sets, but that follows the same probability distribution. The CICIDS2017 dataset will be used for this. Although the test dataset, CICIDS2017, has fewer malicious flow types than the training and validation set from CSECICIDS2018, all of the flow types in CICIDS2017 are present in CSECICIDS2018, and will thus not pose a problem for using CICIDS2017 as a test set.

A simplified version of the computer networks used to simulate the flows can be seen in figure \ref{fig:experimental-dataset-network}. The CICIDS2017 network is to the left, while the CSECICIDS2018 network is to the right. In both computer networks, the benign data had multiple, different sources and destinations. The attacks always targeted the victim network, and came from a separate attack network. The IP addresses of the attack flows can be seen in figure \ref{fig:experimental-dataset-network}, below their respective networks.

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.5]{img/figures/combined_simple_network.pdf}
    \caption[Simple Computer Networks of Used Datasets]{Simple example of the computer network setups used to generate the CICIDS2017 dataset (left), and the CSECICIDS2018 dataset (right). For the full network setup of the CICIDS2017 dataset, see \cite{Sharafaldin-et-al-2018}. For the full network setup of the CSECICIDS2018 dataset, see \cite{CSECICIDS2018}.}
    \label{fig:experimental-dataset-network}
\end{figure}

\section{Tools}

There are various tools and software available to use with and to create deep learning models. The tools used in this thesis to develop the two proposed approaches are Tensorflow\cite{Tensorflow} and Tensorboard, Keras\cite{Chollet-et-al-2015}, Python\cite{Python}, Scikit-learn\cite{scikit-learn}, and LIME\cite{Ribeiro-et-al-2016}.

Python\cite{Python} is a high level programming language with an extensive public code library. All code used in this thesis is written in Python version 3.6, together with the machine learning libraries Tensorflow, API version 1.12\cite{Tensorflow}, Keras version 2.2.4\cite{Chollet-et-al-2015}, and Scikit-learn version 0.20\cite{scikit-learn}. Tensorflow is a machine learning library available to use with Python. Tensorflow simplifies the otherwise complex process of developing machine learning and deep learning algorithms, by providing an API to developers. Machine learning as a field can be difficult and extremely time consuming to develop without having proper knowledge of the science behind it. With Tensorflow, this is no longer as necessary, since the API simplifies many of the most difficult parts into simple to use classes, methods, and functions. Together with Tensorflow, we use Keras which is a deep learning library that can be used together with Tensorflow. To visualize the deep learning model performance, we use Tensorboard, which is a tool integrated in the Tensorflow API. The graphs logged into Tensorboard are used for further development of the two proposed approaches, as well as for model analysis, as can be seen in \cref{analysis}, \nameref{analysis}.

Together with Tensorboard, we use confusion matrices for statistical analysis of model performance. The code for generating and plotting a confusion matrix is based on the open-source example code from the Scikit-learn website\cite{scikit-learn}. A confusion matrix shows the true positive (TP), false positive (FP), false negative (FN), and true negative (TN) rates for a given classification problem when there are two classes. When there are multiple classes, the center diagonal shows the true detection rate for each individual class, while all other boxes shows the falsely predicted labels, as can be seen in e.g.\ figure \ref{fig:p4-te-cm}. We use the confusion matrices to show model performance, and to show how the models perform on different tuning settings.

To properly understand and improve the proposed deep learning algorithms, we use Tensorboard to understand model performance during runtime, and a tool called Local Interpretable Model-Agnostic Explanations (LIME) by Ribeiro et al.\cite{Ribeiro-et-al-2016}. Part of what makes machine learning models difficult to manage, is their inherent black box structure due to  the hidden layers and many feature abstractions. When using a deep learning model to make class predictions, the predictions are based on the activations of the weights and nodes in the preceding layers. It is possible to look at the weights and node values of each layer, but it is difficult to interpret what it means. While a machine learning model can provide good results, it is useful to understand how those results came to be, and not trust blindly in the model's ability to produce them. LIME is a tool used to assist with better understanding of a machine learning model. For tabular data, which is the case of the computer network flow features we use, LIME can be used to explain the prediction probabilities from the deep learning model weights. Each feature is given a weight for each flow, which shows how the different features influenced the model predictions. We can use this tool to learn how the two proposed models classify flows, and for feature removal, to ensure better generalization. More on how we use LIME can be seen in \cref{analysis-lime}

\section{Tuning Presets}
\label{es-parameters}

An important part of any deep learning model is to tune its settings so it is able to produce a useful result. To properly capture the nuances of the two proposed approaches, and as an attempt at exploring which settings work well, we experiment with multiple, promising presets. These will be used for comparison, to show on what settings the models perform well, and on what settings they come up short. Six presets will be presented initially, with more later, each with a reference name for easy lookup. The LBD-VAE will have its own presets, detailed in \cref{analysis-lbd-results}.

The hyperparameters that will be used for tuning are:

\begin{itemize}
    \item Optimizer learning rate (LR)
    \item KL-Loss multiplier (KLM)
    \item Number of training batches iterated (Steps)
\end{itemize}

The dataset transformations used for tuning are:

\begin{itemize}
    \item Scaling technique (ST)
    \begin{itemize}
        \item No scaling (None)
        \item Min-Max normalization (N-18) or (N-18/17)\footnote{Normalization uses sampled min and max values from the used datasets. A notation of (N-18) means the values are sampled from CSECICIDS2018, while a notation of (N-18/17) means the values are sampled from both CSECICIDS2018 and CICIDS2017.}
        \item Logarithmic scaling (Log)
    \end{itemize}
\end{itemize}

Other settings that will be used for tuning:

\begin{itemize}
    \item Type of layers used for encoding and decoding (LT)
    \begin{itemize}
        \item Convolutional layers (Conv)
        \item Fully connected layers (Dense)
    \end{itemize}
    \item Regularizing layer type (RLT)
    \begin{itemize}
        \item Batch normalization (Batch)
    \end{itemize}
\end{itemize}

Unless noted otherwise, all training done with convolutional layers will use a kernel size of 5 for each layer, a stride size of 2 for the first layer, and a stride size of 1 for the other two layers. This means that the 76 input features will be reduced to 38 abstract features at the first convolutional layer of the encoder, 34 features at the second layer, and 30 features for the third layer and the latent layer.

\subsection{Presets}

\begin{table}[htbp]
    \begin{subtable}[b]{0.3\textwidth}
        \caption{Preset 1}
        \label{tab:es-p1}
        \centering
        \arrayrulecolor{black}
        \begin{tabular}{l|r}
            \hline
            Parameter & Value                                             \\
            \arrayrulecolor{black}\hline
            LR        & $1 \cdot 10^{-2}$                                 \\
            KLM       & 1                                                 \\
            Steps     & 15,000                                            \\
            ST        & None                                              \\
            LT        & Conv                                              \\
            RLT       & Batch                                             \\
        \end{tabular}
    \end{subtable}
    \hfill
    \begin{subtable}[b]{0.3\textwidth}
        \caption{Preset 2}
        \label{tab:es-p2}
        \centering
        \arrayrulecolor{black}
        \begin{tabular}{l|r}
            \hline
            Parameter & Value                                             \\
            \arrayrulecolor{black}\hline
            LR        & $1 \cdot 10^{-2}$                                 \\
            \rowcolor{Gray}
            KLM       & $1 \cdot 10^{-2}$                                 \\
            Steps     & 15,000                                            \\
            \rowcolor{Gray}
            ST        & N-18                                              \\
            LT        & Conv                                              \\
            RLT       & Batch                                             \\
        \end{tabular}
    \end{subtable}
    \hfill
    \begin{subtable}[b]{0.3\textwidth}
        \caption{Preset 3}
        \label{tab:es-p3}
        \centering
        \arrayrulecolor{black}
        \begin{tabular}{l|r}
            \hline
            Parameter & Value                                             \\
            \arrayrulecolor{black}\hline
            \rowcolor{Gray}
            LR        & $1 \cdot 10^{-4}$                                \\
            KLM       & $1 \cdot 10^{-2}$                                 \\
            \rowcolor{Gray}
            Steps     & 30,000                                            \\
            \rowcolor{Gray}
            ST        & \scalebox{0.8}{N-18/17}                                              \\
            LT        & Conv                                              \\
            RLT       & Batch                                             \\
        \end{tabular}
    \end{subtable}
    \hfill
    \begin{subtable}[b]{0.3\textwidth}
        \caption{Preset 4}
        \label{tab:es-p4}
        \centering
        \arrayrulecolor{black}
        \begin{tabular}{l|r}
            \hline
            Parameter & Value                                             \\
            \arrayrulecolor{black}\hline
            LR        & $1 \cdot 10^{-4}$                                 \\
            \rowcolor{Gray}
            KLM       & $1 \cdot 10^{-4}$                                 \\
            Steps     & 30,000                                            \\
            \rowcolor{Gray}
            ST        & Log                                               \\
            LT        & Conv                                              \\
            RLT       & Batch                                             \\
        \end{tabular}
    \end{subtable}
    \hfill
    \begin{subtable}[b]{0.3\textwidth}
        \caption{Preset 5}
        \label{tab:es-p5}
        \centering
        \arrayrulecolor{black}
        \begin{tabular}{l|r}
            \hline
            Parameter & Value                                             \\
            \arrayrulecolor{black}\hline
            LR        & $1 \cdot 10^{-4}$                                 \\
            KLM       & $1 \cdot 10^{-4}$                                 \\
            Steps     & 30,000                                            \\
            ST        & Log                                               \\
            \rowcolor{Gray}
            LT        & Dense                                             \\
            RLT       & Batch                                             \\
        \end{tabular}
    \end{subtable}
    \hfill
    \begin{subtable}[b]{0.3\textwidth}
        \caption{\textbf{Preset 6}}
        \label{tab:es-p6}
        \centering
        \arrayrulecolor{black}
        \begin{tabular}{l|r}
            \hline
            Parameter & Value                                             \\
            \arrayrulecolor{black}\hline
            LR        & $1 \cdot 10^{-4}$                                 \\
            \rowcolor{Gray}
            KLM       & None                                              \\
            Steps     & 30,000                                            \\
            ST        & Log                                               \\
            \rowcolor{Gray}
            LT        & Conv                                              \\
            RLT       & Batch                                             \\
        \end{tabular}
    \end{subtable}
    \caption[Tuning Presets]{All presets parameters. The parameters that change between presets have been highlighted in gray. Preset 6 (in bold) only uses P-Loss to improve, which means that it is not a VAE, but just a simple convolutional neural network that performs dimensionality reduction.}
    \label{tab:es-presets}
\end{table}

\begin{document}

\chapter{Experimental Setup}
\label{experimental-setup}

This chapter will be used to present the proposed algorithms from the previous chapter. We will explain the specifications of the system used to run the programs, the computer network setup that the datasets came from, and what tools that were used to create the proposed algorithms. Before moving on to the analysis chapter, we will explain how the models can be tuned, and suggest some presets.

\subsection{System Specifications}

All the experiments were performed on a single system, using the two datasets CSECICIDS2018\cite{CSECICIDS2018} and CICIDS2017\cite{CICIDS2017}. The computer system runs on Windows 10 64-bit version. For deep learning, the most important hardware components are the memory, CPU and GPU. The system has 16GB of RAM, uses a Intel Core i7-5930K CPU with 6 cores at 3.50GHz (stock frequency), and a Nvidia GeForce GTX 1080 graphics card with 8GB of dedicated GPU-memory.

When running the experiments, it is possible to adjust the batch size that is fed to the deep learning models as a hyperparameter. The number of flows in one batch should usually be as high as possible to ensure optimal learning and speed up model convergence time\cite{Smith-et-al-2017, Keskar-et-al-2016}. Because the models mainly run on the GPU, the only limitation on batch size is the dedicated GPU-memory. After running a few experiments, we found a batch size of about 1000 flows per batch to be the optimal amount to ensure stable training. The deep learning models mainly run using the GPU, so the CPU is at about 15\% usage during runtime when the GPU is at max memory load. RAM usage by the model is about 6.5GB during runtime, but it should be noted that this is because we load the whole training dataset into memory to reduce training times. It is possible to rely more on the disk to reduce memory usage, but this would result in slower training times.

\subsection{Datasets}
\label{experimental-computer-networks}

For the two proposed approaches presented in this thesis, we use the CSECICIDS2018 dataset\cite{CSECICIDS2018} for training and validation, and the CICIDS2017 dataset\cite{CICIDS2017} for testing. The terms validation set and test set, are often used interchangeably to describe the same thing, a dataset for improving a machine learning model. For the remainder of this thesis, when we discuss validation sets, it means flows from the same computer network as the training set. The CSECICIDS2018 dataset will be split into two subsets, one is the training set, and the other the validation set. When discussing test sets, it means flows from a different computer network than the ones featured in the training and validation sets, but that follows the same probability distribution. The CICIDS2017 dataset will be used for this. Although the test dataset, CICIDS2017, has fewer malicious flow types than the training and validation set from CSECICIDS2018, all of the flow types in CICIDS2017 are present in CSECICIDS2018, and will thus not pose a problem for using CICIDS2017 as a test set.

A simplified version of the computer networks used to simulate the flows can be seen in figure \ref{fig:experimental-dataset-network}. The CICIDS2017 network is to the left, while the CSECICIDS2018 network is to the right. In both computer networks, the benign data had multiple, different sources and destinations. The attacks always targeted the victim network, and came from a separate attack network. The IP addresses of the attack flows can be seen in figure \ref{fig:experimental-dataset-network}, below their respective networks.

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.5]{img/figures/combined_simple_network.pdf}
    \caption[Simple Computer Networks of Used Datasets]{Simple example of the computer network setups used to generate the CICIDS2017 dataset (left), and the CSECICIDS2018 dataset (right). For the full network setup of the CICIDS2017 dataset, see \cite{Sharafaldin-et-al-2018}. For the full network setup of the CSECICIDS2018 dataset, see \cite{CSECICIDS2018}.}
    \label{fig:experimental-dataset-network}
\end{figure}

\subsection{Tools}

There are various tools and software available to use with and to create deep learning models. The tools used in this thesis to develop the two proposed approaches are Tensorflow\cite{Tensorflow} and Tensorboard, Keras\cite{Chollet-et-al-2015}, Python\cite{Python}, Scikit-learn\cite{scikit-learn}, and LIME\cite{Ribeiro-et-al-2016}.

Python\cite{Python} is a high level programming language with an extensive public code library. All code used in this thesis is written in Python version 3.6, together with the machine learning libraries Tensorflow, API version 1.12\cite{Tensorflow}, Keras version 2.2.4\cite{Chollet-et-al-2015}, and Scikit-learn version 0.20\cite{scikit-learn}. Tensorflow is a machine learning library available to use with Python. Tensorflow simplifies the otherwise complex process of developing machine learning and deep learning algorithms, by providing an API to developers. Machine learning as a field can be difficult and extremely time consuming to develop without having proper knowledge of the science behind it. With Tensorflow, this is no longer as necessary, since the API simplifies many of the most difficult parts into simple to use classes, methods, and functions. Together with Tensorflow, we use Keras which is a deep learning library that can be used together with Tensorflow. To visualize the deep learning model performance, we use Tensorboard, which is a tool integrated in the Tensorflow API. The graphs logged into Tensorboard are used for further development of the two proposed approaches, as well as for model analysis, as can be seen in \cref{analysis}, \nameref{analysis}.

Together with Tensorboard, we use confusion matrices for statistical analysis of model performance. The code for generating and plotting a confusion matrix is based on the open-source example code from the Scikit-learn website\cite{scikit-learn}. A confusion matrix shows the true positive (TP), false positive (FP), false negative (FN), and true negative (TN) rates for a given classification problem when there are two classes. When there are multiple classes, the center diagonal shows the true detection rate for each individual class, while all other boxes shows the falsely predicted labels, as can be seen in e.g.\ figure \ref{fig:p4-te-cm}. We use the confusion matrices to show model performance, and to show how the models perform on different tuning settings.

To properly understand and improve the proposed deep learning algorithms, we use Tensorboard to understand model performance during runtime, and a tool called Local Interpretable Model-Agnostic Explanations (LIME) by Ribeiro et al.\cite{Ribeiro-et-al-2016}. Part of what makes machine learning models difficult to manage, is their inherent black box structure due to  the hidden layers and many feature abstractions. When using a deep learning model to make class predictions, the predictions are based on the activations of the weights and nodes in the preceding layers. It is possible to look at the weights and node values of each layer, but it is difficult to interpret what it means. While a machine learning model can provide good results, it is useful to understand how those results came to be, and not trust blindly in the model's ability to produce them. LIME is a tool used to assist with better understanding of a machine learning model. For tabular data, which is the case of the computer network flow features we use, LIME can be used to explain the prediction probabilities from the deep learning model weights. Each feature is given a weight for each flow, which shows how the different features influenced the model predictions. We can use this tool to learn how the two proposed models classify flows, and for feature removal, to ensure better generalization. More on how we use LIME can be seen in \cref{analysis-lime}

\subsection{Tuning Presets}
\label{es-parameters}

An important part of any deep learning model is to tune its settings so it is able to produce a useful result. To properly capture the nuances of the two proposed approaches, and as an attempt at exploring which settings work well, we experiment with multiple, promising presets. These will be used for comparison, to show on what settings the models perform well, and on what settings they come up short. Six presets will be presented initially, with more later, each with a reference name for easy lookup. The LBD-VAE will have its own presets, detailed in \cref{analysis-lbd-results}.

The hyperparameters that will be used for tuning are:

\begin{itemize}
    \item Optimizer learning rate (LR)
    \item KL-Loss multiplier (KLM)
    \item Number of training batches iterated (Steps)
\end{itemize}

The dataset transformations used for tuning are:

\begin{itemize}
    \item Scaling technique (ST)
    \begin{itemize}
        \item No scaling (None)
        \item Min-Max normalization (N-18) or (N-18/17)\footnote{Normalization uses sampled min and max values from the used datasets. A notation of (N-18) means the values are sampled from CSECICIDS2018, while a notation of (N-18/17) means the values are sampled from both CSECICIDS2018 and CICIDS2017.}
        \item Logarithmic scaling (Log)
    \end{itemize}
\end{itemize}

Other settings that will be used for tuning:

\begin{itemize}
    \item Type of layers used for encoding and decoding (LT)
    \begin{itemize}
        \item Convolutional layers (Conv)
        \item Fully connected layers (Dense)
    \end{itemize}
    \item Regularizing layer type (RLT)
    \begin{itemize}
        \item Batch normalization (Batch)
    \end{itemize}
\end{itemize}

Unless noted otherwise, all training done with convolutional layers will use a kernel size of 5 for each layer, a stride size of 2 for the first layer, and a stride size of 1 for the other two layers. This means that the 76 input features will be reduced to 38 abstract features at the first convolutional layer of the encoder, 34 features at the second layer, and 30 features for the third layer and the latent layer.

\subsubsection{Presets}

\begin{table}[htbp]
    \begin{subtable}[b]{0.3\textwidth}
        \caption{Preset 1}
        \label{tab:es-p1}
        \centering
        \arrayrulecolor{black}
        \begin{tabular}{l|r}
            \hline
            Parameter & Value                                             \\
            \arrayrulecolor{black}\hline
            LR        & $1 \cdot 10^{-2}$                                 \\
            KLM       & 1                                                 \\
            Steps     & 15,000                                            \\
            ST        & None                                              \\
            LT        & Conv                                              \\
            RLT       & Batch                                             \\
        \end{tabular}
    \end{subtable}
    \hfill
    \begin{subtable}[b]{0.3\textwidth}
        \caption{Preset 2}
        \label{tab:es-p2}
        \centering
        \arrayrulecolor{black}
        \begin{tabular}{l|r}
            \hline
            Parameter & Value                                             \\
            \arrayrulecolor{black}\hline
            LR        & $1 \cdot 10^{-2}$                                 \\
            \rowcolor{Gray}
            KLM       & $1 \cdot 10^{-2}$                                 \\
            Steps     & 15,000                                            \\
            \rowcolor{Gray}
            ST        & N-18                                              \\
            LT        & Conv                                              \\
            RLT       & Batch                                             \\
        \end{tabular}
    \end{subtable}
    \hfill
    \begin{subtable}[b]{0.3\textwidth}
        \caption{Preset 3}
        \label{tab:es-p3}
        \centering
        \arrayrulecolor{black}
        \begin{tabular}{l|r}
            \hline
            Parameter & Value                                             \\
            \arrayrulecolor{black}\hline
            \rowcolor{Gray}
            LR        & $1 \cdot 10^{-4}$                                \\
            KLM       & $1 \cdot 10^{-2}$                                 \\
            \rowcolor{Gray}
            Steps     & 30,000                                            \\
            \rowcolor{Gray}
            ST        & \scalebox{0.8}{N-18/17}                                              \\
            LT        & Conv                                              \\
            RLT       & Batch                                             \\
        \end{tabular}
    \end{subtable}
    \hfill
    \begin{subtable}[b]{0.3\textwidth}
        \caption{Preset 4}
        \label{tab:es-p4}
        \centering
        \arrayrulecolor{black}
        \begin{tabular}{l|r}
            \hline
            Parameter & Value                                             \\
            \arrayrulecolor{black}\hline
            LR        & $1 \cdot 10^{-4}$                                 \\
            \rowcolor{Gray}
            KLM       & $1 \cdot 10^{-4}$                                 \\
            Steps     & 30,000                                            \\
            \rowcolor{Gray}
            ST        & Log                                               \\
            LT        & Conv                                              \\
            RLT       & Batch                                             \\
        \end{tabular}
    \end{subtable}
    \hfill
    \begin{subtable}[b]{0.3\textwidth}
        \caption{Preset 5}
        \label{tab:es-p5}
        \centering
        \arrayrulecolor{black}
        \begin{tabular}{l|r}
            \hline
            Parameter & Value                                             \\
            \arrayrulecolor{black}\hline
            LR        & $1 \cdot 10^{-4}$                                 \\
            KLM       & $1 \cdot 10^{-4}$                                 \\
            Steps     & 30,000                                            \\
            ST        & Log                                               \\
            \rowcolor{Gray}
            LT        & Dense                                             \\
            RLT       & Batch                                             \\
        \end{tabular}
    \end{subtable}
    \hfill
    \begin{subtable}[b]{0.3\textwidth}
        \caption{\textbf{Preset 6}}
        \label{tab:es-p6}
        \centering
        \arrayrulecolor{black}
        \begin{tabular}{l|r}
            \hline
            Parameter & Value                                             \\
            \arrayrulecolor{black}\hline
            LR        & $1 \cdot 10^{-4}$                                 \\
            \rowcolor{Gray}
            KLM       & None                                              \\
            Steps     & 30,000                                            \\
            ST        & Log                                               \\
            \rowcolor{Gray}
            LT        & Conv                                              \\
            RLT       & Batch                                             \\
        \end{tabular}
    \end{subtable}
    \caption[Tuning Presets]{All presets parameters. The parameters that change between presets have been highlighted in gray. Preset 6 (in bold) only uses P-Loss to improve, which means that it is not a VAE, but just a simple convolutional neural network that performs dimensionality reduction.}
    \label{tab:es-presets}
\end{table}


\end{document}

\end{document}


==> parts/foreword.tex <==
\begin{document}

\section{Foreword}

some text

\end{document}


==> parts/introduction.tex <==
\begin{document}

\chapter{Introduction}

The Internet has been growing in size ever since its conception, allowing access to any device with networking capabilities. As new and more advanced technology is researched, created and sold, at ever decreasing prices, more and more people gain access to the Internet through one or more networking capable devices. Malicious network traffic does not originate exclusively from personal computers, but can come from multiple sources, many of them from devices in the Internet of things (IoT). In 2017, the amount of network devices was estimated to consist of 18 billion units, according to an ongoing initiative by Cisco to track and forecast networking trends\cite{Cisco-forecast-2019}. This number is expected to increase to about 28.5 billion devices by 2022. Embedded devices are included in these statistics as well, which do not necessarily have Internet connection, but the amount of devices with potential for launching malicious network traffic is still in the billions. Given the sheer number of units available for network attacks, it would be near impossible to manually create solutions for combating the problem of filtering out the malicious traffic from the harmless.

When talking about IoT, we refer to devices with an Internet connection. These include personal computers, smart phones, and other devices such as printers or surveillance cameras with networking capabilities. Some of these devices are less secure than others, and more vulnerable to theft in the sense that they can be used as a part of a botnet, or as a source of attack by an external party. Any device with Internet capabilities has an Internet Protocol (IP) address and an internal computing device, and is thus able to send malicious traffic. Amongst the most notable, and perhaps hardest to prevent are denial of service (DoS) and distributed DoS (DDoS) attacks. DDoS and DoS attacks have become immense threats over the last decade to any Internet connected machine. In 2015, a global survey of a number of companies conducted by Kaspersky found that 50\% of DDoS attacks caused a noticeable disruption in services, and 24\% led to a complete denial of service\cite{Kaspersky-risk-report-2015,Kaspersky-risk-report-2015-original}. As attacks continue to evolve and as the amount of available IoT devices to launch attacks from grow, these percentages could very well increase, as would the demand for working mitigation systems.

DDoS and DoS attacks are similar in intention and often similar in execution. The goal for both types of attacks is to cause a denial of service for their target, either by exhausting the victim’s bandwidth or system resources, such as CPU or memory. In general terms, causing a denial of service means to overload a victim, for example a web server, with traffic. Once a system receives more traffic than its bandwidth or system resources are able to handle, it will be unable to receive or send new traffic data. Although similar, DDoS and DoS are separated into two categories. When we talk about DoS, we mean denial of service attacks that come from one source. DDoS on the other hand, are denial of service attacks originating from a distributed range of machines and networks. Both types of attacks have proven effective and devastating, but the most difficult to handle has been proven to be DDoS. One reasons for this is the potential size of a DDoS attack.

Cisco reported that the average attack size of a DDoS attack in terms of traffic load was 990 Mbps in 2017\cite{Cisco-forecast-2019}. Because of its distributed nature, a DDoS attack can generate attacks much larger than a normal DoS attack. In late 2016, the peak size was reported to be 1.1 Tbps\cite[p.~14]{Scott-2016} as a result of a DDoS attack consisting of multiple compromised IoT devices. In 2018 the peak size was reported by Cisco to have reached 1.7 Tbps originating from a vulnerability in the memcached protocol\cite{Cisco-forecast-2019}, resulting in the largest DDoS attack to date.

Creating an effective mitigation system requires due consideration of multiple facets of both DDoS and DoS attacks. An effective mitigation system needs to be able to handle large amounts of traffic, processing malicious and normal traffic simultaneously. The system is required to separate harmful from harmless traffic, at such a rate that the targeted victim is able to handle the traffic load. Considering that network packets from a DDoS or DoS attack are not harmful in and of themselves, a mitigation system can let through a certain amount of malicious traffic, while prioritizing letting through as much normal traffic as possible, more about this in the \nameref{discussion} chapter, \cref{discussion-partial}. A mitigation system that fails to meet any of these requirements risks exposing the victim to the attack. If unable to handle incoming traffic load to a server, the mitigation system would cause a general slowdown of the server, due to how it needs to inspect each packet before forwarding or allowing the packets through. If unable to separate normal traffic from malicious, the mitigation system risks blocking normal users from accessing the server, or letting too many malicious packets through. Handling large DDoS attacks can be particularly difficult, considering that the defending system has limited resources to spare for defense, while an attack has the potential to capture and use much larger amounts of devices and their resources to overpower the victim.

Current mitigation systems typically focus on some form of pattern recognition or frequency based detection, or a combination of the two. It is common to have a detection system in place but often this only means that it is able to know when an attack is happening, yet is unable to stop it. This puts system administrators in the precarious situation of having to combat the attack manually, which is only feasible after having the victim server shut down\cite{Zargar-et-al-2013}. When discussing detection systems, it generally encompasses systems that are able to recognize when an attack is happening, or has happened in the past by analyzing the network traffic logs. A mitigation system is different in the way that it is able to differentiate malicious from normal traffic on a packet or flow level, i.e.\ based on IP addresses or other packet information during the attack.

Part of what makes it difficult to differentiate between normal and denial of service traffic is because of how they behave similarly. If we compare two network packets in isolation, one is from a legitimate user, and another is from a compromised computer being used as a part of an attack, in a vacuum the differences would be few to none. DDoS and DoS packets are not harmful on their own. It is the amount of traffic they send that in turn overloads a system, drowning out legitimate attempts at access. This makes it difficult to implement solutions that can keep out malicious connections.

A mitigation system needs to be able to detect what packets or IP addresses are malicious, and stop them from entering the network. Using machine learning algorithms could be a potential way for creating such a system. As machine learning can itself potentially find relations between packet information and intent.

In the last few years, we have seen a rise in the usage and success of machine learning algorithms. Machine learning, specifically deep learning, can be applied to a myriad of different problem domains. Including classification of different types of data and anomaly detection, using a variety of different architectures such as convolutional networks or autoencoders\cite{perera-et-al-2018}. Deep learning have proven effective at analyzing and extracting useful data patterns that manual and automatic approaches are unable to solve in other problem domains outside of computer network traffic. Manual and automatic approaches rely on constant updates as well as human interaction to stay effective against DDoS and DoS attacks. A deep learning solution on the other hand, is autonomous, requiring minimal human interaction. These are among the reasons a deep learning solution could prove to be effective at combating DDoS and DoS attacks.

\section{Problem Statement}

This thesis proposes two approaches for DDoS and DoS mitigation, utilizing the framework of the Variational Autoencoder (VAE) by Kingma and Welling\cite{Kingma-and-Welling-2013}. The first approach is the Latent Layer Classification algorithm (LLC-VAE), which aims to identify different types of computer network traffic from the latent layer representations of the VAE. The second approach is the Loss Based Detection algorithm (LBD-VAE), which tries to identify normal and malicious traffic patterns based on the VAE reconstruction loss function. The two proposed approaches are not meant as finished solutions for mitigation systems, nor are they aimed at creating solutions that work against all types of DDoS and DoS attacks. The contribution of this thesis is the research on how deep learning, specifically a VAE, can detect specific types of DDoS and DoS traffic from network flows. In addition, whether this can be generalized to detect other types of DDoS and DoS attacks, and to what extent. This leads to the first problem statement this thesis will explore:

\textbf{\textit{How can we design a solution based on deep learning for detecting DDoS and DoS attacks?}}

And the second problem statement this thesis will explore:

\textbf{\textit{Can a solution based on deep learning replace traditional mitigation methods?}}

If the LLC-VAE and the LBD-VAE are able to detect DDoS and DoS traffic in a computer network, it could dramatically reduce financial losses and increase security for organizations suffering from a large quantity of attacks. The two proposed approaches will not move past the research stage in this thesis, and will only work as proof of concepts. Yet they could realistically be installed as modules in a computer network system similar to a firewall, with a few additions and alterations.

\section{Outline}

\Cref{background}, \nameref{background} will deal with the necessary background information to understand the discussed topics in this thesis. \Cref{related-work}, \nameref{related-work} presents various related works. \Cref{methodology}, \nameref{methodology} discusses the two proposed approaches, as well as the used datasets. \Cref{experimental-setup}, \nameref{experimental-setup} shows the environment in which the proposed approaches have been tested. \Cref{analysis}, \nameref{analysis} is used to discuss the results achieved by the two proposed approaches. In \Cref{discussion}, \nameref{discussion}, we discuss the strengths and weaknesses of the used datasets, and the proposed approaches. We will also explore future work that can be done for the approaches presented in this thesis. Finally in \cref{conclusion}, \nameref{conclusion}, we will look back at the work done, and discuss the contributions of this thesis.

\end{document}


==> parts/methodology.tex <==
\begin{document}

\chapter{Methodology}
\label{methodology}

This chapter will be used to present and discuss the different approaches used in this thesis for DDoS and DoS mitigation. This thesis will focus mainly on the research aspect of mitigating DDoS and DoS, rather than a practical approach. That is to say, the two proposed approaches will only be used in a research environment on pre-made datasets. They will not be used as fully working mitigation systems that can filter computer network traffic live, hence there will be no algorithms for creating traffic flows, or for keeping track of blocked and allowed IP addresses etc. Instead, the two approaches presented here will be used to detect different types of network traffic flows, and label accordingly. This will allow a practical mitigation system to be easily implemented on top of the models presented here, should one or both of the models prove to be effective.

\section{Available Datasets}
\label{methodology-available}

Using representative datasets is paramount when it comes to machine learning algorithms. Some datasets might lean heavily towards certain types of data, causing a machine learning model to learn from a too specific subset of the full feature space, which in turn can cause overfitting. It could also be the case that a dataset lacks important information, or contains erroneous data or labels, missing out on important features that could be the deciding factor in whether the network traffic is classified correctly. Then there are situations where a dataset simply cannot be used for certain types of models, due to an incompatibility in formatting of said datasets with a type of model.

For this thesis, a dataset needs to contain labeled network traffic with DDoS and DoS attacks, preferably labeled specifically to different types of attacks, but at the very least separating normal traffic from malicious. Unfortunately there are not many publicly available datasets that contain captured network traffic with the necessary information. It would be possible to generate such a dataset ourselves, by simulating benign network traffic, adding DDoS and DoS into the mix, and generate datasets from that, although this process can be very time consuming. Creating a proper dataset can be a whole research topic on its own. There are multiple pitfalls, such as properly capturing a representative dataset spanning the expected real world data, as well as inadvertently not making a dataset consisting of artificial correlations. Because of time restrictions, this is not an option for this thesis. For further discussion on this topic, see \cref{discussion-datasets}.

Multiple different publicly available datasets have been considered for use with the two proposed approaches of this thesis. Amongst these are the KDD’99\cite{KDD99}, NSL-KDD\cite{Tavallaee-et-al-2009}, ISCX2012\cite{Shiravi-et-al-2012}, CICIDS2017\cite{Sharafaldin-et-al-2018,CICIDS2017}, and CSECICIDS2018\cite{CSECICIDS2018}. For an overview of other potential datasets, see\cite{Sharafaldin-et-al-2018}. All of these datasets contain labeled network traffic flows, consisting of normal traffic as well as malicious, including DDoS and DoS attacks.

KDD’99 has for many years been the \textit{de-facto} dataset for researchers creating benchmarks for malicious network traffic mitigation systems. This dataset was considered for this thesis, but was ultimately discarded for a variety of reasons. The most important reason was that the data in the KDD’99 dataset is heavily outdated, containing traffic from almost 20 years ago. There are also multiple redundant records, and the data is heavily anonymized, leading to multiple other problems. For the interested reader, see the analysis of the dataset by Tavallaee et al.\cite{Tavallaee-et-al-2009}. The paper by Tavallaee et al. also proposed a new dataset, NSL-KDD, as an improvement over KDD'99. Although some of the shortcomings of the KDD'99 dataset were rectified or improved in NSL-KDD, the data it contains is still outdated by modern standards and contains no IP addresses because of the anonymization of the original. This makes it difficult to base our mitigation system off of it.

\subsection{Datasets Used}
\label{methodology-datasets}

For this thesis, the Intrusion Detection System (IDS) dataset created through a collaboration between the Communications Security Establishment (CSE) and the Canadian Institute for Cybersecurity (CIC), CSECICIDS2018\cite{CSECICIDS2018}, will be used for training the deep learning based models. Furthermore, we will use the CICIDS2017 dataset\cite{CICIDS2017}, as a test set for the deep learning models\footnote{Both datasets, CSECICIDS2018 and CICIDS2017, are from the Canadian Institute for Cybersecurity. This is also the case for the datasets ISCX2012 and NSL-KDD.}. For an analysis of the two IDS datasets and their features, refer to the paper by  Sharafaldin et al.\cite{Sharafaldin-et-al-2018}. A similar dataset, the ISCXIDS 2012 by Shiravi et al.\cite{Shiravi-et-al-2012}, containing many of the same types of attacks have also been considered for use in this thesis. Due to the similarities, only one or two of these datasets were needed, and the newer 2017 and 2018 versions has been chosen for their more recent contents. For a list of the features used in both datasets, see table \ref{tab:methodology-features}. The features were extracted using CICFlowmeter\footnote{CICFlowmeter is a tool made in the Java programming language, used to generate traffic flow data from network packets.}\cite{Lashkari-et-al-2017}, turning the corresponding raw PCAP data into network flows in a CSV file format. The flows are bidirectional, where one flow represents both the forward and backward direction of a group of packets. TCP flows were terminated by a FIN packet, while UDP flows were terminated by a flow timeout. The CSV files are available for public download at\cite{CICIDS2017,CSECICIDS2018}.

\begin{table}[htbp]
    \centering
    \arrayrulecolor{black}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{llll}
        \arrayrulecolor{black}\hline
        Column 1         & Column 2       & Column 3         & Column 4                                \\
        \arrayrulecolor{black}\hline
        Src IP           & Flow IAT Min   & Pkt Len Std      & Subflow Fwd Pkts                        \\
        Dst IP           & Fwd IAT Tot    & Pkt Len Var      & Subflow Fwd Byts                        \\
        Dst Port         & Fwd IAT Mean   & FIN Flag Cnt     & Subflow Bwd Pkts                        \\
        Protocol         & Fwd IAT Std    & SYN Flag Cnt     & Subflow Bwd Byts                        \\
        Flow Duration    & Fwd IAT Max    & RST Flag Cnt     & Init Fwd Win Byts                       \\
        Tot Fwd Pkts     & Fwd IAT Min    & PSH Flag Cnt     & Init Bwd Win Byts                       \\
        Tot Bwd Pkts     & Bwd IAT Tot    & ACK Flag Cnt     & Fwd Act Data Pkts                       \\
        TotLen Fwd Pkts  & Bwd IAT Mean   & URG Flag Cnt     & Fwd Seg Size Min                        \\
        TotLen Bwd Pkts  & Bwd IAT Std    & CWE Flag Count   & Active Mean                             \\
        Fwd Pkt Len Max  & Bwd IAT Max    & ECE Flag Cnt     & Active Std                              \\
        Fwd Pkt Len Min  & Bwd IAT Min    & Down/Up Ratio    & Active Max                              \\
        Fwd Pkt Len Mean & Fwd PSH Flags  & Pkt Size Avg     & Active Min                              \\
        Fwd Pkt Len Std  & Bwd PSH Flags  & Fwd Seg Size Avg & Idle Mean                               \\
        Bwd Pkt Len Max  & Fwd URG Flags  & Bwd Seg Size Avg & Idle Std                                \\
        Bwd Pkt Len Min  & Bwd URG Flags  & Fwd Byts/b Avg   & Idle Max                                \\
        Bwd Pkt Len Mean & Fwd Header Len & Fwd Pkts/b Avg   & Idle Min                                \\
        Bwd Pkt Len Std  & Bwd Header Len & Fwd Blk Rate Avg & Label                                   \\
        Flow IAT Mean    & Pkt Len Min    & Bwd Byts/b Avg   &                                         \\
        Flow IAT Std     & Pkt Len Max    & Bwd Pkts/b Avg   &                                         \\
        Flow IAT Max     & Pkt Len Mean   & Bwd Blk Rate Avg &
    \end{tabular}
    } %End resizebox
    \caption[Default Features Table]{All features used from the CICIDS2017 and CSECICIDS2018 datasets. The features are in order, starting from top to bottom, and from left to right. For an explanation of the features and what they represent, see the dataset information page\cite{CSECICIDS2018}.}
    \label{tab:methodology-features}
\end{table}

\subsubsection{CICIDS2017}
\label{methodology-2017}

This dataset, CICIDS2017\cite{CICIDS2017}, contains a variety of both malicious and benign computer network traffic records. Amongst them, the majority are flows of normal traffic, labeled \texttt{Benign}. The DDoS and DoS attacks are labeled \texttt{DoS Slowloris}, \texttt{DoS Slowhttptest}, \texttt{DoS Hulk}, \texttt{DoS Goldeneye}, and \texttt{DDoS}. The DDoS attack was simulated using a tool called Low Orbit Ion Cannon (LOIC). LOIC is a tool that can be used for HTTP/TCP/UDP flooding of a server. A single LOIC does not generate enough traffic to cause a denial of service, as such it is typically used with many computers simultaneously, composing a DDoS attack. In total there are over 2.2 million flows of benign traffic, and over 380 thousand flows of DDoS and DoS traffic. For a complete enumeration of the data, their classes, and the attack vectors, see table \ref{tab:methodology-2017}. The amount of normal traffic heavily outweighs the amount of malicious traffic. This unevenness of the distributions will be taken into account during training and testing. Deep learning algorithms needs large amounts of data to be able to learn robust, general, and accurate deep features. Whether this dataset and the CSECICIDS2018 dataset provides a sufficient amount of flows for the two proposed approaches will be discussed in \cref{analysis}, \nameref{analysis}. Although there is an unevenness to the distributions between normal and malicious traffic, there is still a considerable amount of malicious traffic that can be used, and previous research using CICIDS2017 has shown that this dataset could be used to achieve adequate results, see \cref{related-lstm-2017} from the related work chapter. Using this dataset for training can pose a challenge when it comes to the Slowloris, Slowhttptest, and Goldeneye attacks, as there are very few examples of those classes compared to the other types of traffic.

\begin{table}[htbp]
    \centering
    \arrayrulecolor{black}
    \begin{tabular}{lrl}
        \hline
        Traffic Type     & Number of Flows                     & Attack Vector  \\
        \arrayrulecolor{black}\hline
        Benign           & 2,273,098                           & None                                                     \\
        DoS Slowloris    & 5,796                               & HTTP/TCP-SYN                                             \\
        DoS Slowhttptest & 5,499                               & HTTP                                                     \\
        DoS Hulk         & 231,073                             & HTTP                                                     \\
        DoS Goldeneye    & 10,293                              & HTTP/TCP                                                 \\
        DDoS LOIC-HTTP   & 128,027                             & HTTP
    \end{tabular}
    \arrayrulecolor{black}
    \caption[CICIDS2017 Overview]{Overview of traffic flow data in the CICIDS2017\cite{CICIDS2017} dataset.}
    \label{tab:methodology-2017}
\end{table}

\subsubsection{CSECICIDS2018}
\label{methodology-2018}

Similar to the 2017 dataset\cite{CICIDS2017}, this version consists of a variety of malicious traffic types, in addition to benign traffic\cite{CSECICIDS2018}. The DDoS and DoS attacks are labelled \texttt{DoS Slowloris}, \texttt{DoS Slowhttptest}, \texttt{DoS Hulk}, \texttt{DoS Goldeneye}, \texttt{DDoS LOIC-HTTP}, \texttt{DDoS LOIC-UDP}, and \texttt{DDoS HOIC-HTTP}. The DDoS attacks in the 2018 dataset are similar to the attacks in the 2017 version, with the exception of a LOIC-UDP, and a High Orbit Ion Cannon (HIOC) attack class. HIOC is an attack tool used to generate a flood attack by overflowing a victim with HTTP GET and POST requests. It was created as an improvement over the previously discussed LOIC, as well as to fix some of its shortcomings. From this dataset we have more than 7.3 million flows of benign traffic available, and over 1.9 million flows of malicious traffic, with various types of DDoS and DoS attacks. Although similar to the 2017 version, most of the attack types have a considerable amount of flows each, the \texttt{Slowloris}, \texttt{Goldeneye}, and \texttt{LOIC-UDP} attacks have notably fewer flows than the other types.

The low amount of training data might negatively impact the accuracy of the proposed mitigation methods on these types of attacks, as the two proposed approaches might have too little data to properly generalize. In \cref{analysis}, \nameref{analysis}, we will discuss how much this impacts the learning process of the two approaches, if at all.

\begin{table}[htbp]
    \centering
    \arrayrulecolor{black}
    \begin{tabular}{lrl}
        \hline
        Traffic Type     & Number of Flows                     & Attack Vector  \\
        \arrayrulecolor{black}\cline{1-2}\arrayrulecolor{black}\cline{3-3}
        Benign           & 7,372,557                           & None                                                     \\
        DoS Slowloris    & 10,990                              & HTTP/TCP-SYN                                             \\
        DoS Slowhttptest & 139,890                             & HTTP                                                     \\
        DoS Hulk         & 461,912                             & HTTP                                                     \\
        DoS Goldeneye    & 41,508                              & HTTP/TCP                                                 \\
        DDoS LOIC-HTTP   & 576,191                             & HTTP                                                     \\
        DDoS LOIC-UDP    & 1,730                               & UDP                                                      \\
        DDoS HOIC-HTTP   & 686,012                             & HTTP
    \end{tabular}
    \arrayrulecolor{black}
    \caption[CSECICIDS2018 Overview]{Overview of traffic flow data in the CSECICIDS2018\cite{CSECICIDS2018} dataset.}
    \label{tab:methodology-2018}
\end{table}

\subsubsection{Dataset files}

For both datasets, we use the pre-generated CSV files publicly available for download\cite{CICIDS2017, CSECICIDS2018}. The PCAP files are available as well, but due to time constraints and the  overall good quality of the CSV files, we will not generate new datasets. The current datasets will however need transformations to streamline the feature names and the number of features, to be consistent between the two datasets used, as well as to fix weaknesses in the datasets. Among the most notable of the weaknesses in CSECICIDS2018 is the lack of source IP, destination IP, and source port on a subset of the flow traffic. To solve this problem, we looked up the attack source and destination IP for each type of attack reported in the computer network, as seen in figure \ref{fig:experimental-dataset-network}, and added them to each flow missing this data. The source ports were not feasible to recover from the original PCAP files in a reasonable time, and will thus be dropped. Another potential issue is the fact that both datasets uses simulated benign data, and not recorded real world traffic. There is no real way to mitigate this shortcoming without using other datasets, for further discussion on this topic see \cref{discussion-datasets}. Some labels in the pre-generated CSV files might be mislabeled, which could lead to unwanted, or erroneous results\cite{Pektacs-and-Acarman-2018}. After inspection of the datasets, this problem seems to be the exception rather than the rule. As long as it is an anomaly in the data, being numerically clearly in the minority, the already noisy and random techniques of machine learning makes their impact negligible.

\section{Deep Learning Algorithms for Mitigation}

DDoS and DoS mitigation has been researched for many years, and several, different approaches have been created. Examples of approaches have been outlined in \cref{background}, \nameref{background} and \cref{related-work}, \nameref{related-work}. Popular methods for mitigation include pattern recognition, similar to how one would detect viruses, or detection of malicious sources based on network traffic frequency. Pattern recognition mitigation systems have proven effective in certain scenarios, such as when a victim is the target of a known attack, but is also known to have several drawbacks. These kinds of systems are prone to human error, and require constant maintenance to operate, needing code updates every time a new attack surface, or whenever a known one is altered. Traffic frequency based mitigation systems work by blocking network traffic based on high traffic frequency, or allotting a certain amount of bandwidth to each connected IP. Monitoring traffic frequency can be effective if there is a lot of traffic from one source, allowing a mitigation system to block attackers that take up too much of a system's resources. A problem with this approach is that sometimes normal users might be regarded as attackers. For example if they try to refresh a website many times because of slow loading. Checking for frequency alone could also let certain types of attacks through, such as DDoS attacks with a large network of machines with different addresses.

With deep learning, it is possible to let the mitigation system filter normal from malicious traffic autonomously. Network traffic can be fed through a deep learning algorithm, which filters individual packets or flows based on learned features. For this thesis, incoming network packets will be transformed into traffic flows, before being fed to the deep learning algorithms. We propose two separate deep learning algorithms to filter network traffic flows, Latent Layer Classification on a Variational Autoencoder (LLC-VAE), and Loss Based Detection on a Variational Autoencoder (LBD-VAE).
These two deep learning algorithms learn patterns by themselves, instead of relying on older techniques where the attack patterns must be inputted manually.

The contribution of this thesis is to research how, and how well the proposed deep learning approaches, the LLC-VAE and the LBD-VAE, can filter malicious from normal traffic. The LLC-VAE and LBD-VAE will be used to learn from a few types of DDoS and DoS attacks, from the datasets outlined in \cref{methodology-datasets}. While there exists many more types of malicious computer network traffic, the samples in these datasets will be used to analyze whether the two proposed approaches can reliably be used as DDoS and DoS mitigation systems. For the remainder of this chapter, we will present how the two proposed approaches are designed, as well as discuss different options for designing them.

\section{LLC-VAE}
\label{methodology-llc-vae}

The first proposed approach, Latent Layer Classification on a Variational Autoencoder (LLC-VAE), utilize the strength of the variational autoencoder\cite{Kingma-and-Welling-2013}, covered in detail in \cref{background-vae}, as the underlying architecture for a latent layer classification network. Based on the ability of the variational autoencoder to learn latent representations of various classes of a dataset, the LLC-VAE approach aims to classify different types of computer network traffic, and separate normal traffic from malicious. The performance will be documented in \cref{analysis}, \nameref{analysis}, together with how the model performs on different settings.

A representation of the LLC-VAE deep learning model can be seen below in figure \ref{fig:methodology-llc}. First, one flow from the dataset is loaded into memory and transformed to readable format by the model. One flow is represented as one feature vector, and together they are grouped into mini-batches before being fed into the encoder. The encoder performs dimensionality reduction on the mini-batch over multiple layers, further transforming the feature vectors, until they have been encoded to the latent layers\footnote{The hidden layers between the VAE encoder and decoder are called latent layers in this thesis.} of means and standard deviations. Based on this the latent layer $z$ is sampled, and the KL-Loss value is produced. This output, now represented as a vector of nodes with reduced dimensions, is sent to a fully connected layer that outputs the unscaled class predictions. The softmax function, short for softargmax\cite[p.~184]{Goodfellow-et-al-2016}, is applied on the class predictions, so that the nodes are normalized to a legal probability density function (PDF), where each node represents a single class. To optimize the predictions, we use cross entropy over the softmax predictions, to generate a numerical loss value which is called \texttt{prediction loss}, or P-Loss for short. The latent layer $z$ also feeds its vector of nodes to the decoder. The decoder aims to accomplish the opposite of the encoder, increasing the dimensionality through multiple layers to generate a reconstruction of the original feature vector. The reconstructed feature vector is an approximation of the input. These two vectors are compared to generate a reconstruction loss, or R-Loss for short, by using mean squared error. $$L(x) = \dfrac{1}{n}\displaystyle\sum_{i=1}^{N} (y_{i} - x_{i})^{2}$$ Here $x$ represents the model input, $y$ the output, and $n$ the number of features. The values generated from each of the loss functions, R-Loss, KL-Loss, and P-Loss, are combined and optimized over. We use the Adam optimizer by Kingma and Ba\cite{Kingma-and-Ba-2014}, to perform stochastic gradient-based optimization of the model. The optimizer will backpropagate through the network, updating the weights between each layer based on the total loss.

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.7]{img/figures/LLC-VAE.pdf}
    \caption[LLC-VAE Model]{Latent layer classification on a VAE. Rectangles represent node layers. Diamond shapes represent the loss values. The trapezoids represents the shrinking nature of the encoder, and the expanding nature of the decoder. The classification layer is a fully connected layer with a softmax activation function.}
    \label{fig:methodology-llc}
\end{figure}

\subsection{Overfitting and Underfitting}

In machine learning there are two cases of learning that one strives to avoid. One is when a model learns representations of the given training dataset specific to that set, at the expense of degraded results for other datasets. This is called overfitting. To combat overfitting, and yet have the models learn generalized representations, we use a validation set during training, to monitor training and ensure correct learning. On the other hand, a too generalized solution will lead to underfitting. That is when a machine learning model does not have the capacity to appropriate the complexity of a given task.

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.47]{img/figures/overunder.pdf}
    \caption[Overfitting and Underfitting]{This figure is an example of a nonlinear function approximating the true function. Image on left hand side is an example of underfitting, the model has not learned enough. Center image is how we want a model to learn, it has approximated the true function almost perfectly. Right hand image is an example of overfitting, the model has learned to perfectly fit the given data, losing its generalizing ability. This figure is from the scikit-learn open-source code library\cite{scikit-learn}.}
    \label{fig:methodology-overunder}
\end{figure}

Deciding on which features are used for the input vectors fed to the two models, and using proper datasets with both enough information and samples, is vital to creating good machine learning approaches. The two approaches explored in this thesis, already have intrinsic feature selection due to our use of an autoencoder architecture, which inherently performs feature selection through dimensionality reduction, as discussed in \cref{background-autoencoders}. We will also adjust some of the features used for training manually, but will otherwise rely on the autoencoder. Using large amounts of training data can be another way to prevent overfitting, as there is a lesser chance for learning from outliers, randomly occurring correlations, and noisy data. Early stopping is a technique that could be used to optimize learning. Early stopping is when a training session is stopped prematurely based on the results of the validation set. If the results from the validation set gets worse after a certain point, but the training set keeps improving, that is a sign of overfitting, hence the training session can be stopped at that point. This case is however unlikely because we have a large number of network flows to train on, reducing the chance for overfitting as a result of outliers and noise.

\subsection{Deciding Dataset Scaling Technique}
\label{methodology-scaling}

Scaling the datasets used in this thesis is important to allow maximum efficiency for the proposed deep learning algorithms. Scaling brings the tabular data in the datasets from a multitude of different scales, into one notionally common scale. Take for example the range of possible IPv4 addresses compared to the range of possible port numbers. The lowest port number would be 0, while the highest possible would be 65,535 because it is represented as an unsigned 16-bit integer. The range of IPv4 addresses on the other hand would range from 0.0.0.0 to 255.255.255.255, which would be from 0 to 4,294,967,295 when converted to decimals. Keep in mind that this example ignores the IP addresses that are reserved for special use, such as broadcasting addresses. This means that the highest IPv4 address is about 60,000 times as large as the highest port number.

\begin{wrapfigure}{L}{0.5\textwidth}
    \centering
    \includegraphics[scale=0.6]{img/figures/scale.pdf}
    \caption[Feature Scaling]{The maximum for both the IP address feature and port feature are now 1, after using a common scale. The bottom arrow depicts how the port range has been relatively increased to fit into the scaled range of the IPv4 address space.}
    \label{fig:methodology-scale}
\end{wrapfigure}

The reasons for scaling different features to better relate to each other is to improve model accuracy, decrease loss, and improve convergence times. The VAE is based on a neural network architecture, and one way a neural network learns is by looking at changes in the features from the network traffic flows. A problem with this, is that deep learning based models interpret the absolute values of features, and not the relative difference. The loss function is greedy, it tries to optimize on large values first. That is why we should scale the data, to keep the weights of all input features of the same relative importance. E.g.\ if one flow use port 80, and another flow use port 730, which is an increase of 650, then the relationship between those two flows shows a change of about 1\%. However, if two flows had a difference in the decimal value of the IP addresses of about 650, that would only be a change of about $1 \cdot 10^{-5}\%$. Because of this, a small change in the port number feature would be seen as more important than a small change in the IP address feature, to the neural network.

In machine learning there are primarily two different techniques for scaling features. Min-max normalization, which is normalizing the data to fit into the range of 0 to 1 using the formula: $$z_{i} = \dfrac{x_{i} - \min(x)}{\max(x) - \min(x)}$$ Alternatively into the range of -1 to 1 when the data contains negative numbers using: $$z_{i} = 2\; \dfrac{x_{i} - \min(x)}{\max(x) - \min(x)} - 1$$ Another popular method is to standardize the data using standard score for normally distributed data: $$z_{i} = \dfrac{x_{i} - \mu}{\sigma}$$ Using either of these techniques will scale the features to such an extent that change in two different features would carry similar importance. A drawback to using min-max feature scaling is the requirement of knowing the minimum and maximum value of each feature. The datasets CICIDS2017\cite{CICIDS2017} and CSECICIDS2018\cite{CSECICIDS2018}, have many unbounded features, such as \texttt{flow duration} or \texttt{timestamp}. Similarly, standardization requires knowing the true population mean value, which is impossible in the general case, because the datasets are only samples from a larger population. This can be worked around by estimating the true population mean from samples with a t-statistic, but might prove problematic if the samples are not a good, generalized representation of the true population.

As a third option, the features can be scaled using the logarithmic value. This ensures that each feature value would retain their uniqueness, while at the same time scaling down large feature values. Perhaps the greatest advantage of using a logarithmic value is that there is no requirement of knowing the true mean, min, or max values. This makes log scaling a prime candidate for scaling unbounded features. Therefore, very large values are not overly prominent. The problem with log scaling is that it is nonlinear, it punishes higher values more than lower values. E.g.\ given an unbounded feature \texttt{Total bytes}, that shows the total number of bytes transferred in a flow. If one flow transferred 5 bytes, and another 10 bytes, the natural logarithm would measure the relative distance to be $2.3025 - 1.6094 = 0.693$. However, if one flow transferred 1,005 bytes, and another 1,010 bytes, the relative distance would be $6.9177 - 6.9127 = 0.005$. Meaning that changes in features with lower absolute values will be seen as more significant. Using log scaling might occasionally be good, i.e.\ when we want distances of larger values to count less. How log scaling affects the proposed approaches in this thesis will be seen in \cref{analysis}, \nameref{analysis}.

A general problem in text processing when mapping values from one space to another, is the difficulty with mapping contextually similar text into numerically similar values. E.g.\ the letter \texttt{a} and \texttt{b} have ASCII values that are numerically close, but not in pronunciation space. The problem is, how we we remap the alphabetic space to the pronunciation space. In our case, we also have features with contextual similarities that need to be mapped to numerically similar values, which is not necessarily the space it was originally in. E.g.\ the ports in a traffic flow may be numerically close, but are not contextually close in the type of traffic that those ports are used for. This is called embedding. Potential solutions to this problem for specific features could be for example Hamming distance, or word2vec\cite{Mikolov-et-al-2013}. Embedding is a very large research topic in its own right, and due to time constraints will not be implemented in this thesis.

\subsection{Deciding What Type of Layers to Use}

A variational autoencoder is inherently a deep learning algorithm, with multiple hidden layers. There is a minimum of three hidden layers, excluding the input and output layers, with potential for adding more. The encoder and decoder has a minimum of one hidden layer each, while there is one hidden layer $z$ as seen in figure \ref{fig:methodology-llc}, also called the latent layer. There are various types of layers available to use for the encoder and decoder in a VAE, some of which will be explored here. Deciding on how many hidden layers that should be present in the encoder and decoder will be decided through tuning in \cref{analysis}, \nameref{analysis}.

\subsubsection{Fully Connected Layers}

A fully connected layer is the layer typically associated with classification problems in multilayer perceptrons, but is also available to use with other neural networks, such as a VAE. The implementation is fairly simple, all nodes in a layer is connected to all nodes of each adjacent layer, where each node stores the node values, and the connections store the weight values. These values are used to predict the outcome of a given problem during the training process. The outputs of this layer type are calculated with the linear function $\text{outputs} = \text{activation}(\text{inputs} \cdot \text{kernel} + \text{bias})$, where kernel is a weight matrix created by the layer. Using multiple fully connected layers will allow for the classification of nonlinear problems\cite{Irie-and-Miyake-1988}. An example of a fully connected neural network can be seen in figure \ref{fig:background-ann}.

\subsubsection{Recurrent Layers}

Recurrence is primarily used for sequence modeling, that is to say a recurrent layer is able to remember what has been seen previously. Intuitively, implementing memory in a neural network to observe relationships between different traffic flows seems like a good idea, allowing a deep learning model to remember previously seen, as well as ongoing, attacks and their sources. This method has shown some success, as discussed in \cref{related-work}, \nameref{related-work}. An approach that implements a memory mechanic will not be presented in this thesis, but the possibility will be discussed further in \cref{discussion-memory}.

\subsubsection{Convolutional Layers}
\label{methodology-conv-layers}

Convolutional layers can help greatly with classifying network traffic flows, with the ability to create complex feature abstractions from simpler ones in order to understand complex feature relationships. Convolutional layers calculate the outputs linearly in a sliding window manner, using the convolution operation often denoted as $(x * w)(t)$, where $x$ is the input function at a given time $t$ and $w$ is the weighting function\cite{Smith-1997}\cite[p.~327]{Goodfellow-et-al-2016}. Convolutional layers have the ability to capture spatial and temporal dependencies, and are therefore excellent for usage in object detection\cite{Sermanet-et-al-2013}, and image recognition\cite{He-et-al-2016}. Convolutional layers have proven effective for a variety of different problems, including multiple classification problems, and is a strong candidate to use with a VAE. While a fully connected layer learns a representation of an input based on each feature, a convolutional layer selects important features with sliding window detectors, making it better at ignoring redundant information and learning useful representations through multiple abstract feature layers.

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.65]{img/figures/convolutions.pdf}
    \caption[Convolutional Layers in an Encoder]{This figure is a simplification of how the encoder part of the VAE works with convolutional layers. The decoder is similar, but performs the same operations in reverse. The rectangles represent the kernels of size 3 nodes across the height and width dimensions respectively. The squares from the input layer represents 5 features. The trapezoids represents the concept of \texttt{Receptive Fields} in ML. The circles represent the abstract feature nodes of the convolutional layers.}
    \label{fig:methodology-convolutions}
\end{figure}

A convolutional layer learns abstract features from the input layer with a technique called \texttt{sliding window}. A matrix, called a kernel, performs mathematical operations on the node values in a layer, beginning with the feature nodes from the input layer. From the example in figure \ref{fig:methodology-convolutions}, there can be seen a total of 5 features from the input layer. The traffic flows used in this thesis are one-dimensional, hence when defining the kernel size we only need to define the size of a single dimension. From the example, each node in the first convolutional layer learns from nodes 1, 2, and 3 in the input layer. The second node in the first convolutional layer learns from input nodes 2, 3, and 4, while the last node learns from input nodes 3, 4, and 5. Put in another way, each node from the first convolutional layer has a receptive field of size 3. Likewise, the second layer also has a local receptive field of 3. When using multiple convolutional layers, each node in each layer has a local receptive field of a given size, but the effective receptive field size increases every time a layer is added. For example, the first layer in figure \ref{fig:methodology-convolutions} has a receptive field size of 3. The following layer will learn from the feature abstractions of the first layer, causing it to have a local size of 3, but an effective size of 5, in the input layer. This means that the node in the second layer has learned an abstraction from the relations between all the nodes in the input layer.

\subsection{Regularization}

The term regularization has a wide range of uses. Regularizing a deep learning model means preventing overfitting, avoiding exploding and vanishing gradients, and generally keeping the training phase stable and improving various issues. As mentioned in \cref{background-autoencoders}, an autoencoder inherently performs a form of regularization. A VAE specifically, performs dimensionality reduction, and as a result, forces the model to choose the most important features through node selection.

Weight regularization is the addition of a penalty term, to prevent exploding gradients. It can be applied to the hidden layers of the encoder and decoder when using convolutional or fully connected layers. Exploding gradients is a problem for many different neural network architectures, where the layer weights grow out of control causing various issues with the model loss. This could for example be when the loss does not gain traction and does not improve, or the loss could end up with a NaN value, due to floating point overflow. We use the weight decay regularization technique, L2, typically called ridge regression, on the kernel values of the convolutional layers. This will encourage the layer weights to grow towards smaller values around 0. Weight regularization might not be necessary, but does not harm the model performance, and so there is no reason not to implement it.

A regularizing layer can be added after each layer in the encoder and decoder. Two different regularizing layers can be used for the approaches in this thesis, dropout layers\cite{Srivastava-et-al-2014} or batch normalization layers\cite{Ioffe-et-al-2015}. Adding either of these to an encoder and a decoder is meant to ensure stable learning, prevent overfitting, and to improve the exploding and vanishing gradients problem. Dropout is a technique that gives a keep probability to each node in a given model network that updates during training. If a node has a keep probability that has sunken below a given threshold, the weights will be multiplied with 0 during the forward pass, causing the gradients to become 0 during backpropagation. As a result of this, a number of nodes in the model network will effectively be removed, forcing the model to learn more robust features and teaching each layer to rely on different nodes from the previous layer. Batch normalization can be used instead of dropout to prevent overfitting, as well as to prevent vanishing and exploding gradients.

\subsection{Latent Layer Classification}

The encoder and decoder of the VAE can be modified to use different types of layers. To represent the vectors $\mu$, $\sigma$, and $z$, we are using fully connected layers. The output from $z$, as seen in figure \ref{fig:methodology-llc}, is sent to another fully connected layer which attempts to predict the classes that the different flows belong to. A softmax cross entropy loss function is used to improve the classification by performing cross-entropy between the predicted classes, and the labeled true classes. In the dataset CSECICIDS2018\cite{CSECICIDS2018}, there are a total of 8 classes, each used for training and validation by the LLC-VAE. Either of the cross-entropy functions, softmax or sigmoid, could be utilized as loss functions for the LLC. Each flow can only belong to one class, and the higher the probability of a flow belonging to one specific class, the less the probability of that flow belonging to another class. That is to say the class predictions are dependent on each other. For the LLC-VAE we will be using the softmax activation function.

The dataset CICIDS2017\cite{CICIDS2017} have two fewer DDoS classes, for a total of 6. This dataset will be used for testing. Having fewer classes for the test network, compared to the training network, is not a problem, as these 6 classes are present in both datasets, and comparison can be done on these classes alone. However, the test results will give less comprehensive results compared to the validation results. Classifying specific DDoS and DoS attacks could pose a different problem. Although the LLC-VAE is able to classify specific attacks and normal computer network traffic, doing so could lead to less accuracy when differing between normal and malicious traffic. When the model needs to do more than anomaly detection, it is required of it to train more precisely tuned weights for the different flow features. This could mean that the model achieves more precise predictions for specific attacks at the cost overall accuracy. For this reason, both a multi class variant, and an anomaly detection variant will be examined in \cref{analysis}, \nameref{analysis}.

\subsubsection{Latent Layer z}

At the core of the VAE is the latent layer $z$ that samples from the vector of means, and vector of standard deviations, recall the explanation in \cref{background-vae}. The two vectors of means and standard deviations are implemented using fully connected layers that are initialized with random values. Previously we discussed how in a VAE, the term $- D_{KL} (q (z|x) ) \, || \, p (z) )$ is used to approximate the true posterior. This is the KL-Loss term, and can be written as: $$\dfrac{1}{2}\sum_{j=1}^{J} = (1 + log((\sigma_{j})^{2}) - (\mu_{j})^{2} - (\sigma_{j})^{2})$$ The KL-Loss term is used as a measurement of the divergence between two probability distributions, the vector $z$ that samples from $\mathcal{N}(\mu_{i}, \sigma_{i}^{2})$, and the standard normal distribution. The sampled vector $z$  is implemented as $z = \mu + \sigma \cdot \varepsilon$ where $\varepsilon$ is an auxiliary noise variable drawn from the standard normal distribution, $\varepsilon \sim \mathcal{N}(0, 1)$. When minimizing the KL-Loss term, the vector of means $\mu$ and vector of standard deviations $\sigma$ will be optimized to resemble the target distribution. This means we can initialize the two fully connected layers with random values, and let them learn the target distribution during model training. As discussed in \cref{background-vae-detail}.

\begin{figure}[htbp] %{L}{0.5\textwidth}
    \centering
    \includegraphics[scale=0.7]{img/figures/latent_layer.pdf}
    \caption[Probability Distribution of a VAE]{Example of multiple network traffic flows in a classification plot, benign in blue dots and malicious in orange squares. Each data point represents one flow at the latent layer $z$. Each data point has a probability distribution $\sigma$ (seen as an encompassing circle), where each point within that distribution has a higher chance of belonging to the same class as the point from which the distribution originates, compared to data points outside it.}
    \label{fig:methodology-latent-distribution}
\end{figure}

The latent layer $z$ not only learns to describe the input flows $x$, but also representations of $x$ that have similar features. The mean and standard deviation vectors which $z$ sample from give a distribution to each flow. Each flow is represented as a data point, and each point have a probability distribution. Other points within the probability distribution have a higher chance of belonging to the same class, as opposed to a normal autoencoder where each point have a direct encoding, only decoding specific encodings in the latent space. Intuitively, this allows a VAE to not only learn latent representations of seen input features, but generalizes in a way that allows for an interpretation of unseen flows and flow features with slight variations.

\section{LBD-VAE}
\label{methodology-lbd-vae}

The second proposed approach, Loss Based Detection on a Variational Autoencoder (LBD-VAE), is a variant of the first approach. Instead of classifying the different traffic types at the latent layer, the LBD-VAE performs anomaly detection based on the reconstruction loss of the VAE after it has been trained. The LBD is based on the notion that an autoencoder is only able to reconstruct data that has been previously shown to it. Both of the proposed approaches uses the underlying framework of the VAE. This means the decisions about the VAE structure, what layers to use, when to use regularization, how the latent layer operates, etc. will remain mostly the same. The LBD-VAE could end up running on different tuning settings compared to the LLC-VAE, but the parameters available for tuning will remain mostly the same.

An overview of the LBD-VAE can be seen in figure \ref{fig:methodology-lbd}. The figure is separated into two parts, "model 1" and "model 2". These are both part of the LBD-VAE model, but will be separated for easier understanding of how the second approach works. The first part, model 1, is simply an implementation of the VAE by Kingma and Welling\cite{Kingma-and-Welling-2013}, and will be trained separately from the second part, model 2. To begin training the LBD-VAE, first we will create a dataset containing exclusively benign computer network traffic from the CSECICIDS2018\cite{CSECICIDS2018} dataset. The idea is that by only training model 1 on benign data, the VAE will only learn the patterns of those types of flows, and as a side effect, be unable to recognize malicious data. Training only on benign data also means that the LBD-VAE have the potential of being a robust mitigation system against any type of attack.

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.6]{img/figures/LBD-VAE.pdf}
    \caption[LBD-VAE Model]{Loss based detection on a VAE. Rectangles represent node layers. Diamond shapes represent the loss values. The trapezoids represents the shrinking nature of the encoder, and the expanding nature of the decoder. The classification layer is a fully connected layer with a sigmoid activation function. The surrounding frames depict two stages of model training. First model 1 is trained to completion, then model 2 is trained, based on the reconstruction loss of model 1.}
    \label{fig:methodology-lbd}
\end{figure}

\subsection{Loss Based Detection}

When training the LBD-VAE, first we need to train the first part, model 1, to completion. After having trained model 1 on exclusively benign data, the idea is that the reconstruction loss will be low for benign data, and higher for malicious data. After that the second part, model 2, is trained based on the reconstruction loss from model 1. During training of model 2, we will be using a mixed dataset with both benign and malicious computer network traffic flows. The input data is fed through the whole model, starting from input $x$ as seen in figure \ref{fig:methodology-lbd}. Each flow will generate a KL-Loss and a R-Loss value, but only the R-Loss will be used to train model 2. The R-Loss will be the only feature used in training a fully connected layer that outputs the unscaled class predictions. To generate a prediction loss value (P-Loss), we perform cross-entropy on the unscaled class predictions with either a softmax or sigmoid activation function\footnote{Both functions can be used here, and can be considered equivalent for a binary classification problem:\\$\text{Sigmoid} = \dfrac{1}{1 + e^{-x}} = \dfrac{1}{1 + \dfrac{1}{e^{x}}} = \dfrac{1}{\dfrac{e^{x} + 1}{e^{x}}} = \dfrac{e^{x}}{1 + e^{x}} = \dfrac{e^{x}}{e^{0} + e^{x}} = \text{Softmax}$}. When performing backpropagation based on the P-Loss to update the weights and node values of model 2, it is important to prevent backpropagation through model 1. In Tensorflow, this can be done by treating the reconstruction loss as a constant, with the use of the function \texttt{tf.stop\_gradient()}. This ensures that model 2 will be trained separately from model 1, and prevent the P-Loss from interfering with the weights and node values of model 1. Failing to prevent backpropagation through model 1 from model 2 would cause the first part to learn from malicious data, which would defeat the purpose of the LBD-VAE approach.

\begin{figure}[htbp]
    \centering
    \includegraphics[scale=0.7]{img/figures/threshold_example.pdf}
    \caption[Example Probability Distribution Function Graph of the LBD Threshold]{Example of a benign and a malicious probability distribution being separated by a linear classifier.}
    \label{fig:methodology-pdf-graph-example}
\end{figure}

An example visualization of how the LBD-VAE will separate benign and malicious traffic can be seen in figure \ref{fig:methodology-pdf-graph-example}. The figure is of two probability distribution functions, the benign data distribution and the malicious data distribution. The vertical line at the center represents the threshold, which is defined by the linear classifier from model 2, as seen in figure \ref{fig:methodology-lbd}. The threshold classifies any incoming computer network flow into one of two classes based on the reconstruction loss of the flow, after passing it through model 1. The idea behind the LBD-VAE is simple. After training model 2, benign and malicious flows will be grouped into two probability distributions. The lower the loss, the higher probability for a flow to be classified as benign. Although the idea is simple, there are multiple challenges with using a linear classifier to separate the flows. One of the major difficulties lies in training the model to be able to recognize different flows. From figure \ref{fig:methodology-pdf-graph-example}, the two probability distributions are fairly well separated, but it could be that they, in reality, end up overlapping to a much higher degree. It could be that using only the reconstruction loss, and feeding it to a linear classifier, is insufficient in handling this problem. To find out whether this is the case, we will train, validate, and test the performance of the LBD-VAE. The results will be documented together with the results from the first approach in \cref{analysis}, \nameref{analysis}.

\end{document}


==> parts/preface.tex <==
\begin{document}

\chapter*{Acknowledgment}

I would like to express my gratitude to my supervisors Hårek Haugerud and Anis Yazidi for their feedback and help. Our discussions helped me steer this thesis in the right direction, and kept me focused on the tasks at hand.

My sincere thanks and appreciation to my dear friend Johan Korsmo, for going out of his way to proofread this work in its entirety. He has been an excellent discussion partner, who has helped me greatly.

Acknowledgments should also be displayed to Toril Molde, for going through and correcting the grammar in this thesis.

Moreover, I would like to express my thanks to the researchers at the Canadian Institute for Cybersecurity, for making the datasets used in this thesis publicly available.

\end{document}


==> parts/related_work.tex <==
\begin{document}

\chapter{Related Work}
\label{related-work}

Techniques to combat DDoS and DoS attacks are many and varied. Some focus on stateless packet information, others rely on meta information from stateful packet flows, fore more in depth on these topics see \cref{background-packet-state}. In this section, we will provide a few relevant research papers and topics in order to create an overview of different strategies and methods to both discover and mitigate DDoS and DoS attacks. We will also present research that aims to improve or adapt existing techniques relevant for our research or future research.

\section{Data Mining and Density-based Geographical Clustering}
IP addresses, although not always reliable to pinpoint exactly where a connection is based, provide the general geographical location such as country and city, unless the address is spoofed or hidden in layers of redirection. Rønning proposed two novel methods for DDoS mitigation, specifically for HTTP flooding, based on hidden data structures in historical traffic\cite{Roenning-2017}. The first method is \textit{A priori}-based frequent networks (AFN), used to discover common known prefixes during training and relating it to unknown data later on. \textit{A priori} in this context is a form of association rule learning, used to investigate frequent item sets and discovering relationships between data variables. The idea is that frequent networks will repeat to a high degree. This means that it will familiarize itself with networks seen often, and thus notice unknown data patterns, such as those from DDoS.

The second method aims to mitigate DDoS based on the geographical location and anomaly detection techniques, using clustering methods. Two algorithms are used for clustering, the simple version, a density-based geographical clustering (DGC), and a variant that aims to improve on this algorithm, called reduced-density geographical clustering (RDGC). At its core, DGC estimates data patterns based on geographical locations, so that if network $z$ is close to a network $x$ that has previously successfully reached a server, then $z$ has a higher chance of reaching the same server. Since this is a clustering algorithm, the clusters must first be defined. The location of the frequent networks are chosen as core points, and all points within a given range threshold of the core, or within a given range threshold of the points belonging to the core, will be grouped together and used to define a cluster. A weakness mentioned by the author, is that DGC might be too simple, allowing too many data points to be clustered. RDGC improves the first algorithm by adding further constraints, such as how many points must be in a cluster lest it be disbanded. After three real life simulations, AFN achieved an acceptance rate of 92.83\% for legitimate traffic, and 99.89\% for illegitimate traffic respectively. RDGC achieved an 77.54\% and 99.93\% respectively. DGC achieved 57.59\% and 99.99\% respectively.

\section{Adaptive History-based IP Filtering}
Goldstein et al.\cite{Goldstein-et-al-2008} proposed an adaptive history-based IP filtering algorithm (AHIF) to automate the process of creating and modifying IP filtering rules for anomaly detection. The mitigation system is applied before traffic is allowed through to the target, so a potential DDoS attack is stopped by rules that are prepared before the attack takes place. Bayesian theory is applied to observed data in order to derive a risk function, based on overall loss. Their approach use this to optimize packet filtering rules by minimizing risk under a certain threshold.

A server that can handle N packages in a given time frame needs to keep traffic load below N. This means that optimally the packages with the highest probability of being legal traffic can be let through, up to a total of N. In practice the AHIF algorithm use a variable threshold to define how much traffic the server can handle at a given time. This all happens before each package is sent through to the server, allowing for quick processing time, and stable servers. In the paper, it is argued that a certain amount of DDoS traffic can be allowed through, as long as the server runs smoothly. Therefore the packages with the highest probability of being legal traffic, even if that includes DDoS, will be allowed through. Only the necessary amount of packets to keep a stable server will be dropped. By adapting the threshold variable during runtime to fit the server load, the practical approach reaches similar results to the theoretically optimal approach.

The practical implementation of this method comes in the form of a binary tree keeping track of the IP addresses, with maximum depth of $n$ where $n$ is the most significant bit, at a maximum of 24. The last 8 bit are not used, with the reasoning that IP addresses can be easily spoofed, especially the last 8 bits, and because many different users might have many different addresses within a 24 bit network mask due to for example DHCP\footnote{Dynamic Host Configuration Protocol, an application layer protocol. Used dynamically assign IP addresses to each device on a network.}. Using 24 bits as maximum depth leads to a maximum of $2^{24}$ number of rules. Processing this amount of rules could take a great amount of time. To combat this problem, a system to prune children leaves to a common parent is implemented, effectively compressing the tree in a way that leads to no loss of rules, and a smaller $n$. The system made by Goldstein et al.\cite{Goldstein-et-al-2008} was able to handle about 100,000 firewall rules at a rate of 40,000 requests per second.


\section{Flow-based Stacked Autoencoder in SDN}
Niyaz et al.\cite{Niyaz-et-al-2016} presents a DDoS detection system for Software-Defined Networks (SDN), that use deep learning to detect multi-vector DDoS attacks from flow traffic, see \cref{background-packet-state}. In a SDN, DDoS attacks happens on the data plane or control plane\footnote{The data plane in a SDN forwards traffic, while the control plane manages what route the traffic will take.}, and their system is thus focused on detecting DDoS on these two planes. Their detection system consists of three modules which they call "Traffic Collector and Flow Installer", "Feature Extractor" and "Traffic Classifier". These modules work to extract multiple different headers from TCP, UDP and ICMP packets, and generate a flow to be fed into the DDoS detection system. Each packet belonging to the same flow has the same source and destination IP, the same source and destination ports, and the same protocol type.

Multiple sparse autoencoders (SAE) are used together to form a deep learning network by stacking them after each other\cite{Niyaz-et-al-2016}. There are two ways to do this, one is to encode and decode as usual on the first autoencoder, and feed decoded output to the second autoencoder, and so on. Another method is to encode and decode as usual for training the network, but instead of using the decoded outputs, the latent layer outputs are fed to the next autoencoder in the line. So if we have the raw input $x$ feeding into the first SAE, it will be encoded into the latent layer values $g$ and decoded to $\hat{x}$. The values $g$ are used as input for the second SAE, which encodes to latent layer values $h$. After this, they apply a softmax classifier on the outputs of $h$\cite{Niyaz-et-al-2016}. The final stacked autoencoder consists of two models with a classifier at the end.

For training and testing, their flow generation system extracts and creates a total of 68 features\cite{Niyaz-et-al-2016}, although separated into three protocols, TCP, UDP and ICMP. Attacks were simulated using Hping3, and Niyaz et al. claim to identify individual DDoS classes with an accuracy of about 95\%. The accuracy for differing between normal and attack traffic is claimed to be 99.82\%.


\section{Anomaly Detection on the CICIDS2017 Dataset Using LSTM}
\label{related-lstm-2017}

In networking, traffic is sent back and forth between machines, and some packets can be said to have a relation to each other, such as the packets transferred during a three-way-handshake. If multiple machines cooperate to send a DDoS attack, it is considered to be the parts of the same attack, even though there are multiple sources. Using machine learning to detect the relationship between packets or flows could potentially allow mitigation methods to prevent malicious traffic based on learned patterns in IP addresses and traffic frequency. Pektas and Acarman\cite{Pektacs-and-Acarman-2018}, and Radford et al.\cite{Radford-et-al-2018}, proposed two different detection methods in their respective papers using the CICIDS2017 dataset\cite{CICIDS2017} amongst others, which will be used in this thesis as well. This dataset, discussed further in \cref{methodology-2017}, is a modern dataset containing network traffic data, both normal and malicious. It is meant for research, as a benchmark for developing detection and mitigation methods.

A method to group together network flows into two-dimensional arrays was proposed by Pektas and Acarman\cite{Pektacs-and-Acarman-2018}. The proposed system aims to detect malicious network traffic using the combination of a convolutional neural network (CNN) and a long short-term memory (LSTM)\footnote{LSTM is based on a recurrent neural network architecture.} network, to learn spatial-temporal features. Each network flow is grouped based on source and destination IP, destination port, protocol, flow direction, and label. Then the group is fed through the model as a 2D array, where each row represents one flow, sorted by their timestamps. If a group consists of a number of flows less than a given threshold value, the group is omitted. This could be considered as a form of frequency based detection added on top of the detection algorithm using a hyper parameter. Since malicious traffic, especially DDoS and DoS attacks, rely on sending large amounts of packets or flows in a given time frame. To configure the model network, a Tree-structured Parzen Estimator (TPE) is used, to tune the model automatically based on hyper parameter search. The authors claim the model is able to detect attack traffic at an accuracy of 99.09\%.

Radford et al.\cite{Radford-et-al-2018} proposed a method for anomaly detection using sequence modeling, utilizing a recurrent neural network (RNN) architecture with a LSTM model\footnote{A RNN is a neural network with the ability to remember previous data inputs. LSTMs is an improvement on this concept, increasing the memory capabilities.}. Five different sequence aggregation rules based on the flows provided in the CICIDS2017 dataset are evaluated using a LSTM model. The research in their paper is partially based on their previous work\cite{Radford-et-al-2018-r7-1}. Once a sequence of computer network traffic flows of length 10 has been generated, it is fed through the LSTM model. There the sequence is given a prediction of whether it is normal or malicious traffic, based on an outliers score\cite{Radford-et-al-2018} and measured using mean area under the curve (AUC). For baseline comparison, a simple frequency based method for outliers detection was used. The sequence aggregation with an LSTM model proved slightly better in a few cases, but was mostly on-par with the frequency based model, or worse. Whether this was because of the LSTM model or the sequence aggregation methods were deemed uncertain.


\section{Malicious traffic detection using entropy-based techniques}
Entropy, from information theory, is a measurement of uncertainty or disorder in a system, often called Shannon entropy\cite{Shannon-2001}. It is a value representing the average rate of information being drawn from a stochastic source of data. A source of data producing an entropy value closer to 1 when normalized is considered hard to predict, and a value closer to 0 is considered easier as there is less uncertainty. Behal et al. proposed the usage of generalized information entropy (GE) and generalized information distance (GID) for separating so called low rate DDoS (LW-DDoS) and high rate DDoS (HR-DDoS) from normal traffic and flash events (FE)\cite{Behal-and-Kumar-2017}. The idea is to group network traffic into sets, where packets were grouped together in 10 second time frames. The entropy and information distance is then measured for each set. It was discovered that DDoS traffic flows had more similar traffic, as their IP addresses are more closely grouped in relation to time. This leads to lower entropy values within a set containing more DDoS traffic, and higher information distances between normal and DDoS traffic.

To better understand the relationships between different features in network traffic and how they can be used for anomaly detection, Nychis et al. published an empirical evaluation on the subject, using entropy\cite{Nychis-et-al-2008}. Features were gathered from bi-directional flow data. The relationships between the features source IP, destination IP, source port, destination port, in-degree, out-degree and flow size distribution (FSD) were measured using entropy, and given correlation scores. Note that FSD is the packet per flow measurement. The study found high correlation between certain features, perhaps most notably between ports and IP addresses. However it was also found that the correlation between ports and addresses had limited usability for anomaly detection, and argued that they are ineffective for both scanning and flood type attacks. Interestingly, the FSD and degree distribution scores had some success in detecting anomalies, and the entropy scores between normal traffic and malicious traffic had a noticeable difference\cite{Nychis-et-al-2008}.


\section{Flow-based DoS attack Detection with techniques based on Computer Vision}
Autoencoders from machine learning can be used for anomaly detection, by separating malicious from normal traffic using pattern recognition. If a data input fed into the model is not recognized, it would be considered an anomaly. Tan et al. proposed the use of computer vision techniques for anomaly detection in network traffic, specifically for DoS attack traffic\cite{Tan-et-al-2015}.

Features from inbound network traffic is fed through the detection system, and stored as one-dimensional feature vectors called records. In computer vision, earth mover’s distance (EMD) can be used to detect dissimilarities between two images. To apply this idea to their system, Tan et al. transforms inbound records into two-dimensional matrices, similar to images. Profiles for normal network traffic is generated based on multivariate correlation analysis (MCA) from previous work\cite{Tan-et-al-2014-r13-1}. MCA works to find correlation between features and generating normal records from the inbound records coming from the datasets. Then a reformulation of EMD\cite{Ling-and-Okada-r13-2} is applied to the generated record matrices, measuring dissimilarities between each record. Any unmatched records will be determined as attacks. Evaluation of the detection system on the KDD’99\cite{KDD99} dataset was reported to have achieved 99.95\% accuracy, and on the ISCXIDS2012\cite{Shiravi-et-al-2012} dataset to be 90.12\%. Both these datasets, and others, will be discussed in \cref{methodology-available}.


\section{Anomaly Detecting With Hidden Semi-Markov Model}
Hidden Markov models (HMM) have a variety of different applications, such as research on time series data or for sequence recognition. Xie and Yu proposed a solution for detecting application layer DDoS attacks as anomalies by learning from user behavior on web pages with a hidden semi-Markov model (HsMM)\cite{Xie-and-Yu-2009}. HsMM is an extension of HMM that adds an explicit state duration, and is made for live training. The HsMM is a behavior model that learns from looking at normal user behavior in regards to how they behave when browsing a given web page, using the address bar, hyper links and reading web page content. From this, a normal user is defined with a mean entropy value which will be used for comparison with the filter. Requests from an outside source reach the victim web page, and are stored over time as a request series, or as it is called in the paper, a HTTP request sequence, similar to how network packets would be handled by a RNN. The average entropy of this sequence is calculated at the detection system filter, and used for comparison with the entropy from the generated user behavior characteristics, made by the HsMM. The research and experiments in the paper were only tested on application layer DDoS attacks, but showed promising results, with as much as 98\% detection rate.

Not many solutions for detecting or mitigating DDoS and DoS attacks focus on learning from user behavior. It could be a potential avenue for further research.

\end{document}

